An RKHS Approach to Estimation with Sparsity Constraints

The investigation of the effects of sparsity or sparsity constraints in signal processing problems has received considerable attention recently. Sparsity constraints refer to the a priori information that the object or signal of interest can be represented by using only few elements of a predefined dictionary. Within this thesis, sparsity refers to the fact that a vector to be estimated has only few nonzero entries. One specific field concerned with sparsity constraints has become popular under the name Compressed Sensing (CS). Within CS, the sparsity is exploited in order to perform (nearly) lossless compression. Moreover, this compression is carried out jointly or simultaneously with the process of sensing a physical quantity. In contrast to CS, one can alternatively use sparsity to enhance signal processing methods. Obviously, sparsity constraints can only improve the obtainable estimation performance since the constraints can be interpreted as an additional prior information about the unknown parameter vector which is to be estimated. Our main focus will be on this aspect of sparsity, i.e., we analyze how much we can gain in estimation performance due to the sparsity constraints.

==> Chap_CS.tex <==
\chapter{Application to Compressed Sensing}
\label{chap_CS}
\section{Introduction}

REVIEW OF COMPRESSED SENSING

The basic measurement equation of CS is given by 
\begin{equation}
\label{equ_CS_measure_model}
\mathbf{y} = \mathbf{M} \mathbf{x} + \mathbf{n} 
\end{equation}
where $\mathbf{M}$ is the CS measurement matrix. 
In general on is interested in recovering the signal vector $\mathbf{s}$ itself from the compressive measurements $\mathbf{y}$. 
%The problem of estimating $\mathbf{x}$ from $\mathbf{y}$ is usually refered to as the ``CS-recovery'' problem. 
An estimation theoretic analysis of the CS recovery problem has been already given in \cite{BabAympAchievCRBSLM} where the authors 
show (under certain technical conditions) the asymptotic (i.e., the signal dimension $N \rightarrow \infty$) achievability of the \CRBfull associated with the problem of estimating $\mathbf{s}$ based on $\mathbf{y}$. 

In the following we will perform an estimation theoretic analysis for a finite dimensional setting of two estimation problems based on the 
measurement equation \eqref{equ_CS_measure_model}. The first estimation problem is that of minimum variance estimation of the signal vector $\mathbf{s}$ itself
which will be seen to be nothing but the SLM presented in Chapter \ref{Chap_SLM}. The second estimation problem is based on the SPCM presented in Chapter \ref{Chap_SCM} consists of minimum variance estimation 
of a parameter $\mathbf{x}$ that determines the covariance of the signal vector $\mathbf{s}$ which is here modeled as a random vector. 

\subsubsection{Restricted Isometry Property and Coherence}
\section{The CS viewpoint of the Sparse Linear Model}
Obviously, except for the different symbol used for the system matrix and parameter or signal vector, the CS measurement model is identical to the observation model \eqref{equ_observation_model} of the SLM.
Therefore in principle we could use the analysis for the SLM to obtain performance bounds for CS recovery schemes, since any
CS recovery scheme can be interpreted as an estimator that tries to estimato $\mathbf{x}$ from observing $\mathbf{y}$. 

However, there is one practical issue that prevents us from directly using our results. Since the performance bounds for the SLM have been 
formulated in terms of sub-matrices of the system matrix, for the CS application one would have to evaluate any specific sub-matrix of the CS measurement matrix $\mathbf{M}$ 
but this is in general not possible due to the large dimensions of the matrix $\mathbf{M}$. 
Therefore we will generalize our analysis of the SLM to obtain performance bounds in terms of certain incomplete information about the matrix $\mathbf{M}$. Within CS such 
an incomplete information describing the properties of $\mathbf{M}$ is given by the restricted isometry property (RIP) \cite{Can06a,Can05} and the concept of coherence \cite{GreedisGood,JustRelax} whose definitions are 
now repeated for convenience: 
\begin{definition}[Restricted Isometry Property]
A matrix $\mathbf{M}$ is said to satisfy the RIP of order $K$ with corresponding RIP constant $\delta_{K}$ if and only if 
\begin{equation} 
\end{equation} 
\end{definition} 
\begin{definition}[Coherence]
\end{definition}

The lower bounds for the CS reconstruction problem basically reformulate the results of Sec. \ref{chap_CS} directly in terms on the RIP constants and coherence. 


%\section{The CS viewpoint of the Sparse Covariance Model}

\section{Compressive Spectrum Estimation}

Compressive spectrum estimation combines techniques from Compressed Sensing with classical spectrum estimation \cite{jung-icassp09,jung-ssp09}.
In principle, the problem is to estimate the correlation structure of a random process $X[n]$ (which is assumed Gaussian and zero-mean) from the observation of a finite length segment of a single realization $x[n]$. 
We will represent the observed finite length segment by a vector $\mathbf{x}$. 

A compressive spectrum estimator does not process the observed signal directly but rather computes 
compressive measurements. While in \cite{jung-icassp09} the compressive measurements are computed linearly by determining the inner products of the signal segment with a small number of random reference signals, 
the method proposed in \cite{jung-ssp09} uses random samples of the ambiguity function $A_{x}[k,l]$ as nonlinear compressive measurements.

%In the following we will use and adapt the RKHS based analysis of sparse covariance estimation so far to derive performance bounds for the compressive spectrum estimators presented in \cite{icas}. 
\subsection{Spectrum Estimator using Linear Measurements} 

The basic setting of the compressive estimator proposed in \cite{jung-icassp09} is as follows: 
We are given compressive measurements $\mathbf{y}$ of the observed realization of the process segment $\mathbf{x}$ and try 
to infer the covariance structure of the process $X[n]$. The compressive estimator does this by implicitly estimating the covariance matrix $\mathbf{C}_{\mathbf{x}}$ of the observed segment.
It is also assumed that the covariance matrix is sparse w.r.t to a certain ONB. In particular this ONB has to consist of signals that are well TF localized, e.g. a local cosine basis. 
We can then represent the etimation problem by a SCM: 
\begin{equation}
\mathbf{y} = \mathbf{M} \mathbf{x} + \mathbf{n} 
\end{equation}
where $\mathbf{M}$ represents the CS measurement matrix and $\mathbf{n} \sim \mathcal{N}(\mathbf{0},\sigma^{2} \mathbf{I})$ with known $\sigma^{2} > 0$. 
Furthermore, we assume that the rows of $\mathbf{M}$ are orthogonal, i.e., $\mathbf{M} \mathbf{M}^{T}$. This assumption simplifies the analysis and is not too restrictive since 
the popular class of CS measurement matrices given by partial Fourier matrices \cite{} satisfies this assumption. 



\subsection{Spectrum Estimator using Nonlinear Measurements} 
Here we consider a different observation model. Instead of performing linear measurements on a
signal whose covariance structure is determined by the parameter to be estimated we 
consider the observation of a linear transformed version of the sample covariance matrix constructed by 
the random vector whose covariance is determined by the vector to be estimated. 

For a first analysis we will ignore the linear transformation and consider performance bounds for estimators that 
observe the sample covariance matrix of one single observation of the random signal $\mathbf{s}$. 
Since $\mathbf{s}$ is distributed Gaussian with zero mean and covariance matrix $\mathbf{C}(\mathbf{x})$ the 
sample covarance matrix $\mathbf{S} \triangleq \mathbf{s} \mathbf{s}^{T}$ (which is random since $\mathbf{s}$ is random) 
is Wishart distributed. Since we consider only 1 observation which is smaller than the rank of $\mathbf{C}(\mathbf{x})$ 
the random sample covariance $\mathbf{S}$ follows a singular Wishart distribution $\mathcal{W}(1,\mathbf{C}(\mathbf{x}))$ \cite{UhligSingularWishart}. 

 






==> Chap_ExpFam.tex <==
\chapter{Generalization: The Sparse Exponential Family}
\label{chap_ExpFam}
\section{Formulation of the estimation problem}
\section{Reobtaining the SLM and the SPCM as special cases} 
\section{The cumulant generating function} 
\section{Lower Variance Bounds for the sparse exponential family} 
\subsection{Re-derivation of SLM and SPCM bounds}
Show how bounds for SLM and SPDCM can be unified via a bound for the sparse exponential family. 
\subsection{New bounds based on isometry}
use isometry of RKHS with the RKHS associated with kernel $R(x1,x2) = beta(x1-x2+x0)$. where beta is given by the cumulant generating function 

\section{Necessity of strict sparsity} 

% 






==> Chap_SCM.tex <==
\chapter{The Sparse Covariance Model}
\label{chap_SCM}
\section{Introduction}


We consider the problem of estimating an unknown parameter vector $\mathbf{x} \in \mathbb{R}^{N}$ using only the 
observation $\mathbf{y} \in \mathbb{R}^{M}$ given via 
\begin{equation}
\label{equ_obs_model}
\mathbf{y} = \mathbf{s} + \mathbf{n} 
\end{equation}
where $\mathbf{n}$ denotes a white Gaussian noise vector, i.e., $\mathbf{n} \sim \mathcal{N}(\mathbf{0}, \sigma^{2} \mathbf{I})$ with known variance $\sigma^{2} > 0$. 
%The measurement matrix $\mathbf{A} \in \mathbb{R}^{M \times N}$ is assumed fixed and known. 
The random signal vector $\mathbf{s}$ is independent of $\mathbf{n}$ 
and distributed as 
\begin{equation}
\label{equ_cov_model}
\mathbf{s} \sim \mathcal{N} (\mathbf{0}, \mathbf{C}(\mathbf{x})) \quad \mbox{,}  \quad \mathbf{C}(\mathbf{x})  \triangleq \sum_{l=1}^{N} \mathbf{C}^{(l)} x_{l}
\end{equation}
%with a covariance matrix of the form 
%\begin{equation}
%\label{equ_cov_model}
%\mathbf{C}(\mathbf{x})  \triangleq \sum_{l=1}^{N} \mathbf{C}^{(l)} x_{l}
%\end{equation}
with the fixed and known positive semidefinite (PSD) matrices $\mathbf{C}^{(l)} \in \mathbf{S}_{+}^{M}$, whose ranks are denoted by $r_{l} \triangleq \mbox{rank}(\mathbf{C}^{(l)})$. 

To summarize, the probability density function (pdf) $f(\mathbf{y}; \mathbf{x})$ of the observation $\mathbf{y}$ parametrized by $\mathbf{x}$ is given as 
\begin{equation}
\label{equ_param_pdf}
f(\mathbf{y}; \mathbf{x}) = \frac{\exp \left(- \frac{1}{2} \mathbf{y}^{T}  (\mathbf{C}(\mathbf{x}) + \sigma^{2} \mathbf{I})^{-1} \mathbf{y} \right)}{(2 \pi)^{M/2} \mbox{det}^{1/2}(\mathbf{C}(\mathbf{x})+\sigma^{2} \mathbf{I})} . 
\end{equation} 

The central assumption for our scope is that of a sparse parameter vector, i.e., we require 
\begin{equation}
\label{equ_sparsity_constr}
\mathbf{x} \in \mathcal{X}_{S,+} \triangleq \{ \mathbf{x}'  \in \mathbb{R}_{+}^{N} \big| \| \mathbf{x}' \|_{0} \leq S \}, 
\end{equation}
with the fixed and known sparsity degree $S$ where typically $S \ll N$. 
In words, we assume that the vector $\mathbf{x}$ has at most $S$ positive nonzero values. Such an assumption can be used 
e.g. in a cognitive radio scenario where the elements of $\mathbf{x}$ represent the received power at a given time in a given frequency band. 
We coin the estimation problem given by the observation model \eqref{equ_obs_model} and the sparsity constraint \eqref{equ_sparsity_constr} the 
sparse covariance model (SCM). 



%The sparse covariance model is defined by the observation pdf 
%\begin{equation}
%f(\mathbf{y}; \mathbf{x})  = \mathcal{N}(\mathbf{0}, \mathbf{C}(\mathbf{x})+ \sigma^{2} \mathbf{I})
%\end{equation}
%with 
%\

%meter vector $\mathbf{x}$ and the matrix $\mathbf{U} \in \mathbb{R}^{MÊ\times N}$ is fixed and known and satsifies some 
%sort of RIR property as we will discuss in detail later on. 
%We allow that some coefficients of $\mathbf{x}$ may occur more than once in the diagonal. 

%Sparsity is enforced on the parameter vector $\mathbf{x}$ via requiring that 
%\begin{equation}
%\mathbf{x} \in \mathcal{X}_{S,+} \triangleq \mathcal{X}_{S} \cap \mathbb{R}^{N}_{+}.   
%\end{equation}


\section{RKHS formulation}
In contrast to the SLM the RKHS formulation is possible only if we restrict domain of the RKHS to $x < 2 x_0$. This 
problem could be circumvented e.g. by using a finite (linear) model or expansion of the estimator and 
using the RKHS formulation for the coefficients of the model. However, the RKHS formulation for the coefficients will in general 
not allow for an exact analytic treatment since the specific properties of the finite esimtator model have to be considered. 

The kernel of the RKHS associated to the SCM given by \eqref{equ_obs_model} and \eqref{equ_cov_model} can be calculated as 
\begin{align} 
\label{equ_kernel_SCM} 
R(\mathbf{x}_{1}, \mathbf{x}_{2})  = \frac{ \det^{1/2} \left( \mathbf{C}_{\mathbf{x}_{0}} \right)}{ \det^{1/2} \bigg( \mathbf{C}_{\mathbf{x}_{1}} \mathbf{C}_{\mathbf{x}_{2}} \big( \mathbf{C}_{\mathbf{x}_{1}}^{-1} + \mathbf{C}_{\mathbf{x}_{2}}^{-1} - \mathbf{C}_{\mathbf{x}_{0}}^{-1} \big) \bigg)}
\end{align}
where we used the shorthand $\mathbf{C}_{\mathbf{x}} \triangleq \mathbf{C}(\mathbf{x}) + \sigma^{2} \mathbf{I}$. 

%\section{Minimum Variance Estimation for the SCM}




\section{The Sparse Diagonal Covariance Model (SDCM)}
\subsection{RKHS associated to SDCM} 
Discussion of why the RKHS approach can only be used if one additionally restricts the parameter sets. 

\subsection{Class of Estimable functions} 
Description of the class of estimable functions for the SDCM via the RKHS - restriction theorem, i.e., consider all restrictions 
of elements of an RKHS with same functional form kernel as SDCM but whose domain is $\mathbb{R}^{N}$. 

\subsection{Characterization of mean function of LMV} 
Discussion of the behavior of the estimator mean for parameters outside the additional restriction that was used for the RKHS approach. 

\subsection{Variance Bounds for the Sparse Diagonal Covariance Model (SDCM)}
The Sparse Diagonal Covariance Model is the special case of the SCM where the PSD matrices $\mathbf{C}^{(l)}$ are projection matrices onto orthogonal subspaces.
\subsection{Special case: Unbiased Estimation for the SDCM}

\subsection{Nonexistence of UMVU estimator for $S < N$} 
The non-existence of a UMVU estimator is a straight consequence of the fact that for $S < N$ the LMVU depends on $\mathbf{x}_{0}$. Can this be proven for the general SCM ???? (Seems to be hard !) 

\subsection{If a UMVU exists for the SDCM it will not exploit sparsity}
This can be proven using the uniqueness (if it exists) of a LMVU together with the fact that the LMVU for $\mathbf{x}_{0} = \mathbf{0}$ is the ordinary non-sparse esitmator...  Can this be proven for the general SCM ???? (Seems to be hard !) 



\section{Variance Bounds for the general SCM} 
The analysis so far relied heavily on the fact that the component PSD matrices $\mathbf{C}^{(l)}$ in the SCM \eqref{equ_cov_model} are projection matrices onto orthogonal subspaces of the observation space $\mathbb{R}^{M}$.
From a theoretical and also practical perspective it would be desirable to have a similar analysis for the general case of arbitrary PSD matrices $\mathbf{C}^{(l)}$. This seems to be difficult since in general the kernel \eqref{equ_kernel_SCM}
of the SCM does not have this appealing factorized form as for SDCM. 

However, we will reuse the analysis of the SDCM and derive lower bounds on the estimator variance for the general case. 
These bounds are the more accurate the closer the matrices $\mathbf{C}^{(l)}$ are to the case of the SDCM. 
In particular we will assume that the matrices $\mathbf{C}^{(l}$ are of the form 
\begin{equation} 
\mathbf{C}^{(l)} = \sum_{k=1}^{r_{l}} \mathbf{a}_{l_{k}} \mathbf{a}_{l_{k}}^{T} 
\end{equation} 
where $\mathbf{a}_{l_{k}}$ is the $l_{k}$th column of a matrix $\mathbf{A}^{M \times N}$, which will be called the ``dictionary''.  
The only requirement we place on the matrix $\mathbf{A}$ is  
\begin{equation} 
\spark(\mathbf{A}) > 2 S. 
\end{equation} 

We will use the fact that reducing the parameter set can only result in  a lower Barankin bound together with the invariance principle. This allows us to reuse our analysis for the SDCM. 

***********************************************************

The main tool for the generalization of the results for the SDCM to the general SCM will be an inversion formula for block matrices: 
\begin{lemma}[Schur complement]
Given the block matrix $\mathbf{M} = \begin{pmatrix} \mathbf{A} & \mathbf{B} Ê\\ \mathbf{C} & \mathbf{D}  \end{pmatrix}$ where the matrix $\mathbf{A}$ is invertible, we have the following inversion forumula 
\begin{equation} 
\mathbf{M}^{-1} =  \begin{pmatrix} \mathbf{A}^-1 + \mathbf{A}^{-1} \mathbf{B} \mathbf{S}^{-1} \mathbf{C} \mathbf{A}^{-1} & -\mathbf{A}^{-1} \mathbf{C}\mathbf{S}^{-1}   Ê\\ -\mathbf{S}^{-1} \mathbf{C} \mathbf{A}^{-1}& \mathbf{S}^{-1}  \end{pmatrix} \,\, \mbox{,}
\end{equation}
where  $\mathbf{S} = \mathbf{D} - \mathbf{C} \mathbf{A}^{-1} \mathbf{B}$ is called the Schur complement of the matrix $\mathbf{M}$. 
\end{lemma}

In order to keep the analysis to follow tractable we will compute lower bounds by projecting $\gamma_{k}$ onto a $2$ dimensional subspace that is given as the span of vectors that are obtained from the kernel by partial derivation of order $0$ and $1$. **** Hopefully these two vectors are orthogonal .... ****


Another, easier way to generalize our results is via the data processing inequality discussed in Sec. \ref{sec_data_processing_inequality}. More precisely, consider an observation $\mathbf{y}$ following the SDCM with model matrices $\mathbf{C}^{(l)}$ being projection matrices onto orthogonal subspaces of $\mathbb{R}^{M}$. By applying an arbitrary but deterministic matrix $\mathbf{A}$ to obtain the modified observation $\tilde{\mathbf{y}}$  we have a modified estimation problem which is an instance of the SCM, i.e., 
\begin{equation}
\tilde{\mathbf{y}'}= \mathbf{s} + \mathbf{n}  \quad \mathbf{C}_{s} = \sum_{l=1}^{N} \tilde{\mathbf{C}}^{(l)} x_{k}
\end{equation}
where the PSD matrices $\tilde{\mathbf{C}}^{(l)}$ are of the form 
\begin{equation} 
\tilde{\mathbf{C}}^{(l)} = \mathbf{A} \mathbf{C}^{(l)} \mathbf{A}^{T} 
\end{equation} 
and the additive noise is distributed as $\mathbf{n} \sim \mathcal{N}(\mathbf{0}, \sigma^{2} \mathbf{A}\mathbf{A}^{T})$. 



\vspace*{10mm}
********Nicht notwendig**** \newline
Another ingredient for the analysis to follow is 
\begin{lemma}
Given an positive definite matrix $\mathbf{J}$ the diagonal elements of the inverse obey 
\begin{equation}
(\mathbf{J}^{-1})_{k,k} \geq \frac{1}{(\mathbf{J})_{k,k}} 
\end{equation} 
\end{lemma}
This can be proven by the Cauchy Schwarz inequality for the inner product $\langle \mathbf{y} , \mathbf{x} \rangle = \mathbf{y}^{T} \mathbf{J} \mathbf{x}$ and the specific vector $\mathbf{x} = \mathbf{e}_{k}$ and $\mathbf{y} = \mathbf{J}^{-1} \mathbf{e}_{k}$. 



\section{Barankin Bound and LMVU estimator for the SDCM}
\section{Constructing Estimators with a prescribed bias for the SDCM}
We now present a scheme for constructing estimators $\hat{x}_{k}$ for the SDCM that are required to yield a given bias. Similarly to Section \ref{sec_constr_est_SLM} our construction 
starts from an estimator that has already the prescribed bias. Then we add an additive component to this estimator whereby this additive component is required to have a mean function that 
vanishes for all $\mathbf{x} \in \mathcal{X}_{S,+}$

\section{Strict Sparsity is Necessary for lower minimum variance in the SDCM} 
Interpretation: sobald man eine (kleine) Kugel im parameterset hat wird die menge aller erlaubten estimators soweit reduziert dass keine verbesserung der varianz moeglich ist. 

\section{Comparison of the Bounds with Existing Estimators} 

% 






==> Chap_SSNM.tex <==
\chapter{The Sparse Linear Model}
\label{chap_SLM}
\section{Introduction}
%\section{Introduction}
%\label{sec_intro_chap_SLM}
%In this section we consider the problem of estimating an unknown nonrandom parameter vector $\mathbf{x} \in \mathbb{R}^{N}$ by using only an observed vector $\mathbf{y}$ 
%which is a linearly transformed noisy version of $\mathbf{x}$, i.e., we have the observation model 
%\begin{equation}
%\label{equ_obs_model_SLM}
%\mathbf{y} = \mathbf{H} \mathbf{x} + \mathbf{n}  
%\end{equation}
%where $\mathbf{H} \in \mathbb{R}^{M \times N}$ is a fixed and known matrix and $\mathbf{n} \sim \mathcal{N}(\mathbf{0}, \sigma^{2} \mathbf{I})$ denotes an additive white Gaussian measurement noise. The noise variance $\sigma^{2}$ is assumed to be positive and known. 
%The goal is to estimate the signal vector $\mathbf{x}$ using the observations $\mathbf{y}$ and the apriori knowledge that the signal vector is $S$-sparse, i.e., 
%\begin{equation}
%\mathbf{x} \in \mathcal{X}_{S} 
%\end{equation}
%where the sparsity degree $S < N$ is fixed and known. Typically we have that $S << N$. 
In this chapter we study the problem of estimating a nonrandom parameter vector $\mathbf{x} \!\in\! \mathbb{R}^{N}\!$
which is known to be strictly
$S$-sparse, i.e., at most $S$ of its entries are nonzero, where $1 \!\leq\! S \!\leq\! N$ (typically $S \!\ll\! N$). We thus 
\vspace{.5mm}
have
\be
\label{equ_SLM_parameter}
\mathbf{x} \!\in\!  \mathcal{X}_{S} \,, \quad\; \text{with} \;\; \mathcal{X}_{S} = \big\{\mathbf{x}' \rmv\!\in\! \mathbb{R}^{N} \big| \ist {\|\mathbf{x}' \|}_{0} \rmv\leq\rmv S \big\} \,.
\vspace{.5mm}
\ee 
%where ${\| \mathbf{x} \|}_{0}$ denotes the number of nonzero entries of $\mathbf{x}$. 
While the sparsity degree $S \in \mathbb{N}$ is assumed to be known, the set of positions of the nonzero entries of $\mathbf{x}$, i.e., the support $\supp(\mathbf{x})$, is unknown. 

The estimation of $\mathbf{x}$ is based on the observed vector $\mathbf{y} \!\in\! \mathbb{R}^{M}\!$ 
%% which is a linearly transformed and noisy version of $\mathbf{x}$: 
given 
\vspace{-.5mm}
by
\be
\label{equ_linear_observation_model}
\mathbf{y} \ist=\ist \mathbf{H} \mathbf{x} + \mathbf{n} \,,
\vspace{.2mm}
\ee
with a known 
%% deterministic 
system matrix $\mathbf{H} \!\in\! \mathbb{R}^{M \times N}\!$ and white Gaussian noise $\mathbf{n} \sim \mathcal{N}(\mathbf{0},  \sigma^{2} \mathbf{I})$ with 
a known positive noise variance $\sigma^{2} >0$. %, i.e., the entries of the noise vector $\mathbf{n} \in \mathbb{R}^{M}$ are i.i.d. zero-mean and unit-variance Gaussian random variables. 
The matrix $\mathbf{H}$ is arbitrary except that mainly it will we assumed to satisfy the standard 
\vspace{-.5mm}
requirement \cite{ZvikaCRB}%% BLIBLABLU
\begin{equation} 
\rm{spark}(\mathbf{H}) \rmv>\rmv   \, S \,, 
\label{equ_spark_cond}
\end{equation} 
where $\rm{spark}(\mathbf{H})$ denotes the minimum number of linearly dependent columns of $\mathbf{H}$ \cite{GreedisGood}.\footnote{For a full column rank matrix $\mathbf{H} \in \mathbb{R}^{M \times N}$, i.e., $\rank(\mathbf{H}) = N$, we define $\rm{spark}(\mathbf{H}) = N$.} 
Note that we also allow $M \!<\! N$ 
%% may be larger than, equal to, or smaller than $N$ 
(this case is relevant to compressed sensing methods as discussed in Section \ref{sec_slm_viewpoint_CS});
however, condition \eqref{equ_spark_cond} implies that $M \!\ge\! S$. 
The requirement \eqref{equ_spark_cond} is reasonable since otherwise we can find two different parameter vectors $\mathbf{x}_{1}, \mathbf{x}_{2} \in \mathcal{X}_{S}$ for 
which the pdf of the observation is identical, i.e., $f(\mathbf{y}; \mathbf{x}_{1}) = f(\mathbf{y}; \mathbf{x}_{2})$ for every $\mathbf{y}$, which means that it is completely impossible to distinguish 
between $\mathbf{x}_{1}$ and $\mathbf{x}_{2}$ only by looking on the observation $\mathbf{y}$. 

%(This assumption will be needed in Section \ref{sec:isometry} to relate the given sparse estimation problem to a nonsparse problem.)
More formally, by combining the observation model \eqref{equ_linear_observation_model} with the requirement \eqref{equ_SLM_parameter} 
we define the \emph{sparse linear model} (SLM) as the specific estimation problem denoted $\mathcal{E}_{\text{\tiny{SLM}}}$ and given as
\begin{equation} 
\label{equ_def_SLM_est_problem}
\mathcal{E}_{\text{\tiny{SLM}}} \triangleq \big( \mathcal{X}_{S}, f_{\text{\tiny{LGM}},\mathbf{H}}(\mathbf{y}; \mathbf{x}), \mathbf{g}(\mathbf{x}) = x_{k} \big), 
\end{equation} 
where $k \in [N]$ is an arbitrary but fixed index (the precise choice of $k$ will be made explicit whenever necessary) and with the statistical model 
\begin{equation} 
\label{equ_def_LGM_stat_model}
 f_{\text{\tiny{LGM}},\mathbf{H}}(\mathbf{y}; \mathbf{x}) = \frac{1}{(2 \pi \sigma^{2})^{M/2} } \exp \left(- \frac{1}{2 \sigma^{2}} \| \mathbf{y} - \mathbf{H} \mathbf{x} \|^{2}_{2} \right).
\end{equation}
By comparing \eqref{equ_def_LGM_stat_model} with the generic form \eqref{equ_def_pdf_exp_fam} of an exponential family, we obtain that the statistical modol of the SLM is nothing but an 
exponential family with sufficient statistic ${\bm \Phi}(\mathbf{y}) = \frac{1}{\sigma^{2}} \mathbf{H}^{T} \mathbf{y}$, cummulant function $ A^{( {\bm \Phi})}(\mathbf{x}) =   \frac{1}{2 \sigma^{2}} \mathbf{x}^{T} \mathbf{H}^{T} \mathbf{H} \mathbf{x}$ and weight $h^{( {\bm \Phi})}(\mathbf{y}) = \exp \left( - \frac{1}{2Ê\sigma^{2}} \mathbf{y}^{T} \mathbf{y} \right)$. % the statistical model of the SLM belongs to the exponential family . In particular, it is obtained by choosing as the sufficient statistic ... 

The SLM is very similar to a well known estimation problem, i.e., the \emph{linear gaussian model} (LGM) \cite{poorsspbook,kay,scharf91} which is given by 
\begin{equation}
\label{equ_def_LGM_est_problem}
\mathcal{E}_{\text{\tiny{LGM}}} \triangleq \big( \mathbb{R}^{N}, f_{\text{\tiny{LGM}},\mathbf{H}}(\mathbf{y}; \mathbf{x}), g(\mathbf{x}) = x_{k} \big).
\end{equation} 
Indeed, the only difference between the LGM $\mathcal{E}_{\text{\tiny{LGM}}}$ and the SLM $\mathcal{E}_{\text{\tiny{SLM}}}$ is the parameter set. 
The SLM is obtained from the LGM by reducing the parameter set from $\mathcal{X} = \mathbb{R}^{N}$ to 
the set of sparse vectors, i.e., $\mathcal{X} = \mathcal{X}_{S}$. If the sparsity degree $S$ is equal to the dimension of the observation, i.e., $S=N$, then the SLM coincides 
with the LGM. 

%The observation 
%\pagebreak %%%%%%%%%%
%model \eqref{equ_observation_model} together with \eqref{equ_SLM_parameter} will be referred to as the 
%\emph{sparse linear model} (SLM).

%Furthermore, note 
%that although the additive noise in the SLM is assumed white with unit variance, this is not a real restriction since the more general case of a Gaussian noise $\mathbf{n}$ in \eqref{equ_linear_observation_model} 
%with an arbitrary but known mean vector ${\bm \mu}$ and nonsingular covariance matrix $\mathbf{C}$ can be reduced to the SLM 
%by means of a noise whitening transformation. 
%Indeed, according to Section \ref{sec_invariance_mve} and Section \ref{sec_suff_stat_RKHS}, minimum variance estimation for an estimation problem with the observation model 
%\begin{equation} 
%\label{equ_obs_model_est_problem_1_noise_whitening}
%\mathbf{y} = \mathbf{H}' \mathbf{x}+ \mathbf{n}
%\end{equation} 
%where the noise $\mathbf{n}$ is distributed as $\mathbf{n} \sim \mathcal{N}({\bm \mu}, \mathbf{C})$, with a known mean vector ${\bm \mu}$ and known non-singular covariance matrix $\mathbf{C}$, is equivalent 
%to minimum variance estimation for the estimation problem whose observation is given by 
%\begin{equation}
%\label{equ_mod_obs_model_SLM}
%\mathbf{y}' \triangleq  \mathbf{C}'   (\mathbf{y} - {\bm \mu})=  \mathbf{C}' \mathbf{H}' \mathbf{x} + \mathbf{n}' ,
%\end{equation}
%where $\mathbf{C}' \triangleq \sqrt{\mathbf{C}^{-1}}$ and $\mathbf{n}' = \mathbf{C}' (\mathbf{n}-{\bm \mu})$. 
%Note that since $\mathbf{y}'$ is obtained by an invertible map from the observation $\mathbf{y}$ in \eqref{equ_obs_model_est_problem_1_noise_whitening} we trivially have that $\mathbf{y}'$ is a sufficient statistic for the estimation problem with observation model \eqref{equ_obs_model_est_problem_1_noise_whitening} (cf. Section \ref{sec_suff_stat_RKHS}). % and thus 
%%Since one can also verify easily that $\mathbf{n}' \sim \mathcal{N} (\mathbf{0}, \mathbf{I})$, we have that
%%in the context of minimum variance estimation, the problem of estimating $\mathbf{x}$ using the 
%%observation model \eqref{equ_obs_model_est_problem_1_noise_whitening} is equivalent to the problem of estimating $\mathbf{x}$ using the observation model \eqref{equ_mod_obs_model_SLM} which 
%However, since obviously $\mathbf{n}' \sim \mathcal{N}(\mathbf{0}, \mathbf{I})$ we have that \eqref{equ_mod_obs_model_SLM} is nothing but the observation model of the SLM with system matrix $\mathbf{H} =  \mathbf{C}'  \mathbf{H}'$. 
%To summarize: we can reduce any estimation problem with observation model 
%\eqref{equ_obs_model_est_problem_1_noise_whitening} to the SLM. 
%A precise formulation of this equivalence will be given by Theorem \ref{thm_arb_cov_matrix_red_SLM} in Section \ref{sec_RKHS_basic_facts_SLM}.
%We conclude this section by a statement allowing us, for fixed $S$, $M$ and $N$, to reduce an estimation problem with observation model \eqref{equ_obs_model_est_problem_1_noise_whitening} with 
%a system matrix $\mathbf{H} \in \mathbb{R}^{M \times N}$ and where the noise $\mathbf{n}$ can have an arbitrary mean ${\bm \mu} \in \mathbb{R}^{M}$ and (invertible) covariance matrix $\mathbf{C}$, 
%to the SLM with the same $S$, $M$ and $N$ but different system matrix $\mathbf{H}$, i.e., $\mathbf{H}' \neq \mathbf{H}$ in general. 
%To that end we denote the statistical model corresponding to \eqref{equ_obs_model_est_problem_1_noise_whitening} by $f_{\text{\tiny{LGM'}},\mathbf{H}', \mathbf{C}}(\mathbf{y}; \mathbf{x})$. 
%It is given explicitly by 
%\begin{equation}
%f_{\text{\tiny{LGM'}},\mathbf{H}',\mathbf{C}}(\mathbf{y}; \mathbf{x}) = \frac{1}{(2 \pi)^{M/2} \det( \mathbf{C} ) } \exp \left( - \frac{1}{2} (\mathbf{y} - \mathbf{H}' \mathbf{x} - {\bm \mu})^{T} \mathbf{C}^{-1} (\mathbf{y} - \mathbf{H}' \mathbf{x} - {\bm \mu}) \right). 
%\end{equation} 
%Then we can state
%\begin{theorem}
%\label{thm_arb_cov_matrix_red_SLM}
%Consider for specific choices for $S$, $M$, $N$, $\mathbf{H} \in \mathbb{R}^{M \times N}$ the two estimation problems $\mathcal{E}_{\text{\tiny{SLM}}}=\left( \mathcal{X}_{S}, f_{\text{\tiny{LGM'}},\mathbf{H}'}(\mathbf{y}; \mathbf{x}), g(\mathbf{x})=x_{k}Ê\right)$ 
%and $\mathcal{E}' = \left( \mathcal{X}_{S}, f_{\text{\tiny{LGM'}},\mathbf{H}',\mathbf{C}}(\mathbf{y}; \mathbf{x}), g(\mathbf{x})=x_{k}Ê\right)$ 
%with associated system matrices $\mathbf{H}$ and $\mathbf{H}'$. 
%If $\mathbf{H} = \sqrt{\mathbf{C}^{-1}}\mathbf{H}'$ we have for any prescribed bias $c(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}$ and parameter vector $\mathbf{x}_{0} \in \mathcal{X}_{S}$ that 
%the RKHS associated with the two specific minimum variance problems $\mathcal{M} = \left( \mathcal{E}_{\text{\tiny{SLM}}},c(\cdot), \mathbf{x}_{0} \right)$, $\mathcal{M}' = \left( \mathcal{E}',c(\cdot), \mathbf{x}_{0} \right)$ are identical, i.e., 
%\begin{equation}
%\mathcal{H}(\mathcal{M}) = \mathcal{H}(\mathcal{M}').
%\end{equation} 
%In particular we have that the minimum achievable variances are equal, i.e., 
%\begin{equation}
%L_{\mathcal{M}} = L_{\mathcal{M}'}. 
%\end{equation} 
%\end{theorem}
%\begin{proof} 
%The statistical model $f_{\text{\tiny{LGM'}},\mathbf{H}'}(\mathbf{y}; \mathbf{x})$ corresponds to the observation model $\mathbf{y} = \mathbf{H}' \mathbf{x} + \mathbf{n}$ where $\mathbf{n} \sim \mathcal{N}({\bm \mu}, \mathbf{C})$. 
%A sufficient statistic for $\mathcal{E}' = \left( \mathcal{X}_{S}, f_{\text{\tiny{LGM'}},\mathbf{H}}(\mathbf{y}; \mathbf{x}), g(\mathbf{x})=x_{k}Ê\right)$ is given by 
%$\mathbf{y}' = \sqrt{\mathbf{C}^{-1}} (\mathbf{y}- {\bm \mu}) = \sqrt{\mathbf{C}^{-1}}\mathbf{H}' \mathbf{x} +  \sqrt{\mathbf{C}^{-1}} (\mathbf{y}- {\bm \mu})$.
%We already mentioned in Section \ref{sec_intro_chap_SLM} that the pdf of $\mathbf{y}'$ (parametrized by $\mathbf{x}$) so defined is nothing but the statistical model of the SLM with $\mathbf{H} =\sqrt{\mathbf{C}^{-1}}\mathbf{H}'$
%, i.e., $f_{\text{\tiny{LGM}},\mathbf{H}}(\mathbf{y}'; \mathbf{x})$. From this the statement follows from Theorem \ref{thm_suff_stat_RKHS_invar}. 
%\end{proof}

The SLM is relevant e.g. for sparse channel estimation \cite{Carbonelli06} where the sparse parameter vector $\mathbf{x}$ represents the taps of a linear time invariant (LTI) channel and the system matrix $\mathbf{H}$ represents the training signal. Generally, the SLM can be used for any type of sparse deconvolution \cite{MallatBook} like in optical coherence tomography (OCT) \cite{KailOCTIcassp09}, where the sparse vector $\mathbf{x}$ models the layer structure of the human eye and the matrix 
$\mathbf{H}$ represents the properties of the measurement device. 

An important special case of the SLM is given by $\mathbf{H} \!=\! \mathbf{I}$ (so that $M \!=\! N$), 
\vspace{-1mm}
i.e., 
\be
\label{equ_observation_model_SSNM}
\mathbf{y} \ist=\ist \mathbf{x} + \mathbf{n} \,,
\ee
where again $\mathbf{x} \!\in\!  \mathcal{X}_{S}$ and $\mathbf{n} \sim \mathbb{R}^{N}$ denotes additive white Gaussian noise (AWGN), i.e., $\mathbf{n} \sim \mathcal{N}(\mathbf{0}, \sigma^{2}  \mathbf{I})$ with known variance $\sigma^{2} > 0$. This will be referred to as the \emph{sparse signal in noise model} (SSNM). 
Formally, the SSNM is defined as the estimation problem
\begin{equation} 
\label{equ_def_SSNM_est_problem}
\mathcal{E}_{\text{SSNM}} \triangleq \big( \mathcal{X}_{S}, f_{\text{\tiny{LGM}},\mathbf{I}}(\mathbf{y}; \mathbf{x}), \mathbf{g}(\mathbf{x}) = x_{k} \big), 
\end{equation} 
i.e., with the statistical model \eqref{equ_def_LGM_stat_model} for the specific choice $\mathbf{H} = \mathbf{I}$ for the system matrix. 
The SSNM can be used, e.g., for channel estimation \cite{Carbonelli06} when %%% AJ
%% whenever 
%% it is assumed that 
the 
%% time-invariant 
channel consists only of 
%% very 
few significant taps and an orthogonal training signal is used \cite{OptimalTrainingDong}. 
Another potential application for the SSNM is image denoising using an orthonormal wavelet basis \cite{Donoho94idealspatial}. 
Note that due to Theorem \ref{thm_data_proc_inequ_classical_est} we have that any bound on the minimum achievable variance of 
a minimum variance problem $\mathcal{M}_{\text{\tiny{SSNM}}}=\left( \mathcal{E}_{\text{\tiny{SSNM}}}, c(\cdot), \mathbf{x}_{0} \right)$ entails a 
lower bound on the minimum achievable variance for a minimum variance problem for any estimation problem with parameter set $\mathcal{X}_{S}$ and 
observation model 
\begin{equation}
\mathbf{y} = \mathbf{H}(\mathbf{x} + \mathbf{n}) 
\end{equation}
where $\mathbf{H} \in \mathbb{R}^{M \times N}$ is an arbitrary but fixed system matrix and $\mathbf{n} \in \mathbb{R}^{N}$ denotes AWGN, 
i.e., $\mathbf{n} \sim \mathcal{N}(\mathbf{0}, \sigma^{2} \mathbf{I})$ with known positive variance $\sigma^{2} > 0$. 
 
%We note that parts of this work were previously presented in \cite{AlexZvikaICASSP}. 

The SLM has been considered in \cite{JustRelax} where the authors analyze the performance of specific estimation schemes that are based on convex optimization problems. 
In a minimax estimation context the SLM has been studied in \cite{RaskuttiMinmaxSLM,VerzelenMinmaxSLM} where the authors derive bounds on the minimax risk (cf. Section \ref{sec_minimax_est}) and also 
discuss estimators that come close to these bounds. An asymptotic analysis of minimax estimation for the SSNM is given in the seminal work \cite{DonohoJohnstone94,Donoho94idealspatial}.
In our context, i.e., minimum variance estimation, lower bounds on the minimum achievable estimation variance for the SLM have been studied recently: 
In particular, the CRB for the SLM was derived and analyzed in \cite{ZvikaCRB,ZvikaSSP}.
In \cite{AlexZvikaICASSP} lower and upper bounds on the minimum achievable variance of unbiased estimators were derived for the SSNM by using techniques that differ from the RKHS approach that will 
be used in this thesis. A remarkable property of the lower bounds presented in \cite{ZvikaCRB} and \cite{AlexZvikaICASSP} is the fact that they 
exhibit a discontinuity when passing from the case ${\| \mathbf{x} \|}_{0} \!=\! S$ to the case ${\| \mathbf{x} \|}_{0} \!<\! S$. 
%More precisely these lower bounds are upper semicontinuous, whereas we have 
%\begin{theorem}
%Consider the class of minimum variance problems $\mathcal{M}(\mathbf{x}_{0}) \triangleq \left(\mathcal{E}_{\text{\tiny{SLM}}},c(\cdot), \mathbf{x}_{0} \right)$ paramtrized by $\mathbf{x}_{0}$. We then 
%have that the minimum achievable variance $L_{\mathcal{M}(\mathbf{x}_{0})}$ viewed as a function of $\mathbf{x}_{0}$ is lower semicontionous.   
%\end{theorem} 
%\begin{proof} 
%First note that the variance of any estimator for the SLM is a continuos function of the parameter $\mathbf{x}$. 
%\end{proof} 
%Thus, there necessarily is some gap between the lower bounds in \cite{ZvikaCRB} and \cite{AlexZvikaICASSP} and the minimum achievable variance, i.e., these lower bounds cannot be tight. 


In this chapter, we use the mathematical framework of RKHS %\cite{aronszajn1950,Parzen59,Duttweiler73b} 
to derive novel lower bounds on the variance of estimators for the SLM. 
%It is worth noting that some established lower 
%% variance 
%bounds like the CRB and the Hammersley-Chapman-Robbins bound \cite{GormanHero} have pleasing geometric interpretations 
%in the RKHS framework. 
%The RKHS framework allows pleasing geometric interpretations of existing bounds, including the CRB, the Hammersley-Chapman-Robbins bound \cite{GormanHero}, 
%and the Barankin bound \cite{Barankin49}.
The bounds which will be derived here hold for estimators with a given differentiable bias function.
%%  which can be specified arbitrarily. 
For the special case of the SSNM, we obtain a lower bound for unbiased estimators 
%% (i.e., estimators whose bias is identically zero) 
which is tighter
%%  (higher) 
than the bounds in \cite{ZvikaCRB,ZvikaSSP,AlexZvikaICASSP} and, moreover, is a continuous function of $\mathbf{x}$. As we will show, RKHS theory relates the 
%% variance 
lower bound for the SLM to that obtained for a 
%% simpler 
specific LGM. The RKHS framework has been previously applied to estimation \cite{Parzen59,Duttweiler73b} but, 
to the best of our knowledge, not to the SLM.
%% it has not so far been used for the estimation of sparse vectors. 
%% To the best of our knowledge, RKHS theory has not been previously applied to the estimation of sparse vectors !!!!!.

This chapter is organized as follows:
In Section \ref{sec_RKHS_SLM}, we introduce and discuss the RKHS associated to minimum variance problems that arise from the SLM.
%Relevant elements of RKHS theory are summarized in Section \ref{sec_rkhs}.
In Section \ref{sec_RKHS_Lower_Bounds_SLM}, we use RKHS theory first to reinterpret existing lower bounds from the geometrical RKHS perspective and then to 
derive novel lower bounds on the variance of estimators for the SLM which have a prescribed bias and mean function. 
%Section \ref{sec_constr_est_SLM} presents a RKHS based method for constructing estimators with a given bias and mean function. 
The important special case of the SLM given by the SSNM is discussed in Section \ref{sec_SSNM}, where we derive a closed form 
for the minimum achievable variance, i.e., the Barankin bound and corresponding LMV estimator. 
A discussion on the necessity for strict sparsity requirements is presented in Section \ref{sec_strict_sparstiy_SLM}. The SLM viewpoint on 
the CS recovery problem is presented in Section \ref{sec_slm_viewpoint_CS}. 
%After analyzing the SLM in the context of CS recovery in Section \ref{sec_SLM_CS} we 
Finally, we compare the theoretical bounds with the actual variance behavior of some popular estimation schemes in Section \ref{sec_numerical_SLM}.

The key results of this chapter have been presented in part already in \cite{AlexZvikaICASSP,RKHSAsilomar2010,AlexZvikaJournal,RKHSISIT2011}. 

%Section \ref{sec_lower_bounds_SSNM} considers the special case of unbiased estimation within the SSNM. 
%Section \ref{sec_numerical} presents a numerical comparison of the new bound with the variance of two established estimation schemes.


\section{RKHS Associated with the SLM}
\label{sec_RKHS_SLM}

%The SLM refers to the specific estimation problem $\mathcal{E}_{\text{\tiny{SLM}}}$ and 
We will denote any minimum variance problem that 
is obtained from $\mathcal{E}_{\text{\tiny{SLM}}}$ (cf. \eqref{equ_def_SLM_est_problem}) by additionally fixing a prescribed bias function $c(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}$ 
and parameter vector $\mathbf{x}_{0} \in \mathcal{X}_{S}$, by 
\begin{equation}
\label{equ_def_min_var_problem_SLM}
\mathcal{M}_{\text{\tiny{SLM}}} \triangleq \left( \mathcal{E}_{\text{\tiny{SLM}}}, c(\cdot), \mathbf{x}_{0} \right).
\end{equation} 
It should be clear from context which bias function $c(\cdot)$ and fixed parameter vector $\mathbf{x}_{0}$ is used within the minimum variance problem $\mathcal{M}_{\text{\tiny{SLM}}}$. 
Note that the restriction to the specific parameter function $g(\mathbf{x}) = x_{k}$ in the SLM \eqref{equ_def_SLM_est_problem} is no real restriction, 
since we do not constrain the prescribed bias $c(\cdot)$ used for the minimum variance problem $\mathcal{M}_{\text{\tiny{SLM}}}$ 
and according to Theorem \ref{thm_equ_bias_param_function} it is no loss of generality if one fixes either the prescribed bias or the parameter function of a minimum variance problem, but not both.

The estimation problem $\mathcal{E}_{\text{\tiny{SLM}}}$ satisfies the requirements of Postulate \ref{assumption_RKHS_minvarproblem}, 
since it can be easily verified that $\mathsf{E}_{\mathbf{x}_{0}} \left \{ \frac{ f_{\text{\tiny{LGM}},\mathbf{H}}(\mathbf{y}; \mathbf{x}_{1}) }{  f_{\text{\tiny{LGM}},\mathbf{H}}(\mathbf{y}; \mathbf{x}_{0})}   \frac{ f_{\text{\tiny{LGM}},\mathbf{H}}(\mathbf{y}; \mathbf{x}_{1}) }{  f_{\text{\tiny{LGM}},\mathbf{H}}(\mathbf{y}; \mathbf{x}_{0})} \right \}  < \infty$ for any $\mathbf{x}_{1}, \mathbf{x}_{2} \inÊ\mathcal{X}_{S}$.
Therefore, according to Section \ref{sec_def_RKHS_MVP} we can associate with the minimum variance problem $\mathcal{M}_{\text{\tiny{SLM}}}$ 
a RKHS $\mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}})$ whose kernel $R_{\mathcal{M}_{\text{\tiny{SLM}}}}(\cdot,\cdot): \mathcal{X}_{S} \times \mathcal{X}_{S} \rightarrow \mathbb{R}$ is given 
as (cf. \eqref{equ_def_kernel_M}): 
\begin{align}
\label{equ_kernel_SLM}
R_{\mathcal{M}_{\text{\tiny{SLM}}}}(\mathbf{x}_{1}, \mathbf{x}_{2})  & =  \mathsf{E}_{\mathbf{x}_{0}} \{ \rho_{\mathcal{M}_{\text{\tiny{SLM}}}}(\mathbf{y},\mathbf{x}_{1}) \rho_{\mathcal{M}_{\text{\tiny{SLM}}}}(\mathbf{y},\mathbf{x}_{2}) \}  
=  \mathsf{E}_{\mathbf{x}_{0}} \left \{ \frac{ f_{\text{\tiny{LGM}},\mathbf{H}}(\mathbf{y}; \mathbf{x}_{1}) }{  f_{\text{\tiny{LGM}},\mathbf{H}}(\mathbf{y}; \mathbf{x}_{0})}   \frac{ f_{\text{\tiny{LGM}},\mathbf{H}}(\mathbf{y}; \mathbf{x}_{2}) }{  f_{\text{\tiny{LGM}},\mathbf{H}}(\mathbf{y}; \mathbf{x}_{0})} \right \} Ê\nonumberÊ\\
&  \hspace*{-20mm} = \int_{\mathbf{y}} \frac{ f_{\text{\tiny{LGM}},\mathbf{H}}(\mathbf{y}; \mathbf{x}_{1})  f_{\text{\tiny{LGM}},\mathbf{H}}(\mathbf{y}; \mathbf{x}_{2}) }{  f_{\text{\tiny{LGM}},\mathbf{H}}(\mathbf{y}; \mathbf{x}_{0})}d \mathbf{y}  \nonumberÊ\\
&  \hspace*{-20mm} = \int_{\mathbf{y}} \frac{1}{(2 \pi \sigma^{2})^{M/2} }  
\frac{ \exp  \left(-\frac{1}{2\sigma^{2}} \| \mathbf{y} - \mathbf{H} \mathbf{x}_{1} \|^{2}_{2} \right)  \exp \left(-\frac{1}{2 \sigma^{2}}  \| \mathbf{y} - \mathbf{H} \mathbf{x}_{2} \|^{2}_{2} \right) }
{   \exp \left( -\frac{1}{2 \sigma^{2}} \| \mathbf{y} - \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} \right)}d \mathbf{y}  \nonumber \\
& \hspace*{-20mm} = \int_{\mathbf{y}} \frac{1}{(2 \pi \sigma^{2} )^{M/2} }   \exp \bigg( -\frac{1}{2 \sigma^{2}} \left( \| \mathbf{y} \|^{2}_{2}- 2\mathbf{y}^{T} \mathbf{H} (\mathbf{x}_{1}+\mathbf{x}_{2}-\mathbf{x}_{0}) +  \|  \mathbf{H} \mathbf{x}_{1} \|^{2}_{2} + \|  \mathbf{H} \mathbf{x}_{2} \|^{2}_{2} -  \| \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} \right) \bigg) d \mathbf{y} \nonumber \\
& \hspace*{-20mm} = \int_{\mathbf{y}} \frac{1}{(2 \pi \sigma^{2} )^{M/2} }  \times \nonumber \\ 
&  \hspace*{-20mm}  \exp \bigg(-\frac{1}{2\sigma^{2}}  \left( \| \mathbf{y} - \mathbf{H}(\mathbf{x}_{1}+\mathbf{x}_{2}-\mathbf{x}_{0})  \|^{2} + 2 \mathbf{x}_{0}^{T}\mathbf{H}^{T} \mathbf{H} (\mathbf{x}_{1} + \mathbf{x}_{2}) - 2 \mathbf{x}_{1}^{T}\mathbf{H}^{T} \mathbf{H} \mathbf{x}_{2} - 2 \mathbf{x}_{0}^{T} \mathbf{H}^{T} \mathbf{H} \mathbf{x}_{0} \right) \bigg) d \mathbf{y} \nonumber \\ 
& \hspace*{-20mm}  =  \exp   \left( \frac{1}{\sigma^{2}} (\mathbf{x}_{1} - \mathbf{x}_{0})^{T}\mathbf{H}^{T} \mathbf{H} (\mathbf{x}_{2} - \mathbf{x}_{0}) \right). 
\end{align} 
Obviously, the kernel $R_{\mathcal{M}_{\text{\tiny{SLM}}}}(\cdot,\cdot)$ is differentiable in the sense of Definition \ref{def_differentiable_kernel} 
up to any order $m \in \mathbb{N}$ and therefore Theorem \ref{thm_der_repr_prop} applies 
to the RKHS $\mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}})$ (note that this RKHS consists of functions $f(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}$). 

%\paragraph{RKHS Properties $S=N$}
Let us now consider the SLM for the specific case $S=N$ for which the SLM coincides with the LGM. 
We will denote by 
\begin{equation} 
\label{equ_def_min_var_problem_LGM}
\mathcal{M}_{\text{\tiny{LGM}}} \triangleq \left( \mathcal{E}_{\text{\tiny{LGM}}}, \tilde{c}(\cdot), \mathbf{x}_{0} \right)
\end{equation} 
any minimum variance problem arising from the LGM $\mathcal{E}_{LGM}$ by fixing a prescribed bias function $\tilde{c}(\cdot): \mathbb{R}^{N} \rightarrow \mathbb{R}$ 
and parameter vector $\mathbf{x}_{0} \in \mathcal{X}_{S}$.\footnote{Note that we require $\mathbf{x}_{0} \in \mathcal{X}_{S}$ even if the parameter set of the LGM is $\mathbb{R}^{N} \supseteq \mathcal{X}_{S}$.}
The corresponding RKHS will be denoted by $\mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}})$, i.e., $\mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}})$ is the 
RKHS associated to the kernel $R_{\text{\tiny{LGM}}}(\cdot,\cdot): \mathbb{R}^{N} \times \mathbb{R}^{N} \rightarrow \mathbb{R}$: 
\begin{equation} 
R_{\mathcal{M}_{\text{\tiny{LGM}}}}(\mathbf{x}_{1}, \mathbf{x}_{2}) =  \exp   \left(\frac{1}{\sigma^{2}}  (\mathbf{x}_{1} - \mathbf{x}_{0})^{T} \mathbf{H}^{T} \mathbf{H} (\mathbf{x}_{2} - \mathbf{x}_{0}) \right). 
\end{equation} 

As can be verified easily, the restriction $\mathcal{M}_{\text{\tiny{LGM}}}\big|_{\mathcal{X}_{S}}$ of the minimum variance problem $\mathcal{M}_{\text{\tiny{LGM}}}$ given by \eqref{equ_def_min_var_problem_LGM} coincides with the minimum variance problem $\mathcal{M}_{\text{\tiny{SLM}}}$ given by \eqref{equ_def_min_var_problem_SLM} with prescribed bias $c(\cdot) = \tilde{c}(\cdot) \big|_{\mathcal{X}_{S}}$. 
%We have the following relation between the RKHS $\mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}})$ associated with the minimum variance problem $\mathcal{M}_{\text{\tiny{SLM}}}$
%with specific choices for $S$, $M$, $N$, $\mathbf{H}$, $c(\cdot)$ and $\mathbf{x}_{0} \in \mathcal{X}_{S}$ and the RKHS $\mathcal{M}_{\text{\tiny{LGM}}}$ associated with the minimum variance problem $\mathcal{M}_{\text{\tiny{LGM}}}$ 
%that uses the same $M$, $N$, $\mathbf{H}$, prescribed bias $c(\cdot)$ and $\mathbf{x}_{0}$: 
\begin{theorem}
\label{thm_relation_RKHS_LGM_SLM}
Consider the minimum variance problem $\mathcal{M}_{\text{\tiny{LGM}}}= \left( \mathcal{E}_{\text{\tiny{SLM}}},\tilde{c}(\cdot),\mathbf{x}_{0} \right)$ with an arbitrary but fixed choice for 
$\sigma$, $M$, $N$, $\mathbf{H}$, prescribed bias $\tilde{c}(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}$ and parameter vector $\mathbf{x}_{0} \in \mathcal{X}_{S}$. We then have that 
for any sparsity degree $S \in [N]$, the RKHS $\mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}})$ associated with $\mathcal{M}_{\text{\tiny{SLM}}}=\mathcal{M}_{\text{\tiny{LGM}}}\big|_{\mathcal{X}_{S}}$
consists of the restrictions of any function $f(\cdot): \mathbb{R}^{N} \rightarrow \mathbb{R}$ belonging to the RKHS $\mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}})$ to the subdomain $\mathcal{X}_{S} \subseteq \mathbb{R}^{N}$, i.e., 
\begin{equation}
 \mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}}) = \{ f(\cdot) \big|_{\mathcal{X}_{S}} \,\, \big| \,\,  f(\cdot) \in \mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}}) \}. 
\end{equation} 
Moreover, the norm of any element $f(\cdot) \in \mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}})$ is given by 
\begin{align} 
\| f(\cdot) \|_{\mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}})}  & = \min_{ g(\cdot) \in \mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}})} \| g(\cdot) \|_{\mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}})}  \\Ê
 \mbox{s.t.} & \quad f(\mathbf{x}) = g(\mathbf{x}) \quad \forall \mathbf{x} \in \mathcal{X}_{S}. \nonumber 
\end{align}
\end{theorem} 
\begin{proof}
This result is obtained from the application of Theorem \ref{thm_reducing_domain_RKHS} to the specific RKHS $\mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}})$ and $\mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}})$
since the associated kernels obviously satisfy $R_{\mathcal{M}_{\text{\tiny{SLM}}}}(\cdot,\cdot) =R_{\mathcal{M}_{\text{\tiny{LGM}}}}(\cdot,\cdot) \big|_{\mathcal{X}_{S} \times \mathcal{X}_{S}}$. 
\end{proof}


The RKHS $\mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}})$ associated with the minimum variance problem $\mathcal{M}_{\text{\tiny{LGM}}}$ has already been analyzed in \cite{Duttweiler73b}. 
However, we will now present an alternative characterization of the RKHS $\mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}})$ that is based on a congruence with 
a specific RKHS that has some pleasing properties. In particular we have 
\begin{theorem}
\label{thm_isometry_LGM}
Consider the RKHS $\mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}})$ associated with  $\mathcal{M}_{\text{\tiny{LGM}}} \triangleq \left( \mathcal{E}_{\text{\tiny{LGM}}}, \tilde{c}(\cdot), \mathbf{x}_{0} \right)$ 
with an arbitrary system matrix $\mathbf{H} \in \mathbb{R}^{M \times N}$, not necessarily satisfying \eqref{equ_spark_cond}
and denote its thin SVD by $\mathbf{H} = \mathbf{U} \mathbf{\Sigma} \mathbf{V}^{T}$. 
Then we have that any function $f(\cdot) \in \mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}})$ is constant w.r.t. to translations by vectors $\mathbf{x}' \in \mathbb{R}^{N}$ 
that belong to the null-space of $\mathbf{H}$, i.e., 
\begin{equation} 
\label{equ_invar_prop_LGM_kernel_H}
f(\mathbf{x}) = f(\mathbf{x} + \mathbf{x}')
\end{equation}
for any $\mathbf{x}' \in \mathcal{N}(\mathbf{H})$, $\mathbf{x}\in \mathbb{R}^{N}$.  
%for any $\mathbf{x}' \in \Ker(\mathbf{H})$.
Furthermore, the RKHS $\mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}})$ is isometric to the RKHS $\mathcal{H}(R_{g}^{(D)})$ for $D=\rank( \mathbf{H} )$, 
where the RKHS $\mathcal{H}(R_{g}^{(D)})$ is defined via the kernel $R_{g}^{(D)}(\cdot,\cdot): \mathbb{R}^{D} \times \mathbb{R}^{D} \rightarrow \mathbb{R}$: 
\begin{equation}
\label{equ_def_kernel_R_g}
R_{g}^{(D)}(\mathbf{x}_{1}, \mathbf{x}_{2}) \triangleq \exp \left( \mathbf{x}_{1}^{T} \mathbf{x}_{2} \right).
\end{equation}
The specific mapping $\mathsf{K}_{g}[\cdot]: \mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}}) \rightarrow \mathcal{H}(R_{g}^{(D)})$ given by 
\begin{equation} 
\label{equ_def_isometry_LGM}
f(\cdot) \mapsto \widetilde{f}(\cdot) =  \mathsf{K}_{g}[f(\cdot)] :  \widetilde{f}(\mathbf{x}') 
= f(\sigma \widetilde{\mathbf{H}} \mathbf{x}') \exp\left( - \frac{1}{2 \sigma^{2}} \| \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} + \frac{1}{\sigma} (\mathbf{x}')^{T}  \widetilde{\mathbf{H}}^{\dagger}\mathbf{x}_{0}\right),
\end{equation} 
where $\widetilde{\mathbf{H}} \triangleq \mathbf{V} \mathbf{ \Sigma}^{-1}$, 
%where $\mathbf{B} \triangleq \mathbf{H}^{T}\mathbf{H}$, 
is a congruence from $\mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}})$ to $\mathcal{H}(R_{g}^{(D)})$. 
\end{theorem}
\begin{proof}
Consider the specific function $f_{\mathbf{x}_{1}}(\cdot) = R_{\mathcal{M}_{\text{\tiny{LGM}}}}(\cdot, \mathbf{x}_{1} )$ where $\mathbf{x}_{1} \in \mathbb{R}^{N}$ is arbitrary but fixed.
We then have for any $\mathbf{x}' \in \mathcal{N}(\mathbf{H})$ and $\mathbf{x} \inÊ\mathbb{R}^{N}$ that
\begin{align}
f_{\mathbf{x}_{1}}(\mathbf{x} + \mathbf{x}') & = \exp   \left( \frac{1}{\sigma^{2}}  (\mathbf{x} + \mathbf{x}' - \mathbf{x}_{0})^{T}\mathbf{H}^{T} \mathbf{H} (\mathbf{x}_{1} - \mathbf{x}_{0}) \right) \nonumber \\Ê
& = \exp\left( \frac{1}{\sigma^{2}} (\mathbf{x} - \mathbf{x}_{0})^{T}\mathbf{H}^{T} \mathbf{H} (\mathbf{x}_{2} - \mathbf{x}_{0}) \right) = f_{\mathbf{x}_{1}}(\mathbf{x}).
\end{align} 
From this it follows straightforwardly that any function $f(\cdot) \in \linspan \left \{ R_{\mathcal{M}_{\text{\tiny{LGM}}}}(\cdot, \mathbf{x} ) \right \}_{\mathbf{x} \in \mathbb{R}^{N}}$ satisfies \eqref{equ_invar_prop_LGM_kernel_H}. 
%Due to Theorem \ref{thm_constr_RKHS_closure_linear_span} any $f(\cdot) \in \mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}})$ can 
%be approximated arbitrarily well by an element of the set $\linspan \left \{ R_{\mathcal{M}_{\text{\tiny{LGM}}}}(\cdot, \mathbf{x} ) \right \}_{\mathbf{x} \in \mathbb{R}^{N}}$. 
%Thus, for any $\varepsilon >0$ we can find a $f'(\cdot) \in \linspan \left \{ R_{\mathcal{M}_{\text{\tiny{LGM}}}}(\cdot, \mathbf{x} ) \right \}_{\mathbf{x} \in \mathbb{R}^{N}}$ such that $\| f(\cdot) - f'(\cdot) \|_{\mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}})} \leq \varepsilon$ which implies via Theorem \ref{thm_cauchy_schwarz} and the reproducing property (cf. \eqref{equ_reproduction_property}) that we can make the difference $f(\mathbf{x}) - f'(\mathbf{x})$ arbitrarily small at any point $\mathbf{x} \in \mathbb{R}^{N}$. 
Consider a general $f(\cdot) \in  \mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}})$ and fix an arbitrary $\mathbf{x} \in \mathbb{R}^{N}$ and $\mathbf{x}' \in \mathcal{N}(\mathbf{H})$. 
We then have for any $f'(\cdot) \in \linspan \left \{ R_{\mathcal{M}_{\text{\tiny{LGM}}}}(\cdot, \mathbf{x} ) \right \}_{\mathbf{x} \in \mathbb{R}^{N}}$ it holds that 
\begin{align} 
\label{equ_inver_prop_LGM_arb_f_kernel_H}
f(\mathbf{x}+ \mathbf{x}') - f(\mathbf{x}) & = (f(\mathbf{x}+ \mathbf{x}')-f'(\mathbf{x}+\mathbf{x}')) - (f(\mathbf{x})-f'(\mathbf{x}))+ f'(\mathbf{x}+\mathbf{x}')-f'(\mathbf{x}) \nonumber \\Ê
 &\stackrel{(a)}{=} (f(\mathbf{x}+ \mathbf{x}')-f'(\mathbf{x}+\mathbf{x}')) - (f(\mathbf{x})-f'(\mathbf{x})) 
\end{align} 
where $(a)$ follows from the fact that $f'(\cdot)$ satisfies \eqref{equ_invar_prop_LGM_kernel_H}. 
Since we can make the last expression of \eqref{equ_inver_prop_LGM_arb_f_kernel_H} arbitrarily small by Theorem \ref{thm_norm_impl_point_convergence}, 
we have that $f(\mathbf{x}+ \mathbf{x}')= f(\mathbf{x})$ which concludes the proof of \eqref{equ_invar_prop_LGM_kernel_H}. 

For the following we note that based on the thin SVD $\mathbf{H} = \mathbf{U} \mathbf{\Sigma} \mathbf{V}^{T}$ of $\mathbf{H}$ we have the relations
\begin{equation}
\label{equ_proof_isometr_R_g_quadr_form} 
\mathbf{H}^{T}\mathbf{H} = \mathbf{V} \mathbf{\Sigma}^{2} \mathbf{V}^{T} =  ( \widetilde{\mathbf{H}}^{\dagger})^{T}\widetilde{\mathbf{H}}^{\dagger}
\end{equation} 
and
\begin{equation}
\label{equ_proof_isometr_R_g_pseudo_inver_tilde_H} 
\widetilde{\mathbf{H}}^{T}\mathbf{H}^{T}\mathbf{H} =\mathbf{\Sigma}^{-1} \mathbf{V}^{T}  \mathbf{V} \mathbf{\Sigma}^{2} \mathbf{V}^{T}  =\mathbf{\Sigma} \mathbf{V}^{T} =\widetilde{\mathbf{H}}^{\dagger}.
\end{equation} 
%Note that for the LGM we have due to $S=N$ and \eqref{equ_spark_cond} that the matrix $\mathbf{B} = \mathbf{H}^{T} \mathbf{H}$ is positive definite. 
%Therefore, we can compute $(\mathbf{H}^{T}\mathbf{H})^{\dagger/2}$, e.g. via an eigenvalue decomposition of $\mathbf{B}$. 
Consider the two sets of functions given by
\begin{equation} 
\label{equ_proof_isometr_R_g_set_A_in_R_LGM}
\mathcal{A} \triangleq \left \{ f_{\mathbf{x}}(\cdot) \triangleq  R_{\mathcal{M}_{\text{\tiny{LGM}}}}(\cdot, \sigma \mathbf{x} ) \right \}_{\mathbf{x} \in \mathbb{R}^{N}}
\end{equation} 
and 
\begin{equation} 
\mathcal{B} \triangleq \left \{ g_{\mathbf{x}} (\cdot) \triangleq \exp\left( \frac{1}{2 \sigma^{2}} \| \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} -  \frac{1}{\sigma}\mathbf{x}^{T} (\mathbf{H}^{T} \mathbf{H}) \mathbf{x}_{0} \right)R_{g}^{(D)}(\cdot, \widetilde{\mathbf{H}}^{\dagger} \mathbf{x}) \right \}_{\mathbf{x} \in \mathbb{R}^{N}}.
\end{equation} 
By Theorem \ref{thm_constr_RKHS_closure_linear_span} and the obvious (since $\sigma \mathbb{R}^{N} = \mathbb{R}^{N}$ and $\widetilde{\mathbf{H}}^{\dagger} \mathbb{R}^{N} = \mathbb{R}^{D}$) facts that 
$\linspan \{\mathcal{A} \}=  \linspan  \left \{ R_{\mathcal{M}_{\text{\tiny{LGM}}}}(\cdot, \mathbf{x} ) \right \}_{\mathbf{x} \in \mathbb{R}^{N}}$ and $\linspan \{\mathcal{B} \}=  \linspan  \{ R_{g}^{(D)}(\cdot, \mathbf{x} ) \}_{\mathbf{x} \in \mathbb{R}^{D}}$,
%\end{equation} 
it follows that $\mathcal{A}$ and $\mathcal{B}$ span the two RKHS $\mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}})$ and $\mathcal{H}(R_{g}^{(D)})$ respectively. 
Therefore, for any two vectors $\mathbf{x}_{1}, \mathbf{x}_{2} \in \mathbb{R}^{N}$:
\begin{align}
 \langle f_{\mathbf{x}_{1}}(\cdot) ,  f_{\mathbf{x}_{2}}(\cdot) \rangle_{\mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}})} & =
 \langle R_{\mathcal{M}_{\text{\tiny{LGM}}}}(\cdot,\sigma \mathbf{x}_{1}), R_{\mathcal{M}_{\text{\tiny{LGM}}}}(\cdot,Ê\sigma \mathbf{x}_{2}) \rangle_{\mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}})} \nonumber  \\
& \hspace*{-40mm} = \exp   \left( \frac{1}{\sigma^{2}} ( \sigma \mathbf{x}_{1} - \mathbf{x}_{0})^{T} \mathbf{H}^{T} \mathbf{H} (\sigma \mathbf{x}_{2} - \mathbf{x}_{0}) \right) \nonumber \\Ê
&\hspace*{-40mm} = \exp\left( \frac{1}{2 \sigma^{2}} \| \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} -  \frac{1}{\sigma} \mathbf{x}_{1}^{T} (\mathbf{H}^{T} \mathbf{H}) \mathbf{x}_{0} \right)  \exp   \left(  \mathbf{x}_{1}^{T} (\mathbf{H}^{T} \mathbf{H}) \mathbf{x}_{2}  \right)\exp\left( \frac{1}{2 \sigma^{2}} \| \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} - \frac{1}{\sigma} \mathbf{x}_{2}^{T} (\mathbf{H}^{T} \mathbf{H}) \mathbf{x}_{0} \right) \nonumber \\
&\hspace*{-40mm} \stackrel{(a)}{=} \exp\left( \frac{1}{2\sigma^{2}} \| \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} -  \frac{1}{\sigma} \mathbf{x}_{1}^{T} (\mathbf{H}^{T} \mathbf{H}) \mathbf{x}_{0} \right)  \exp   \left(  \mathbf{x}_{1}^{T}( \widetilde{\mathbf{H}}^{\dagger})^{T}\widetilde{\mathbf{H}}^{\dagger} \mathbf{x}_{2}  \right)\exp\left( \frac{1}{2 \sigma^{2}} \| \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} - \frac{1}{\sigma} \mathbf{x}_{2}^{T} (\mathbf{H}^{T} \mathbf{H}) \mathbf{x}_{0} \right) \nonumber \\
& \hspace*{-40mm} =  \bigg\langle \exp\left( \frac{1}{2 \sigma^{2}} \| \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} - \frac{1}{\sigma} \mathbf{x}_{1}^{T} (\mathbf{H}^{T} \mathbf{H}) \mathbf{x}_{0} \right)R_{g}^{(D)}(\cdot, \widetilde{\mathbf{H}}^{\dagger} \mathbf{x}_{1}), \nonumber \\ 
& \exp\left( \frac{1}{2 \sigma^{2}} \| \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} -  \frac{1}{\sigma}\mathbf{x}_{2}^{T} (\mathbf{H}^{T} \mathbf{H}) \mathbf{x}_{0} \right)R_{g}^{(D)}(\cdot,\widetilde{\mathbf{H}}^{\dagger} \mathbf{x}_{2}) \bigg\rangle_{\mathcal{H}(R_{g}^{(D)})} \nonumber \\Ê
&\hspace*{-40mm}  = \langle g_{\mathbf{x}_{1}}(\cdot) , g_{\mathbf{x}_{2}}(\cdot) \rangle_{\mathcal{H}(R_{g}^{(D)})}
\end{align}
where  $(a)$ follows from \eqref{equ_proof_isometr_R_g_quadr_form}.

Now, for an arbitrary $\mathbf{x} \in \mathbb{R}^{N}$ lets denote by $h_{\mathbf{x}}(\cdot) = \mathsf{K}_{g}[f_{\mathbf{x}}(\cdot)] \in \mathcal{H}(R_{g}^{(D)})$ the image of the function $f_{\mathbf{x}}(\cdot) \in  \mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}})$ (cf. \eqref{equ_proof_isometr_R_g_set_A_in_R_LGM}) under the mapping $\mathsf{K}_{g}[\cdot]$ defined in \eqref{equ_def_isometry_LGM}. 
We have
\begin{align}
h_{\mathbf{x}}(\mathbf{x}') & = f_{\mathbf{x}}( \sigma\widetilde{ \mathbf{H}} \mathbf{x}') \exp\left( - \frac{1}{2 \sigma^{2}} \| \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} + \frac{1}{\sigma} (\mathbf{x}')^{T} \widetilde{\mathbf{H}}^{\dagger} \mathbf{x}_{0}\right) \nonumber \\Ê
& = R_{\mathcal{M}_{\text{\tiny{LGM}}}}( \sigma \widetilde{\mathbf{H}}\mathbf{x}',\sigma \mathbf{x}) \exp\left( - \frac{1}{2 \sigma^{2}} \| \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} + \frac{1}{\sigma} (\mathbf{x}')^{T}\widetilde{\mathbf{H}}^{\dagger} \mathbf{x}_{0}\right) \nonumber  \\Ê
& =  \exp   \left( \frac{1}{\sigma^{2}}  (Ê\sigma \widetilde{\mathbf{H}} \mathbf{x}' - \mathbf{x}_{0})^{T} \mathbf{H}^{T} \mathbf{H} (\sigma \mathbf{x} - \mathbf{x}_{0}) \right)\exp\left( - \frac{1}{2\sigma^{2}} \| \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} + \frac{1}{\sigma} (\mathbf{x}')^{T} \widetilde{\mathbf{H}}^{\dagger} \mathbf{x}_{0}\right) \nonumber \\Ê
& \stackrel{(a)}{=}  \exp   \left(  (\mathbf{x}')^{T}\widetilde{\mathbf{H}}^{\dagger} \mathbf{x} +  \frac{1}{2 \sigma^{2}} \| \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} -  \frac{1}{\sigma} \mathbf{x}^{T} (\mathbf{H}^{T} \mathbf{H}) \mathbf{x}_{0}  \right)  \nonumber \\Ê
& = g_{\mathbf{x}}(\mathbf{x}'),
\end{align} 
where in $(a)$ we used \eqref{equ_proof_isometr_R_g_pseudo_inver_tilde_H}. 
The statement follows then straightforwardly from Theorem \ref{thm_suff_con_congruence_RKHS}. 
\end{proof}

In the following we will make use of the obvious facts summarized in 
\begin{lemma}
\label{lem_R_g_is_differentiable} 
The kernel $R_{g}^{(D)}(\cdot,\cdot): \mathbb{R}^{D} \times \mathbb{R}^{D} \rightarrow \mathbb{R}$ defined in \eqref{equ_def_kernel_R_g} is differentiable (cf. Definition \ref{def_differentiable_kernel}).
We have that for any vector $\mathbf{x}_{c} \in \mathbb{R}^{D}$, index set $\mathcal{K} \subseteq [D]$ and $\varepsilon >0$, the $\varepsilon$-$\mathcal{K}$-neighborhood of $\mathbf{x}_{c}$ (cf. \eqref{equ_def_epsilon_K_neighborhood}) belongs
to the domain of $R_{g}^{(D)}(\cdot,\cdot)$, i.e., $\mathcal{N}^{\mathcal{K}}_{\mathbf{x}_{c}}(\varepsilon) \subseteq \mathbb{R}^{D}$.
\end{lemma}

The RKHS $\mathcal{H}(R_{g}^{(D)})$ is entirely characterized by
\begin{theorem}
\label{thm_entire_character_H_R_g}
The RKHS $\mathcal{H}(R_{g}^{(D)})$ is separable and it contains the 
functions $g^{(\mathbf{p})}(\cdot): \mathbb{R}^{D} \rightarrow \mathbb{R}$ given by 
\begin{equation} 
g^{(\mathbf{p})} (\mathbf{x}) \triangleq  \frac{1}{\sqrt{\mathbf{p}!}} \frac{ \partial^{\mathbf{p}} R_{g}^{(D)}(\mathbf{x}, \mathbf{x}_{2})}{\partial \mathbf{x}_{2}^{\mathbf{p}}}\big|_{\mathbf{x}_{2} = \mathbf{0}} = \frac{1}{\sqrt{\mathbf{p}!}} \mathbf{x}^{\mathbf{p}},
\end{equation}
where $\mathbf{p} \in \mathbb{Z}_{+}^{D}$ is an arbitrary multi-index, i.e., 
\begin{equation}
\label{equ_part_der_element_RKHS_Rg}
\mathbf{p} \in \mathbb{Z}_{+}^{D} \Rightarrow g^{(\mathbf{p})}(\cdot) \in \mathcal{H}(R_{g}^{(D)}). 
\end{equation}
The inner-product of an arbitrary function $f(\cdot) \in \mathcal{H}(R_{g}^{(D)})$ with $g^{(\mathbf{p})}(\cdot)$ is given by 
\begin{equation} 
\label{equ_inner_prod_part_der_RKHS_Rg}
\langle f (\cdot), g^{(\mathbf{p})}(\cdot) \rangle_{\mathcal{H}(R_{g}^{(D)})} = \frac{1}{\sqrt{\mathbf{p}!}} \frac{ \partial^{\mathbf{p}} f(\mathbf{x})} {\partial \mathbf{x}^{\mathbf{p}}} \bigg|_{\mathbf{x} = 0}. 
\end{equation} 
Moreover, the set $\big\{ g^{(\mathbf{p})}(\cdot) \in \mathcal{H}(R_{g}^{(D)}) \big\}_{\mathbf{p} \in \mathbb{Z}_{+}^{D}}$ forms an ONB for $\mathcal{H}(R_{g}^{(D)})$. Thus 
any function $f(\cdot) \in \mathcal{H}(R_{g}^{(D)})$ can be written point-wise as 
\begin{equation}
\label{equ_series_repr_RKHS_R_g}
f(\mathbf{x}) = \sum_{\mathbf{p} \in \mathbb{Z}_{+}^{D}} a[\mathbf{p}] g^{(\mathbf{p})}(\mathbf{x}) =   \sum_{\mathbf{p} \in \mathbb{Z}_{+}^{D}} a[\mathbf{p}] \frac{1}{\sqrt{\mathbf{p}!}} \mathbf{x}^{\mathbf{p}},
\end{equation} 
with  a unique coefficient sequence $a[\mathbf{p}] \in \ell^{2}(\mathbb{Z}_{+}^{D})$. 
\end{theorem} 
\begin{proof}
The separability of $\mathcal{H}(R_{g}^{(D)})$ follows from \cite[Theorem 7]{HeinRKHS2004}, since obviously the domain $\mathbb{R}^{D}$ is separable and the kernel $R_{g}^{(D)}(\cdot,\cdot)$ is continuous. 
The validity of \eqref{equ_part_der_element_RKHS_Rg} and \eqref{equ_inner_prod_part_der_RKHS_Rg} follows from Lemma \ref{lem_R_g_is_differentiable} and Theorem \ref{thm_der_repr_prop}. 
By the power (Taylor) series representation of the exponential function \cite{RudinBook}, we have that the kernel $R_{g}^{(D)}(\cdot,\cdot)$ can be written point-wise as 
\begin{equation} 
R_{g}^{(D)}(\mathbf{x}_{1}, \mathbf{x}_{2}) = \exp ( \mathbf{x}_{1}^{T} \mathbf{x}_{2} ) = 
\sum_{\mathbf{p} \in \mathbb{Z}_{+}^{D}} \frac{1}{\mathbf{p}!} \mathbf{x}_{1}^{\mathbf{p}} \mathbf{x}_{2}^{\mathbf{p}} = 
\sum_{\mathbf{p} \in \mathbb{Z}_{+}^{D}} g^{(\mathbf{p})}(\mathbf{x}_{1}) g^{(\mathbf{p})}(\mathbf{x}_{2}),
\end{equation} 
which implies via Theorem \ref{thm_pointwise_series_kernel_ONB} that the set $\big\{ g^{(\mathbf{p})}(\cdot) \in \mathcal{H}(R_{g}^{(D)}) \big\}_{\mathbf{p} \in \mathbb{Z}_{+}^{D}}$ forms an ONB for $\mathcal{H}(R_{g}^{(D)})$, since it can be easily verified by \eqref{equ_inner_prod_part_der_RKHS_Rg} that $\langle g^{(\mathbf{p})}(\cdot),g^{(\mathbf{p}')}(\cdot) \rangle_{\mathcal{H}(R_{g}^{(D)})} = \delta_{\mathbf{p}, \mathbf{p}'}$.
The series representation in \eqref{equ_series_repr_RKHS_R_g} finally follows from Theorem \ref{thm_isometry_hilbert_space_coeffs_space}.  
\end{proof}

An specific class of functions that belong to $\mathcal{H}(R_{g}^{(D)})$ is presented in   
\begin{theorem} 
\label{thm_exp_times_finite_order_polynom_Rg}
Consider a coefficient sequence $a[\mathbf{p}]: \mathbb{Z}_{+}^{D} \rightarrow \mathbb{R}$ which satisfies the inequality
\begin{equation} 
\label{thm_specific_class_R_g_bound_coeffs}
| a[\mathbf{p}] | \leq C^{|\mathbf{p}|},
\end{equation} 
where $C>0$ is an arbitrary positive constant. 
The RKHS $\mathcal{H}(R_{g}^{(D)})$ contains any function $f(\cdot): \mathbb{R}^{D} \rightarrow \mathbb{R}$, given by 
$f(\mathbf{x}) = \exp( \mathbf{x}^{T} \mathbf{x}_{1}) \sum_{\mathbf{p} \in \mathbb{Z}_{+}^{D}} \frac{a[\mathbf{p}]}{\mathbf{p}!} \mathbf{x}^{\mathbf{p}}$, % \sum_{l=1}^{L} a_{l} \mathbf{x}^{\mathbf{p}_{l}}
%\end{equation}
where $\mathbf{x}_{1} \in \mathbb{R}^{D}$ is arbitrary. % and a coefficient sequence $a[\mathbf{p}] \in \mathbb{R}$ which satisfies \eqref{thm_specific_class_R_g_bound_coeffs}.% and $\mathbf{p}_{l} \in \mathbb{N}_{0}^{N}$. 
\end{theorem}
\begin{proof}
%Since under the assumption that \eqref{thm_specific_class_R_g_bound_coeffs} holds, both factors $\exp( \mathbf{x}^{T} \mathbf{x}_{1}) =\sum_{\mathbf{p} \in \mathbb{Z}_{+}^{D}} \frac{\mathbf{x}_{1}^{\mathbf{p}}}{\mathbf{p}!} \mathbf{x}^{\mathbf{p}}$ and $\sum_{\mathbf{p} \in \mathbb{Z}_{+}^{D}} \frac{a[\mathbf{p}]}{\mathbf{p}!} \mathbf{x}^{\mathbf{p}}$ are power series that are convergent everywhere on $\mathbb{R}^{D}$ 
Since $\exp( \mathbf{x}^{T} \mathbf{x}_{1}) =\sum_{\mathbf{p} \in \mathbb{Z}_{+}^{D}} \frac{\mathbf{x}_{1}^{\mathbf{p}}}{\mathbf{p}!} \mathbf{x}^{\mathbf{p}}$ and $\sum_{\mathbf{p} \in \mathbb{Z}_{+}^{D}} \frac{a[\mathbf{p}]}{\mathbf{p}!} \mathbf{x}^{\mathbf{p}}$ are power series that 
converge everywhere in $\mathbb{R}^{D}$ we can by \cite{KranzPrimerAnalytic}  write their product $f(\cdot)$ also as a power series in the form
\begin{equation}
\label{equ_proof_prod_analy_exp_in_R_g_4}
f(\mathbf{x}) = \sum_{\mathbf{p} \in \mathbb{Z}_{+}^{D}} c[\mathbf{p}] \mathbf{x}^{\mathbf{p}},
\end{equation} 
where the coefficients $c[\mathbf{p}]$ are obtained as \cite{KranzPrimerAnalytic} 
\begin{equation}
\label{equ_proof_prod_analy_exp_in_R_g_133}
c[\mathbf{p}] = \sum_{ \mathbf{n} \leq \mathbf{p}}   \frac{1}{\mathbf{n}!  (\mathbf{p}- \mathbf{n})!} a[\mathbf{p}] \mathbf{x}_{1}^{\mathbf{n}}. 
\end{equation} 
Now we show that the coefficients $d[\mathbf{p}]\triangleq c[\mathbf{p}] \sqrt{\mathbf{p}!}$ are square summable, i.e., $d[\mathbf{p}] \in \ell^{2}(\mathbb{Z}_{+}^{D})$ which 
then implies via \eqref{equ_proof_prod_analy_exp_in_R_g_4} and Theorem \ref{thm_entire_character_H_R_g} that $f(\cdot) \in \mathcal{H}(R_{g}^{(D)})$.

Indeed, using \eqref{thm_specific_class_R_g_bound_coeffs} and \eqref{equ_proof_prod_analy_exp_in_R_g_133}, we obtain the bound 
\begin{align} 
d[\mathbf{p}] & \leq \sum_{ \mathbf{n} \leq \mathbf{p}}   \frac{\sqrt{\mathbf{p}!}}{\mathbf{n}!  (\mathbf{p}- \mathbf{n})!} C^{|\mathbf{p}|} \| \mathbf{x}_{1}\|_{\infty}^{|\mathbf{n}|}  \frac{1}{\sqrt{\mathbf{p}!}} \sum_{ \mathbf{n} \leq \mathbf{p}}   \frac{\mathbf{p}!}{\mathbf{n}!  (\mathbf{p}- \mathbf{n})!} C^{|\mathbf{p}|} \| \mathbf{x}_{1}\|_{\infty}^{|\mathbf{n}|}= \frac{1}{\sqrt{\mathbf{p}!}} (C + \| \mathbf{x}_{1}\|_{\infty})^{|\mathbf{p}|}, 
\end{align} 
which obviously (e.g. via the ratio test \cite{RudinBookPrinciplesMatheAnalysis}) implies that $d[\mathbf{p}] \in \ell^{2}(\mathbb{Z}_{+}^{D})$.
%The statement is proved via Theorem \ref{thm_der_repr_prop} by noting that 
%\begin{equation}
%\exp( \mathbf{x}^{T} \mathbf{x}_{1}) \sum_{l=1}^{L} a_{l} \mathbf{x}^{\mathbf{p}_{l}} =  \sum_{l=1}^{L} a_{l}  \frac{\partial^{\mathbf{p}_{l}}  R_{g}(\mathbf{x}, \mathbf{x}_{2})}{\partial \mathbf{x}_{2}^{\mathbf{p}}} \bigg|_{\mathbf{x}_{2} = \mathbf{x}_{1}}.
%\end{equation} 
\end{proof} 
Note that Theorem \ref{thm_exp_times_finite_order_polynom_Rg} trivially implies that $\mathcal{H}(R_{g}^{(D)})$ contains any function $f(\cdot): \mathbb{R}^{D} \rightarrow \mathbb{R}$ that can be written as
\begin{equation}
f(\mathbf{x}) = \exp( \mathbf{x}^{T} \mathbf{x}_{1}) \sum_{l \in [L]} a_{l} \mathbf{x}^{\mathbf{p}_{l}}
\end{equation}
with arbitrary $\mathbf{x}_{1} \in \mathbb{R}^{D}$, $L \in \mathbb{N}$, $a_{l} \in \mathbb{R}$ and $\mathbf{p}_{l} \in \mathbb{Z}_{+}^{D}$. 

We will also make use of 
\begin{theorem}
\label{thm_part_der_any_origin_complete_R_g}
For an arbitrary parameter vector $\mathbf{x}_{c} \in \mathbb{R}^{D}$ and multi-index $\mathbf{p} \in \mathbb{Z}_{+}^{D}$ we define the function $g^{(\mathbf{p})}_{\mathbf{x}_{c}}(\cdot): \mathbb{R}^{D} \rightarrow \mathbb{R}$ by
\begin{equation}
g^{(\mathbf{p})}_{\mathbf{x}_{c}}(\mathbf{x}) \triangleq  \frac{\partial^{\mathbf{p}}  R_{g}^{(D)}(\mathbf{x}, \mathbf{x}_{2})}{\partial \mathbf{x}_{2}^{\mathbf{p}}} \bigg|_{\mathbf{x}_{2} = \mathbf{x}_{c}}.
\end{equation}
We then have that the function $g^{(\mathbf{p})}_{\mathbf{x}_{c}}(\cdot)$ belongs to the RKHS $\mathcal{H}(R_{g}^{(D)})$, i.e., 
\begin{equation} 
\label{equ_part_der_arb_point_eval_in_Rg}
\mathbf{p} \in \mathbb{Z}_{+}^{D},\mathbf{x}_{c} \in \mathbb{R}^{D} \Rightarrow g^{(\mathbf{p})}_{\mathbf{x}_{c}}(\cdot) \in \mathcal{H}(R_{g}^{(D)}). 
\end{equation}
The inner product of an arbitrary function $f(\cdot) \in \mathcal{H}(R_{g}^{(D)})$ with the function $g^{(\mathbf{p})}_{\mathbf{x}_{c}}(\mathbf{x})$ is given by  
\begin{equation}
\label{equ_part_der_inner_prod_R_g}
\langle g^{(\mathbf{p})}_{\mathbf{x}_{c}}(\cdot) , f(\cdot) \rangle_{\mathcal{H}(R_{g}^{(D)})} = \frac{\partial^{\mathbf{p}}  f(\mathbf{x})}{\partial \mathbf{x}^{\mathbf{p}}} \bigg|_{\mathbf{x} = \mathbf{x}_{c}}. 
\end{equation} 

Moreover, the set $\{ g^{\mathbf{p}}_{\mathbf{x}_{c}}(\cdot) \}_{\mathbf{p} \in \mathbb{Z}_{+}^{D}}$ is complete for $\mathcal{H}(R_{g}^{(D)})$, which implies 
in particular that if two functions $f(\cdot), g(\cdot) \in \mathcal{H}(R_{g}^{(D)})$ take on the same values on $\mathcal{B}(\mathbf{x}_{c},r) \subseteq \mathbb{R}^{D}$ with an arbitrary radius $r>0$, then 
they are identical, i.e., $f(\cdot) = g(\cdot)$. 
\end{theorem}
\begin{proof} 
The validity of \eqref{equ_part_der_arb_point_eval_in_Rg} and \eqref{equ_part_der_inner_prod_R_g} follows from Theorem \ref{thm_der_repr_prop} by the fact that $R_{g}^{(D)}(\cdot,\cdot)$ is a differentiable kernel. 
%The completeness is proved via Theorem \ref{thm_set_spans_space_implies_completeness} by showing that the set  $\{ g^{\mathbf{p}}_{\mathbf{x}_{c}}(\cdot) \}_{\mathbf{p} \in \mathbb{N}_{0}^{N}}$ spans 
%$\mathcal{H}(R_{g})$. To that end it is by Theorem \ref{thm_densensess_lin_space_denseness_rkhs} sufficient to show that for any function $f(\cdot) \in \mathcal{L}(R_{g})$ and $\varepsilon > 0$ we can find a finite linear combination $g(\cdot) = \sum_{l=1}^{L} a_{l} g^{\mathbf{p}_{l}}_{\mathbf{x}_{c}}(\cdot)$ with $L \in \mathbb{N}$,$a_{l} \in \mathbb{R}$, $\mathbf{p}_{l} \in \mathbb{N}_{0}^{N}$ such 
%that $\| g(\cdot) - f(\cdot) \|_{\mathcal{H}(R_{g})} \leq \varepsilon$. 
To prove the completeness (cf. Definition \ref{def_complete_set}) of the set $\{ g^{(\mathbf{p})}_{\mathbf{x}_{c}}(\cdot) \}_{\mathbf{p} \in \mathbb{Z}_{+}^{D}}$ we consider an arbitrary function 
$f(\cdot) \in \mathcal{H}(R_g)$ and note that by \eqref{equ_series_repr_RKHS_R_g} of Theorem \ref{thm_entire_character_H_R_g} it can be represented as a 
power series which converges everywhere in $\mathbb{R}^{D}$. 
According to \cite[Proposition 1.2.3]{KranzPrimerAnalytic} we can then represent the function as
%the well-known Taylor expansion \cite{RudinBook} of the exponential function we have 
\begin{equation} 
\label{equ_proof_part_der_span_R_g_LGM_taylor}
f(\mathbf{x}) = \sum_{\mathbf{p}: |\mathbf{p}| \leq L}  \frac{\partial^{\mathbf{p}}  f(\mathbf{x})}{\partial \mathbf{x}^{(\mathbf{p})}} \bigg|_{\mathbf{x} = \mathbf{x}_{c}}  \frac{1}{\mathbf{p}!} ( \mathbf{x}- \mathbf{x}_c ) ^{\mathbf{p}}  + R_{L}(\mathbf{x})
\end{equation} 
where the remainder term $R_{L}(\mathbf{x})$ is such that for any $\mathbf{x} \in \mathbb{R}^{D}$ we have that $\lim_{L \rightarrow \infty} |R_{L}(\mathbf{x})| = 0$. 
By using \eqref{equ_part_der_inner_prod_R_g} we can rewrite \eqref{equ_proof_part_der_span_R_g_LGM_taylor} as 
\begin{equation} 
\label{equ_proof_part_der_span_R_g_LGM_taylor_inner_prod}
f(\mathbf{x})= \sum_{\mathbf{p}: |\mathbf{p}| \leq L}  \frac{\langle g^{(\mathbf{p})}_{\mathbf{x}_{c}}(\cdot), f(\cdot) \rangle_{\mathcal{H}(R_{g}^{(D)})} }{\mathbf{p}!} (\mathbf{x}-\mathbf{x}_{c})^{\mathbf{p}}    + R_{L}(\mathbf{x}).
\end{equation} 
Thus we conclude that if $\langle g^{(\mathbf{p})}_{\mathbf{x}_{c}}(\cdot) , f(\cdot) \rangle_{\mathcal{H}(R_{g}^{(D)})}=0$ for all $\mathbf{p} \in \mathbb{Z}_{+}^{D}$, the function $f(\cdot)$ necessarily has to be zero for all arguments, i.e., $f(\cdot) \equiv 0$. 
\end{proof}

\section{Minimum Variance Estimation for the SLM}
\label{sec_RKHS_basic_facts_SLM}
In the next section we will derive lower bounds on the minimum achievable variance $L_{\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0})}$ for a class of minimum variance problems denoted
by $\{ \mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0}) \}_{\mathbf{x}_{0} \in \mathcal{X}_{S}}$ where 
\begin{equation}
\label{equ_def_SLM_func_x_0}
\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0}) \triangleq \left( \mathcal{E}_{\text{\tiny{SLM}}}, c(\cdot), \mathbf{x}_{0} \right)
\end{equation}
for a fixed choice for the SLM parameters $\sigma$, $S$, $M$, $N$, $\mathbf{H}$ and prescribed bias function $c(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}$. 
For the special case $S=N$, i.e., where the SLM coincides with the LGM we will use the shorthand
\begin{equation}
\mathcal{M}_{\text{\tiny{LGM}}}(\mathbf{x}_{0}) \triangleq \left( \mathcal{E}_{\text{\tiny{LGM}}}, \tilde{c}(\cdot), \mathbf{x}_{0} \right).
\end{equation}
In this section we present some fundamental properties of $L_{\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0})}$. 

The following statement gives a detailed characterization of the class of valid bias functions for $\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0})$ and moreover 
states explicit expressions of the minimum achievable variance and corresponding LMV estimator for a valid bias function. 
\begin{theorem}
\label{thm_condition_valid_bias_SLM}
Consider the SLM $\mathcal{E}_{\text{\tiny{SLM}}}$ with specific values of $S$, $M$, $N$, $\mathbf{H} \in \mathbb{R}^{M \times N}$ and 
denote the thin SVD of $\mathbf{H}$ by $\mathbf{H} = \mathbf{U} \mathbf{\Sigma} \mathbf{V}^{T}$.
For a specific choice for $\mathbf{x}_{0} \in \mathcal{X}_{S}$, we have that a prescribed bias function $c(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}$ 
is valid for $\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0}) \triangleq \left(\mathcal{E}_{\text{\tiny{SLM}}},c(\cdot), \mathbf{x}_{0}\right) $, i.e., $L_{\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0})} < \infty$, 
if and only if it can be written for every $\mathbf{x} \in \mathcal{X}_{S}$ as 
\begin{equation} 
\label{equ_condition_gamma_valid_SLM_fourier_series_R_g}
c(\mathbf{x}) = \exp \left(  \frac{1}{2 \sigma^{2}} \| \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} - \frac{1}{\sigma^{2}} \mathbf{x}^{T}\mathbf{H}^{T} \mathbf{H} \mathbf{x}_{0} \right) \sum_{\mathbf{p} \in \mathbb{Z}_{+}^{N}} \frac{1}{\sqrt{\mathbf{p}!}} a[\mathbf{p}] \bigg( \frac{1}{\sigma} \widetilde{\mathbf{H}}^{\dagger} \mathbf{x}\bigg)^{\mathbf{p}} - x_{k},
\end{equation} 
with a specific coefficient sequence $a[\mathbf{p}] \in \ell^{2}(\mathbb{Z}_{+}^{D})$,  $D = \rank(\mathbf{H})$, and $\widetilde{\mathbf{H}} \triangleq \mathbf{V} \mathbf{ \Sigma}^{-1}$. 
%\begin{equation} 
%c(\mathbf{x}) = \gamma(\mathbf{x})  - x_{k}
%\end{equation}
%with a function $\gamma(\cdot): \mathbb{R}^{N} \rightarrow \mathbb{R}$ that is such that there exists a 
%coefficient sequence $a[\mathbf{p}] \in \ell^{2}(\mathbb{Z}_{+}^{D})$,  $D = \rank(\mathbf{H})$, that solves the equation
%\begin{equation} 
%\label{equ_condition_gamma_valid_SLM_fourier_series_R_g}
%\gamma( \sigma \widetilde{\mathbf{H}} \mathbf{x})  \exp\left( - \frac{1}{2\sigma^{2}} \| \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} +Ê\frac{1}{\sigma} \mathbf{x}^{T}  \widetilde{\mathbf{H}}^{\dagger}\mathbf{x}_{0}\right)
%= \sum_{\mathbf{p} \in \mathbb{Z}_{+}^{D}} \frac{1}{\sqrt{\mathbf{p}!}} a[\mathbf{p}] \mathbf{x}^{\mathbf{p}},
%\end{equation}
%where $\widetilde{\mathbf{H}} \triangleq \mathbf{V} \mathbf{ \Sigma}^{-1}$,
%for every $\mathbf{x} \in \mathbb{R}^{D}$. 
If a prescribed bias function $c(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}$ is valid for $\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0})$ then we have that $c(\cdot)$ is necessarily continuos. 

The minimum achievable variance for $\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0})$ is obtained via the minimum squared $\ell^{2}(\mathbb{Z}_{+}^{D})$ norm $\| a[\cdot] \|_{\ell^{2}(\mathbb{Z}_{+}^{D})} \triangleq \sqrt{\sum_{\mathbf{p} \in \mathbb{Z}_{+}^{D}} | a[\mathbf{p}]|^{2}}$ 
among all coefficient sequences $a[\mathbf{p}] \in \ell^{2}(\mathbb{Z}_{+}^{D})$ that solve \eqref{equ_condition_gamma_valid_SLM_fourier_series_R_g}, i.e., 
\begin{equation}
\label{equ_def_min_var_SLM_opt_coeff_sequences}
L_{\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0})} = 
\min_{ \substack{ a[\mathbf{p}] \in \ell^{2}(\mathbb{Z}_{+}^{D}) \\ a[\mathbf{p}] \mbox{ solves \eqref{equ_condition_gamma_valid_SLM_fourier_series_R_g}}}} \| a[\cdot] \|^{2}_{\ell^{2}(\mathbb{Z}_{+}^{D})} - (c(\mathbf{x}_{0}) + x_{0,k})^{2}
\end{equation} 

Furthermore, given any valid bias function $c(\cdot)$, we have that for every coefficient sequence $a[\mathbf{p}] \in \ell^{2}(\mathbb{Z}_{+}^{D})$ which solves \eqref{equ_condition_gamma_valid_SLM_fourier_series_R_g}, that 
the specific estimator $\hat{g}(\cdot): \mathbb{R}^{M} \rightarrow \mathbb{R}$ given by 
\begin{equation} 
\label{equ_est_arb_coeffs_SLM}
\hat{g}(\cdot) \triangleq \exp \big( - \frac{1}{2\sigma^{2}} \| \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} \big) \sum_{\mathbf{p} \in \mathbb{Z}^{D}_{+}} \frac{a[\mathbf{p}]}{\sqrt{\mathbf{p}!}} \frac{ \partial^{\mathbf{p}} \bigg( \rho_{\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0})}(\cdot,\sigma \widetilde{\mathbf{H}} \mathbf{x}) \exp \big( \frac{1}{\sigma} \mathbf{x}_{0}^{T} \mathbf{H}^{T} \mathbf{H} \widetilde{\mathbf{H}} \mathbf{x} \big) \bigg)}{ \partial \mathbf{x}^{\mathbf{p}}} \Bigg|_{\mathbf{x} = \mathbf{0}} 
\end{equation}
is an allowed estimator for $\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0})$, i.e., $\hat{g}(\cdot) \in \mathcal{F}(\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0}))$. 

Finally, the estimator obtained from \eqref{equ_est_arb_coeffs_SLM} by the specific coefficient sequence $a_{0}[\mathbf{p}] \in  \ell^{2}(\mathbb{Z}_{+}^{D})$, which has 
the minimum $\ell^{2}(\mathbb{Z}_{+}^{D})$ norm $\| a[\cdot] \|_{\ell^{2}(\mathbb{Z}_{+}^{D})} \triangleq \sqrt{\sum_{\mathbf{p} \in \mathbb{Z}_{+}^{D}} | a[\mathbf{p}]|^{2}}$ among all coefficient 
sequences that solve \eqref{equ_condition_gamma_valid_SLM_fourier_series_R_g}, is the LMV estimator for $\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0})$. 
\end{theorem} 

\begin{proof}
By Theorem \ref{thm_main_facts_RKHS_MVE} we have that the prescribed bias function $c(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}$ is valid for $\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0})$ 
if and only if $c(\mathbf{x}) + x_{k} \in \mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0}))$ which by Theorem 
\ref{thm_relation_RKHS_LGM_SLM} is the case if and only if there exists a function $\gamma(\cdot) \in \mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}}(\mathbf{x}_{0}))$ such that $\gamma(\mathbf{x}) = c(\mathbf{x}) + x_{k}$ for every $\mathbf{x} \in \mathcal{X}_{S}$. 

Furthermore, by Theorem \ref{thm_isometry_LGM} $\gamma(\cdot) \in \mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}}(\mathbf{x}_{0}))$ if and only if 
\begin{equation} 
\label{equ_cond_bias_valid_isom_R_g_D}
\gamma( \sigma \widetilde{\mathbf{H}} \mathbf{x})  \exp\left( - \frac{1}{2 \sigma^{2}} \| \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} + \frac{1}{\sigma} \mathbf{x}^{T}  \widetilde{\mathbf{H}}^{\dagger}\mathbf{x}_{0}\right)  \in \mathcal{H}(R_{g}^{(D)}),
\end{equation} 
with $D=\rank(\mathbf{H})$, which by Theorem \ref{thm_entire_character_H_R_g} is the case if and 
only if there exists a coefficient sequence $a[\mathbf{p}] \in \ell^{2}(\mathbb{Z}_{+}^{D})$ that solves \eqref{equ_condition_gamma_valid_SLM_fourier_series_R_g} for every $\mathbf{x} \in \mathbb{R}^{D}$.
Thus, if a specific prescribed bias function $c(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}$ is valid for $\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0})$ it can be 
written due to \eqref{equ_cond_bias_valid_isom_R_g_D}, \eqref{equ_condition_gamma_valid_SLM_fourier_series_R_g}, \eqref{equ_invar_prop_LGM_kernel_H} and the obvious fact $\Ker(\mathbf{H}) = \Ker(\widetilde{\mathbf{H}}^{\dagger})$ as 
\begin{equation} 
\label{equ_decomp_bias_valid_SLM_fourier_series_R_g}
c(\mathbf{x}) = h \left(\frac{1}{\sigma} \widetilde{\mathbf{H}}^{\dagger} \mathbf{x}\right)  - x_{k}
\end{equation}
with the function $h(\cdot): \mathbb{R}^{N} \rightarrow \mathbb{R}$ given by
\begin{equation}
\label{equ_decomp_bias_valid_SLM_fourier_series_R_g_1}
h(\mathbf{x}) = \exp \left(  \frac{1}{2 \sigma^{2}} \| \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} - \frac{1}{\sigma} \mathbf{x}^{T} \widetilde{\mathbf{H}}^{\dagger} \mathbf{x}_{0} \right) \sum_{\mathbf{p} \in \mathbb{Z}_{+}^{N}} \frac{1}{\sqrt{\mathbf{p}!}} a[\mathbf{p}]  \mathbf{x}^{\mathbf{p}},
\end{equation}
where $a[\mathbf{p}] \in \ell^{2}(\mathbb{Z}_{+}^{D})$. Upon combining \eqref{equ_decomp_bias_valid_SLM_fourier_series_R_g} with \eqref{equ_decomp_bias_valid_SLM_fourier_series_R_g_1} we verify \eqref{equ_condition_gamma_valid_SLM_fourier_series_R_g}. 

The function $h(\cdot)$ is continuous since $ \exp \left(  \frac{1}{2} \| \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} - \mathbf{x}^{T} (\mathbf{H}^{T} \mathbf{H})^{1/2} \mathbf{x}_{0} \right)$ is obviously continuous and 
the continuity of $\sum_{\mathbf{p} \in \mathbb{Z}_{+}^{N}} \frac{1}{\sqrt{\mathbf{p}!}} a[\mathbf{p}]  \mathbf{x}^{\mathbf{p}}$ follows from the fact that this power series converges for every $\mathbf{x} \in \mathbb{R}^{N}$ (cf. \cite{KranzPrimerAnalytic}). 
We can therefore conclude from \eqref{equ_decomp_bias_valid_SLM_fourier_series_R_g} that $c(\mathbf{x})$ has to be continuous. However, the continuity of any valid bias function $c(\cdot)$ could also be verified more directly using Theorem \ref{thm_continous_kernel_implies_cont_func} since the kernel $R_{\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0})}$ (cf. \eqref{equ_kernel_SLM}) is obviously continuous. 

The relation \eqref{equ_def_min_var_SLM_opt_coeff_sequences} follows then from Theorem \ref{thm_relation_RKHS_LGM_SLM}, Theorem \ref{thm_isometry_LGM}, Theorem \ref{thm_entire_character_H_R_g} and Theorem \ref{thm_fourier_onb}, since 
the right hand side of \eqref{equ_condition_gamma_valid_SLM_fourier_series_R_g} yields any function $f(\cdot) \in \mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0}))$ by suitable choice for the coefficient sequence $a[\mathbf{p}]$.

Now consider a valid bias function $c(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}$ and a coefficient sequence $a[\mathbf{p}] \in \ell^{2}(\mathbb{Z}_{+}^{D})$ that solves \eqref{equ_condition_gamma_valid_SLM_fourier_series_R_g}. 
Then we have by Theorem \ref{thm_isometry_LGM} that the ``extended'' bias function $\tilde{c}(\cdot): \mathbb{R}^{N} \rightarrow \mathbb{R}$ given by 
\begin{align} 
\tilde{c}(\mathbf{x}) & =  \exp \left(  \frac{1}{2 \sigma^{2}} \| \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} - \frac{1}{\sigma^{2}} \mathbf{x}^{T} \mathbf{H}^{T} \mathbf{H} \mathbf{x}_{0} \right) 
\sum_{\mathbf{p} \in \mathbb{Z}_{+}^{N}} \frac{a[\mathbf{p}]}{\sqrt{\mathbf{p}!}}   \bigg(\frac{1}{\sigma} \widetilde{\mathbf{H}}^{\dagger} \mathbf{x}\bigg)^{\mathbf{p}} - x_{k} \nonumber \\ 
& = \exp \big( - \frac{1}{2\sigma^{2}} \| \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} \big)  \sum_{\mathbf{p} \in \mathbb{Z}_{+}^{N}} \frac{a[\mathbf{p}]}{\sqrt{\mathbf{p}!}}   
\frac{ \partial^{\mathbf{p}} \bigg( R_{\text{\tiny{LGM}}}(\mathbf{x}, \sigma \widetilde{\mathbf{H}} \mathbf{x}') \exp \big( \frac{1}{\sigma} \mathbf{x}_{0}^{T} \mathbf{H}^{T} \mathbf{H} 
\widetilde{\mathbf{H}} \mathbf{x}' \big) \bigg)}{\partial \mathbf{x}'^{\mathbf{p}}}\Bigg|_{\mathbf{x}'=\mathbf{0}} - x_{k} \label{equ_def_arb_bias_coeffs_LGM_2}
\end{align} 
is valid for $\mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}}(\mathbf{x}_{0}))$ and by its very definition satisfies $\tilde{c}(\cdot) \big|_{\mathcal{X}_{S}} = c(\cdot)$ implying $\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0}) = \mathcal{M}_{\text{\tiny{LGM}}}(\mathbf{x}_{0})) \big|_{\mathcal{X}_{S}}$. 
Using Theorem \ref{thm_der_repr_prop_mult_func}, Theorem \ref{thm_main_facts_RKHS_MVE} and Theorem \ref{thm_isometry_RKHS_rhos_derivative_kernel} it can be verified that the estimator $\hat{g}(\cdot)$ defined by \eqref{equ_est_arb_coeffs_SLM} for a coefficient sequence $a[\mathbf{p}] \in \ell^{2}(\mathbb{Z}_{+}^{D})$ is nothing but the LMV estimator for $\mathcal{M}_{\text{\tiny{LGM}}}(\mathbf{x}_{0})$. % with the bias in \eqref{equ_def_arb_bias_coeffs_LGM_2} using the same coefficient sequence. 
Because it is the LMV estimator for the minimum variance problem $\mathcal{M}_{\text{\tiny{LGM}}}(\mathbf{x}_{0})$ we have by Theorem \ref{thm_main_facts_RKHS_MVE}, Theorem \ref{thm_isometry_LGM}, Theorem \ref{thm_entire_character_H_R_g} 
and Theorem \ref{thm_fourier_onb} that $v(\hat{g}(\cdot); \mathbf{x}_{0}) = \| a[\cdot] \|^{2}_{\ell^{2}(\mathbb{Z}_{+}^{D})} - (c(\mathbf{x}_{0}) + x_{0,k})^{2}$. 
Since $\tilde{c}(\cdot) \big|_{\mathcal{X}_{S}} = c(\cdot)$ we have that this estimator has the prescribed bias $c(\cdot)$ on the subset $\mathcal{X}_{S} \subseteq \mathcal{X}$ and trivially also finite variance at $\mathbf{x}_{0} \in \mathcal{X}_{S}$ (because it is a LMV estimator for $\mathcal{M}_{\text{\tiny{LGM}}}(\mathbf{x}_{0})$ at this specific parameter vector), i.e., it is an allowed estimator for $\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0})$. Finally, if the coefficient sequence $a[\mathbf{p}]$ in \eqref{equ_est_arb_coeffs_SLM} is chosen as the optimum of the problem \eqref{equ_def_min_var_SLM_opt_coeff_sequences} then we have obviously that the corresponding estimator given by \eqref{equ_est_arb_coeffs_SLM} is the LMV estimator for $\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0})$ since its variance at $\mathbf{x}_{0}$ is by definition the solution of \eqref{equ_def_min_var_SLM_opt_coeff_sequences}. 
%Moreover the LMV estimator for $\mathcal{M}_{\text{\tiny{LGM}}}(\mathbf{x}_{0})$ with the bias $c(\cdot)$ 
%we have that for a valid bias function $c(\cdot)$ we can write the prescribed mean $\gamma(\mathbf{x}) = c(\mathbf{x}) + x_{k}$ as: 
\end{proof}
One specific implication of Theorem \ref{thm_condition_valid_bias_SLM} concerning the problem of sparsity pattern detection (cf. \cite{EstThSparsPattRec,KarbasiSuppRecCS,WainInfThBoundsSparsPattRec}) 
is stated in 
\begin{theorem}
\label{thm_non_esit_finite_var_unbiased_est_supp}
There exists no estimator $\hat{g}(\mathbf{y})$ of a real valued function $g(\supp(\mathbf{x}))$ of the support of $\mathbf{x} \in \mathcal{X}_{S}$ which uses only the observation \eqref{equ_linear_observation_model} of the SLM $\mathcal{E}_{\text{\tiny{SLM}}}$, is unbiased for every $\mathbf{x} \in \mathcal{X}_{S}$ and has 
a finite variance at any $\mathbf{x}_{0} \in \mathcal{X}_{S}$.
\end{theorem}
\begin{proof}
Lets encode the set of all subsets of $[N]$, i.e., the power set $\mathcal{P} ( [N] )$, by an injective mapping $\mathfrak{i}(\cdot): \mathcal{P} ( [N] ) \rightarrow \mathbb{R}$, i.e., to each subset $\mathcal{S} \subseteq [N]$ we assign the unique number $\mathfrak{i}( \mathcal{S}) \in \mathbb{R}$. For the proof of the statement we can without loss of generality restrict ourselves to the specific function $g(\supp(\mathbf{x})) = \mathfrak{i}(\supp(\mathbf{x}))$.  
Consider then the SLM $\mathcal{E}_{\text{\tiny{SLM}}}$, but instead of estimating the parameter function $g(\mathbf{x}) = x_{k}$ (for some fixed index $k \in [N]$) we are 
interested in unbiased estimation the support $\supp(\mathbf{x})$, i.e., we 
use the parameter function $g(\mathbf{x}) = \mathfrak{i}(\supp (\mathbf{x} ))$. According to Section \ref{sec_equ_bias_param_function} this is equivalent to a minimum variance problem associated with the ordinary SLM $\mathcal{E}_{\text{\tiny{SLM}}}$, i.e., with the parameter function $g(\mathbf{x}) = x_{k}$ and using the prescribed bias function $c'(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}: c'(\mathbf{x}) = \mathfrak{i}(\supp(\mathbf{x})) - x_{k}$ which is obviously discontinuous. 
However, since the prescribed bias function $c'(\cdot)$ is discontinuous we have by Theorem \ref{thm_condition_valid_bias_SLM} that this bias function is not valid for any minimum variance problem  
$\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0})$ with $\mathbf{x}_{0} \in \mathcal{X}_{S}$, i.e., there exists no estimator with the bias $c'(\cdot)$ and finite variance at any point $\mathbf{x}_{0} \in \mathcal{X}_{S}$. 
Thus, by Theorem \ref{thm_estimable_equiv_valid}, we have that the parameter function $g(\mathbf{x}) = \mathfrak{i}(\supp (\mathbf{x} ))$ is not estimable for the SLM $\mathcal{E}_{\text{\tiny{SLM}}}$ at any $\mathbf{x}_{0} \in \mathcal{X}_{S}$, which is just an equivalent formulation of the statement. 
\end{proof}
It is important to note that Theorem \ref{thm_non_esit_finite_var_unbiased_est_supp} asserts the impossibility of a finite variance estimator of the support 
of the parameter vector $\mathbf{x}$ which is unbiased for all $\mathbf{x} \in \mathcal{X}_{S}$. 
However, even if it might seem at first sight, Theorem \ref{thm_non_esit_finite_var_unbiased_est_supp} does not contradict \cite{EstThSparsPattRec,KarbasiSuppRecCS} 
since the authors of \cite{EstThSparsPattRec,KarbasiSuppRecCS} intentionally reduce the parameter set $\mathcal{X}_{S}$ of the SLM to a smaller parameter set $\mathcal{X}'$ which includes only vectors $\mathbf{x}$ 
with exactly $S$ non-zeros, i.e., $\| \mathbf{x} \|_{0} = S$ and whose smallest non-zero magnitude is not smaller than a given threshold $\theta_{min}$, i.e., $\min_{k \in \supp(\mathbf{x})} |x_{k}| \geq \theta_{min}$. 

The next statement shows that if a bias function is valid for $\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0})$ at some $\mathbf{x}_{0} \in \mathcal{X}_{S}$ it needs not necessarily be then also valid for any $\mathbf{x}_{0} \in \mathcal{X}_{S}$. 
\begin{theorem}
Consider the SLM $\mathcal{E}_{\text{\tiny{SLM}}}$ with arbitrary values of $S$, $N$ and $\mathbf{H}$. Then in the general case 
there are bias functions $c(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}$ that are valid for $\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0})$ for some choices for $\mathbf{x}_{0}$, i.e., $L_{\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0})} < \infty$ for some $\mathbf{x}_{0} \in \mathcal{X}_{S}$, but not for all possible choices for $\mathbf{x}_{0} \in \mathcal{X}_{S}$, i.e., for some $\mathbf{x}_{0} \in \mathcal{X}_{S}$ we have $L_{\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0})} = \infty$. 
\end{theorem} 
\begin{proof}
We prove this statement by using a specific choice for $S$, $M$, $N$, $\sigma^{2}$ and $\mathbf{H}$ and explicitly constructing a 
prescribed bias function $c(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}$ which is valid only for certain choices for $\mathbf{x}_{0}$ but not for any choice for $\mathbf{x}_{0}$. 
In particular we fix $S=M=N=\sigma^{2}=1$ as well as $\mathbf{H}=\mathbf{I}$. For this specific instance of the SLM we consider 
the specific prescribed bias function $c_{0}(x)$ (note that the parameter $x$ is a scalar for $N=1$) given as 
\begin{equation}
\label{equ_proof_not_everywhere_valid_LGM_1}
c_{0}(x) = \sum_{p\in \mathbb{Z}_{+}} \frac{1}{\sqrt{p!}} p^{-0.6} x^{p} - x.
\end{equation} 
 
We now show that this bias function is valid for $x_{0} =  0$ but not for any $x_{0} >0$. 
The validity of the bias function $c_{0}(x)$ for $x_0 = 0$ follows straightforwardly by its construction in \eqref{equ_proof_not_everywhere_valid_LGM_1} from Theorem \ref{thm_condition_valid_bias_SLM}. 
Now lets assume that $x_{0} > 0$. %We then have by Theorem \ref{thm_condition_valid_bias_SLM} that $c(x)$ is valid for $\mathcal{M}(\mathbf{x}_{0})$ if and only if the product between
%$\gamma(\mathbf{x}) = c(\mathbf{x}) + \mathbf{x}$ and $\exp \left( - \frac{x_{0}^2}{2} + x_0 x \right)$ is given by a series  
%is such that
According to \cite{KranzPrimerAnalytic} we have that the product $(c_{0}(x) +x)\exp \left( - \frac{x_{0}^2}{2} + x_0 x \right)$ can be written uniquely as a power-series, i.e., 
\begin{equation} 
(c_{0}(x) +x) \exp \left( - \frac{x_{0}^2}{2} + x_0 x \right) = \sum_{p \in \mathbb{Z}_{+}} \frac{1}{\sqrt{p!}} a_{0}[p] x^{p}
\end{equation} 
where the coefficients $a_{0}[p]$ are unique and given explicitly \cite{KranzPrimerAnalytic} by 
\begin{equation} 
a_{0}[p] = \exp \left( -\frac{x_{0}^{2}}{2} \right)  \sqrt{p!} \sum_{l=0}^{p} {\frac{ (p-l)^{-0.6} }{\sqrt{(p-l)!}}\frac{x_0^{l}}{l!}}. 
\end{equation}
For $p>1$ and $x_{0} >0$, these coefficients can be lower bounded by 
\begin{align} 
a_{0}[p] & \geq x_0 \exp \left( -\frac{x_{0}^{2}}{2} \right)  \sqrt{p!} \frac{(p-1)^{-0.6}}{\sqrt{(p-1)!}}  = 
x_0 \exp \left( -\frac{x_{0}^{2}}{2} \right)  \sqrt{p} (p-1)^{-0.6}  \nonumber \\ 
& \geq x_0  \exp \left( -\frac{x_{0}^{2}}{2} \right) \sqrt{p-1} (p-1)^{-0.6} = x_0 \exp \left( -\frac{x_{0}^{2}}{2} \right)  (p-1)^{-0.1}
\end{align} 
which implies that $a_{0}[p] \notin \ell^{2}(\mathbb{Z}_{+})$ and in turn, via Theorem \ref{thm_condition_valid_bias_SLM}, that the bias function $c_{0}(\mathbf{x})$ is not valid for $x_{0} > 0$. 
\end{proof}

The shape of $L_{\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0})}$ (viewed as a function of $\mathbf{x}_{0} \in \mathcal{X}_{S})$ is characterized by 
\begin{theorem} 
\label{thm_SLM_min_achiev_var_lower_semi_cont}
Consider the SLM $\mathcal{E}_{\text{\tiny{SLM}}}$ with specific values of $S$, $M$, $N$ and $\mathbf{H}$ and a prescribed bias function $c(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}$ that is valid for 
any $\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0})$ (cf. \eqref{equ_def_SLM_func_x_0}) with $\mathbf{x}_{0} \in \mathcal{X}_{S}$. 
Then the minimum achievable variance $L_{\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0})}$ exists, i.e., is finite for every $\mathbf{x}_{0}$, and viewed as a function of $\mathbf{x}_{0}$ is lower semi-continuous. 
\end{theorem} 
\begin{proof} 
This fact follows from Theorem \ref{thm_lower_semi_cont_varying_kernel} by noting that the kernel $R_{\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0})}(\cdot,\cdot)$ (cf. \eqref{equ_kernel_SLM}) obviously satisfies \eqref{equ_def_cont_varying_kernel}.
\end{proof} 

Finally, we give two sufficient conditions on the prescribed bias $c(\cdot)$ to be valid for $\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0})$ with arbitrary $\mathbf{x}_{0} \in \mathcal{X}_{S}$:  
\begin{theorem} 
\label{thm_suff_cond_valid_erervwhere_SLM_power_series}
Consider the minimum variance problem $\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0})$ with system matrix $\mathbf{H} \in \mathbb{R}^{M \times N}$ and a prescribed bias function $c(\mathbf{x})$ which is given as a product of an exponential 
and a power series, i.e., 
\begin{equation}
\label{equ_prescr_bias_finite_order_polynom_SLM}
c(\mathbf{x}) = \exp \left( \mathbf{x}_{1}^{T} \mathbf{x} \right) \sum_{\mathbf{p} \in \mathbb{Z}_{+}^{D}} \frac{a[\mathbf{p}]}{\mathbf{p}!}  \bigg( \frac{1}{\sigma} \widetilde{\mathbf{H}}^{\dagger} \mathbf{x}\bigg)^{\mathbf{p}} , 
\end{equation} 
with an arbitrary vector $\mathbf{x}_{1} \in \mathbb{R}^{N}$. 
Then we have if the coefficients satisfy $| a[\mathbf{p}] | \leq C^{|\mathbf{p}|}$ with an arbitrary constant $C$, the bias $c(\cdot)$ is valid for any $\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0})$ with $\mathbf{x}_{0} \in \mathcal{X}_{S}$. 
\end{theorem}
\begin{proof} 
The statement follows from Theorem \ref{thm_exp_times_finite_order_polynom_Rg}, Theorem \ref{thm_isometry_LGM}, Theorem \ref{thm_relation_RKHS_LGM_SLM} and Theorem \ref{thm_main_facts_RKHS_MVE}. 
\end{proof}
Note that it is obvious from Theorem \ref{thm_suff_cond_valid_erervwhere_SLM_power_series} that any bias function which is a finite-order polynomial, i.e.,  
$c(\mathbf{x}) = \sum_{l=1}^{L} a_{l} \mathbf{x}^{\mathbf{p}_{l}}$ with coefficients $a_{l} \in \mathbb{R}$, multi-indices $\mathbf{p}_{l} \in \mathbb{Z}_{+}^{N}$ and a finite number $L \in \mathbb{N}$, is valid for any $\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0})$ with $\mathbf{x}_{0} \in \mathcal{X}_{S}$. 
This trivial case of a finite order polynomial includes unbiased estimation where $c(\mathbf{x}) \equiv 0$. We note 
also that except for the unbiased case, estimators with a bias function $b(\hat{g}(\cdot),\mathbf{x})$ that is a finite order polynomial are in general undesirable for the SLM. This 
is due the bias variance tradeoff \eqref{equ_bias_var_decomp} which implies that if the bias of an estimator is unbounded (which can be the case for a finite order polynomial) also the MSE of this estimator is unbounded. 

By definition of a valid bias function, we have trivially that any given finite variance estimator induces a valid bias function: 
\begin{lemma}
Consider an estimator $\hat{x}_{k}(\mathbf{y})$ for the LGM $\mathcal{E}_{\text{\tiny{LGM}}}$ that has finite variance everywhere, i.e., $v(\hat{x}_{k}(\cdot); \mathbf{x}) < \infty$ for every $\mathbf{x} \in \mathbb{R}^{N}$. 
Then the bias function $c(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}: c(\mathbf{x}) = b(\hat{x}_{k}(\cdot); \mathbf{x})$ is valid for $\mathcal{M}_{\text{\tiny{SLM}}}(\mathbf{x}_{0})$ (where $\sigma$, $M$, $N$ and $\mathbf{H}$ are the same as for $\mathcal{E}_{\text{\tiny{LGM}}}$) with arbitrary $\mathbf{x}_{0} \in \mathcal{X}_{S}$.
\end{lemma}
%Based on Theorem \ref{thm_RKHS_LGM_indep_x_0} one can prove ????
%\begin{theorem}
%Consider the estimation problem $\mathcal{E}_{\text{\tiny{LGM}}}$ for the LGM and a given prescribed bias function $c(\cdot)$. 
%If there exists any $\mathbf{x}_{0} \in \mathbb{R}^{N}$ such that the bias function $c(\cdot)$ is valid for the minimum variance problem $\mathcal{M}_{\mathbf{x}_{0}} =...$ then 
%the bias function is valid for every minimum variance problem $\mathcal{M} = ...$ with $\mathbf{x}'_{0} \in \mathbb{R}^{N}$.  
%\end{theorem} 



\section{Lower Bounds on Estimator Variance for the SLM}
\label{sec_RKHS_Lower_Bounds_SLM}
In this section we will derive lower bounds for the minimum achievable variance $L_{\mathcal{M}_{\text{\tiny{SLM}}}}$ where 
the parameters $\sigma$, $S$, $M$, $N$, $\mathbf{H}$, $c(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}$, and 
$\mathbf{x}_{0} \in \mathcal{X}_{S}$ of the minimum variance problem $\mathcal{M}_{\text{\tiny{SLM}}}=\left( \mathcal{E}_{\text{\tiny{SLM}}},c(\cdot),\mathbf{x}_{0}\right)$ are assumed arbitrary but fixed. 
Furthermore, we will assume from now on that the prescribed bias function $c(\cdot)$ is valid. This is no real restriction since the lower bounds that will be derived are 
finite and therefore trivially apply also formally if $c(\cdot)$ is not valid, in which case $L_{\mathcal{M}_{\text{\tiny{SLM}}}}=\infty$ per definition (cf. Definition \ref{def_min_ach_var}). 

The various bounds that will be presented are similar in that they are based on a projection of the 
prescribed mean function $\gamma(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}: \gamma(\mathbf{x}) \triangleq c(\mathbf{x}) + x_{k}$ 
(which satisfies $\gamma(\cdot) \in \mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}})$ if $c(\cdot)$ is valid) on 
an arbitrary subspace $\mathcal{U}$ of the RKHS $\mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}})$. Indeed (as already discussed after Theorem \ref{thm_main_facts_RKHS_MVE}), by Theorem \ref{thm_main_facts_RKHS_MVE} and Theorem \ref{thm_orthog_proj_ineq} we have 
for an arbitrary subspace $\mathcal{U} \subseteq \mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}})$ the bound 
\begin{equation}
L_{\mathcal{M}_{\text{\tiny{SLM}}}} = \| \gamma(\cdot) \|^{2}_{\mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}})} - \left( \gamma(\mathbf{x}_{0}) \right)^{2} \geq 
\| \mathcal{P}_{\mathcal{U}} \gamma(\cdot) \|^{2}_{\mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}})} - \left( \gamma(\mathbf{x}_{0}) \right)^{2}.
\end{equation}
%where $\gamma(\mathbf{x}) \triangleq c(\mathbf{x}) + x_{k}$ denotes the prescribed mean function of $\mathcal{M}_{\text{\tiny{SLM}}}$. 

The first bound is based on a generalization of the CRB and has already been presented in \cite{ZvikaCRB}:
\begin{theorem}
\label{thm_CRB_SLM}
If the prescribed bias $c(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}$ is such that the partial derivatives $\frac{\partial c(\mathbf{x})}{\partial x_{l}} \big|_{\mathbf{x} = \mathbf{x}_{0}}$ exist for $l \in [N]$ 
then we have 
\begin{align} 
& L_{\mathcal{M}_{\text{\tiny{SLM}}}} \geq \sigma^{2} \mathbf{b}^{T} \left( \mathbf{H}^{T} \mathbf{H} \right)^{\dagger} \mathbf{b} & \mbox{when}\,\, \| \mathbf{x}_{0} \|_{0} < S \label{equ_CRB_SLM_not_full_sparsity} \\Ê
& L_{\mathcal{M}_{\text{\tiny{SLM}}}} \geq  \sigma^{2}\mathbf{b}_{\mathbf{x}_{0}}^{T} \left( \mathbf{H}_{\mathbf{x}_{0}}^{T} \mathbf{H}_{\mathbf{x}_{0}} \right)^{\dagger} \mathbf{b}_{\mathbf{x}_{0}} & \mbox{when}\,\, \| \mathbf{x}_{0} \|_{0} = S \label{equ_CRB_SLM_full_sparsity} 
\end{align} 
where $\mathbf{b} \in \mathbb{R}^{N}$ is defined element-wise by $b_{l} \triangleq  \delta_{k,l} + \frac{\partial c(\mathbf{x})}{\partial x_{l}} \big|_{\mathbf{x} = \mathbf{x}_{0}}$ and 
$\mathbf{b}_{\mathbf{x}_{0}} \in \mathbb{R}^{S}$, $\mathbf{H}_{\mathbf{x}_{0}} \in \mathbb{R}^{M \times S}$ denote the restrictions to the entries and columns of $\mathbf{b}$ and $\mathbf{H}$ respectively, which are indexed by $\supp(\mathbf{x}_{0})$. 
\end{theorem} 
\begin{proof}
Since $c(\cdot)$ is assumed valid, we have by Theorem \ref{thm_main_facts_RKHS_MVE} that the prescribed mean function $\gamma(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}: \gamma(\mathbf{x}) = c(\mathbf{x}) + x_{k}$ 
belongs to the RKHS $\mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}})$. 

For the case $\| \mathbf{x}_{0} \|_{0} < S$ consider the subspace $\mathcal{U}_{1} \triangleq \linspan \{ v_{0}(\cdot) \cup \{ v_{l}(\cdot) \}_{l \in [N]}Ê\}$ 
spanned by the functions $v_{0} (\cdot) \triangleq R_{\mathcal{M}_{\text{\tiny{SLM}}}} (\cdot, \mathbf{x}_{0})$ and 
\begin{equation}
v_{l}(\cdot) \triangleq \frac{ \partial^{\mathbf{e}_{l}} R_{\mathcal{M}_{\text{\tiny{SLM}}}} (\cdot, \mathbf{x}_{2})}  {\partial \mathbf{x}_{2}^{\mathbf{e}_{l}}} \bigg|_{\mathbf{x}_{2} = \mathbf{x}_{0}} 
\end{equation} 
for $l \in [N]$. 
We have trivially $v_{0}(\cdot) \in \mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}})$ and by Theorem \ref{thm_der_repr_prop} we have also that $v_{l} (\cdot)  \in \mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}})$ for $l \in [N]$. 
In a completely analogous manner as the RKHS based derivation of Theorem \ref{thm_unconstr_CR} one can show that 
$\langle v_{0}(\cdot), v_{l} (\cdot) \rangle_{ \mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}})} = 0$ for $l \in [N]$,  
$\langle v_{l}(\cdot), v_{l'}(\cdot) \rangle_{ \mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}})} = \sigma^{2} \left( \mathbf{H}^{T} \mathbf{H} \right)_{l,l'}$ for $l,l' \in [N]$ 
and $\langle  v_{l}(\cdot), \gamma(\cdot) \rangle_{ \mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}})} = b_{l}$ for $l \in [N]$. 
The bound \eqref{equ_CRB_SLM_not_full_sparsity} is then obtained via Theorem \ref{thm_main_facts_RKHS_MVE} and Theorem \ref{thm_norm_projection_finite_dim_subspace} 
by projecting $\gamma(\cdot)$ on the subspace $\mathcal{U}_{1}$. 

In an almost identical manner one can prove the bound \eqref{equ_CRB_SLM_full_sparsity} for the case $\| \mathbf{x}_{0} \|_{0} = S$. Indeed, the only difference is that 
instead of using the subspace $\mathcal{U}_{1}$ one has to use the subspace $\mathcal{U}_{2} \triangleq \linspan \{ v_{0}(\cdot) \cup \{ v_{l}(\cdot) \}_{l \in \supp(\mathbf{x}_{0})}Ê\}$.
\end{proof} 
The formulation of the bound in \cite{ZvikaCRB} slightly differs from Theorem \ref{thm_CRB_SLM} in that the authors of \cite{ZvikaCRB} present 
a bound on the variance $v(\hat{\mathbf{x}}(\cdot); \mathbf{x}_{0})$ of a vector-valued estimator that estimates $\mathbf{x}$ itself and not only the $k$th coefficient $x_{k}$ as we consider. 
However, according to Section \ref{sec_sep_vector_scalar_param_function}, by adding the bound in Theorem \ref{thm_CRB_SLM} over the minimum variance problems $\mathcal{M}_{\text{\tiny{SLM}}}$ 
with varying index $k$ in \eqref{equ_def_SLM_est_problem}, one obtains exactly the same bound as presented in \cite{ZvikaCRB}.

We note two important aspects of Theorem \ref{thm_CRB_SLM}: 
First, if the matrix $\mathbf{H}$ has full column rank, i.e, $\rank(\mathbf{H}) = N$, and we consider unbiased estimation, i.e., $c(\cdot) \equiv 0$, then we have that the bound in \eqref{equ_CRB_SLM_not_full_sparsity} 
coincides with the variance of the well known least-squares (LS) estimator \cite{kay,scharf91} given as 
\begin{equation}
\label{equ_def_ord_LS_est}
\hat{x}_{k,\text{\tiny{LS}}} (\mathbf{y}) \triangleq \mathbf{e}_{k}^{T} (\mathbf{H}^{T} \mathbf{H})^{-1} \mathbf{H}^{T} \mathbf{y}, 
\end{equation}
which implies that in this case the inequality in \eqref{equ_CRB_SLM_not_full_sparsity} becomes an equality, i.e., $L_{\mathcal{M}_{\text{\tiny{SLM}}}} = \sigma^{2} \mathbf{b}^{T} \left( \mathbf{H}^{T} \mathbf{H} \right)^{\dagger} \mathbf{b}$.
Indeed, a straightforward calculation reveals that $\hat{x}_{k,\text{\tiny{LS}}}(\cdot)$ is unbiased and has variance 
\begin{equation} 
\label{equ_var_ord_LS_est}
v(\hat{x}_{k,\text{\tiny{LS}}}(\cdot); \mathbf{x}_{0})= \sigma^{2} \mathbf{e}_{k}^{T} \left( \mathbf{H}^{T} \mathbf{H} \right)^{\dagger} \mathbf{e}_{k} =\sigma^{2} \mathbf{e}_{k}^{T} \left( \mathbf{H}^{T} \mathbf{H} \right)^{-1} \mathbf{e}_{k}
\end{equation} 
where the last equality follows from $\rank(\mathbf{H}) = N$. Thus we have that under these conditions the LS estimator is the LMVU for the SLM at every parameter vector $\mathbf{x}_{0} \in \mathcal{X}_{S}$ with 
$\| \mathbf{x}_{0} \|_{0} < S$.
Since (by Theorem \ref{thm_uniqueness_LMV}) it is the unique LMVU for $\mathbf{x}_{0}$ with $\|\mathbf{x}_{0}\|_{0} < S$, we have that if a UMVU would exists it necessarily would be the ordinary LS estimator $\hat{x}_{k,LS}(\cdot)$ which does 
not exploit the sparsity assumptions encoded by the parameter set $\mathcal{X}_{S}$ and which has the constant variance \eqref{equ_var_ord_LS_est} for every $\mathbf{x} \in \mathcal{X}_{S}$. 
However, as already shown in \cite{AlexZvikaICASSP,AlexZvikaJournal} and discussed in Section \ref{sec_SSNM}, there does not exist a UMVU estimator for the SLM in the general case. 

A second important aspect of Theorem \ref{thm_CRB_SLM} is that the lower bound given by \eqref{equ_CRB_SLM_not_full_sparsity} and \eqref{equ_CRB_SLM_full_sparsity} is not a continuos function of $\mathbf{x}_{0}$ in general.
Indeed, for the case $\mathbf{H}=\mathbf{I}$ and $c(\cdot) Ê\equiv 0$ considered in \cite{AlexZvikaICASSP,AlexZvikaJournal} it can be verified that the bound given by \eqref{equ_CRB_SLM_not_full_sparsity} and \eqref{equ_CRB_SLM_full_sparsity} 
is a strictly upper semi-continuous function $\mathbf{x}_{0}$. 
Consider e.g. $\mathcal{M}_{\text{\tiny{SLM}}}=\left( \mathcal{E}_{\text{\tiny{SLM}}},c(\cdot),\mathbf{x}_{0}\right)$ with $\mathbf{H} = \mathbf{I}$, $S=1$, $M=N=2$, $k=2$, $c(\cdot)Ê\equiv 0$ and 
a parameter vector $\mathbf{x}_{0}$ of the form $\mathbf{x}_{0} = c (1,0)^{T}$ where $c \geq 0$. The corresponding bound 
given by Theorem \ref{thm_CRB_SLM} is equal to $0$ for all $c>0$ and equals $1$ for $c=0$.
However, since by Theorem \ref{thm_SLM_min_achiev_var_lower_semi_cont} the minimum achievable variance $L_{\mathcal{M}_{\text{\tiny{SLM}}}}$ has to be a lower-semicontinuous function of $\mathbf{x}_{0}$, we have 
that the bound in Theorem \ref{thm_CRB_SLM} cannot be tight, i.e., we have a strict inequality in \eqref{equ_CRB_SLM_not_full_sparsity} or \eqref{equ_CRB_SLM_full_sparsity} in general. 

While the bound in Theorem \ref{thm_CRB_SLM} was based on a generalization of the CRB (cf. Section \ref{sec_CRB}), the authors of \cite{AlexZvikaICASSP} present a lower bound on 
$L_{\mathcal{M}_{\text{\tiny{SLM}}}}$ for $\mathbf{H}=\mathbf{I}$ and $c(\cdot) \equiv 0$ that is 
based on a generalization of the HCRB (cf. Section \ref{sec_HCRB}):
\begin{theorem}
\label{thm_HCRB_SLM}
Consider the minimum variance problem $\mathcal{M}_{\text{\tiny{SLM}}}=\left( \mathcal{E}_{\text{\tiny{SLM}}},c(\cdot),\mathbf{x}_{0}\right)$ with $\mathbf{H} = \mathbf{I}$ and $c(\cdot) \equiv 0$. 
Then we have the bound  
\begin{align} 
 \label{equ_HCRB_SLM_not_full_sparsity}  & L_{\mathcal{M}_{\text{\tiny{SLM}}}} \geq \sigma^{2} & \mbox{when}\,\, |\supp(\mathbf{x}_{0}) \cup \{k\} | < S+1  \\Ê
 \label{equ_HCRB_SLM_full_sparsity} & L_{\mathcal{M}_{\text{\tiny{SLM}}}} \geq \sigma^{2} \frac{N-S-1}{N-S}   \exp \left(-\xi_{0}^{2}/ \sigma^{2} \right) 			& \mbox{when}\,\, |\supp(\mathbf{x}_{0}) \cup \{k\} | = S+1
\end{align} 
where $\xi_{0}$ denotes the value of the $S$-largest (in magnitude) entry of $\mathbf{x}_{0}$. 
\end{theorem} 
\begin{proof}
The bias function $c(\cdot) \equiv 0$ is assumed to be valid, i.e., the mean function $\gamma(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}: \gamma(\mathbf{x}) = x_{k}$ belongs to $\mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}})$. 
%The bound \eqref{equ_HCRB_SLM_not_full_sparsity} for the case $\|\mathbf{x}_{0} \|_{0} < S$ coincides with the bound \eqref{equ_HCRB_SLM_not_full_sparsity} when 
%Theorem \ref{thm_CRB_SLM} is applied to the special case with $\mathbf{H}=\mathbf{I}$ and $c(\cdot)$.

First consider the case where $|\supp(\mathbf{x}_{0}) \cup \{k\} | = S+1$ (which can only occur if $N > S$). 
In order to show \eqref{equ_HCRB_SLM_full_sparsity} we denote by $j_{0}$ and $\xi_{0}$ respectively the index and value of the $S$-largest (in magnitude) entry of $\mathbf{x}_{0}$. 
We then introduce the subspace 
$\mathcal{U}_{1}^{(t)} \triangleq \linspan \{ v_{0}(\cdot) \cup \{ v^{(t)}_{l}(\cdot) \}_{l \in [N]}Ê\}$ which is parametrized by $t \in \mathbb{R}$ and spanned by the vectors 
$v_{0}(\cdot) \triangleq R_{\mathcal{M}_{\text{\tiny{SLM}}}} (\cdot, \mathbf{x}_{0})$, $v_{l}^{(t)}(\cdot) \triangleq R_{\mathcal{M}_{\text{\tiny{SLM}}}} (\cdot, \mathbf{x}_{0}-\mathbf{e}_{j}\xi_{0}+t\mathbf{e}_{l})-R_{\mathcal{M}_{\text{\tiny{SLM}}}} (\cdot, \mathbf{x}_{0})$ for $l \in [N] \setminus \supp(\mathbf{x}_{0})$ and 
$v_{l}^{(t)}(\cdot) \triangleq R_{\mathcal{M}_{\text{\tiny{SLM}}}} (\cdot, \mathbf{x}_{0}+t\mathbf{e}_{l})-R_{\mathcal{M}_{\text{\tiny{SLM}}}} (\cdot, \mathbf{x}_{0})$ for $l \in \supp(\mathbf{x}_{0})$. 
Similarly to the RKHS based derivation of the HCRB in Theorem \ref{thm_HCRB} one can show by a projection of the mean function $\gamma(\cdot) \in \mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}})$ on the subspace $\mathcal{U}^{(t)}$ that 
\begin{equation}
\label{equ_derivation_SLM_HCRB_bound_1}
L_{\mathcal{M}_{\text{\tiny{SLM}}}} \geq  t^2 \mathbf{e}_{k}^{T} \mathbf{V}^{\dagger} \mathbf{e}_{k}
\end{equation} 
where $\mathbf{V} \in \mathbb{R}^{N \times N}$ is defined element-wise as 
\begin{align} 
\left(\mathbf{V} \right)_{m,n} & \triangleq \langle v^{(t)}_{m}(\cdot), v^{(t)}_{n}(\cdot) \rangle_{\mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}})}  = \nonumber \\Ê
& \hspace*{-10mm}  R_{\mathcal{M}_{\text{\tiny{SLM}}}} (\mathbf{x}_{0}+t\mathbf{e}_{m}, \mathbf{x}_{0}+t\mathbf{e}_{n}) 
- R_{\mathcal{M}_{\text{\tiny{SLM}}}} (\mathbf{x}_{0}, \mathbf{x}_{0}+t\mathbf{e}_{m}) - R_{\mathcal{M}_{\text{\tiny{SLM}}}} (\mathbf{x}_{0}+t\mathbf{e}_{n}, \mathbf{x}_{0}) + 
R_{\mathcal{M}_{\text{\tiny{SLM}}}} (\mathbf{x}_{0}, \mathbf{x}_{0})  \nonumber \\Ê
& = \exp( t^{2} \mathbf{e}_{n}^{T}\mathbf{e}_{m}/ \sigma^{2}) - 1 -1 + 1 = \delta_{m,n} \exp(t^{2}/\sigma^{2}) -1 .
\end{align}  
As shown in \cite{AlexZvikaJournal} the bound in \eqref{equ_HCRB_SLM_full_sparsity} is obtained from \eqref{equ_derivation_SLM_HCRB_bound_1} as the limit $\lim_{t \rightarrow 0} t^2 \mathbf{e}_{k}^{T} \mathbf{V}^{\dagger} \mathbf{e}_{k}$. 

Now we consider the remaining case where $|\supp(\mathbf{x}_{0}) \cup \{k\} | < S+1$.
In an analogous manner as before except of using the subspace $\mathcal{U}_{2}^{(t)} \triangleq \{ v_{0}(\cdot), v^{(t)}(\cdot) Ê\}$ instead of $\mathcal{U}_{1}^{(t)}$, 
where $v^{(t)}(\cdot) \triangleq R_{\mathcal{M}_{\text{\tiny{SLM}}}} (\cdot, \mathbf{x}_{0}+t\mathbf{e}_{k})-R_{\mathcal{M}_{\text{\tiny{SLM}}}} (\cdot, \mathbf{x}_{0})$,
one obtains 
\begin{equation}
\label{equ_derivation_SLM_HCRB_bound_2}
L_{\mathcal{M}_{\text{\tiny{SLM}}}} \geq t^2 \|v^{(t)}(\cdot) \|^{-2}_{\mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}})}.
\end{equation} 
Since the squared norm of $v^{(t)}(\cdot)$ can be calculated as 
\begin{align}
 \|v^{(t)}(\cdot) \|^{2}_{\mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}})} & = 
\langle v^{(t)}(\cdot), v^{(t)}(\cdot) \rangle_{\mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}})}  = \nonumber \\Ê
& \hspace*{-30mm}  R_{\mathcal{M}_{\text{\tiny{SLM}}}} (\mathbf{x}_{0}+t\mathbf{e}_{k}, \mathbf{x}_{0}+t\mathbf{e}_{k}) 
- R_{\mathcal{M}_{\text{\tiny{SLM}}}} (\mathbf{x}_{0}, \mathbf{x}_{0}+t\mathbf{e}_{k}) - R_{\mathcal{M}_{\text{\tiny{SLM}}}} (\mathbf{x}_{0}+t\mathbf{e}_{k}, \mathbf{x}_{0}) + 
R_{\mathcal{M}_{\text{\tiny{SLM}}}} (\mathbf{x}_{0}, \mathbf{x}_{0})  \nonumber \\Ê
& = \exp( t^{2} \mathbf{e}_{k}^{T}\mathbf{e}_{k}/ \sigma^{2}) - 1 - 1 + 1 =  \exp(t^{2}/\sigma^{2}) -1,
\end{align} 
one straightforwardly obtains the bound $L_{\mathcal{M}_{\text{\tiny{SLM}}}} \geq \sigma^{2}$ from \eqref{equ_derivation_SLM_HCRB_bound_2} by the limit $\lim_{t \rightarrow 0}   t^2/(\exp(t^{2}/ \sigma^{2}) -1)$.
Since the variance of the specific unbiased estimator $\hat{g}(\mathbf{y}) = y_{k}$ for the SLM is equal to $\sigma^{2}$, we have that $L_{\mathcal{M}_{\text{\tiny{SLM}}}} = \sigma^{2}$. 
%Similarly, for $k \in \supp(\mathbf{x}_{0})$ and $\| \mathbf{x}_{0} \|_{0} = S$ the bound \eqref{equ_HCRB_SLM_not_full_sparsity} is obtained by using the subspace 
%$\mathcal{U}_{2}^{(t)} \triangleq \{ v_{0} \cup \{ v^{(t)}_{l} \}_{l \in [N]}Ê\}$
\end{proof} 
The bound given in Theorem \ref{thm_HCRB_SLM} has been presented in a slightly different in \cite{AlexZvikaICASSP,AlexZvikaJournal} where 
a lower bound on the variance $v(\hat{\mathbf{x}}(\cdot), \mathbf{x}_{0})$ of an unbiased estimator of the parameter vector $\mathbf{x}$ itself, instead of the single coefficient $x_{k}$, has been derived.\footnote{More precisely, 
a lower bound on the MSE of any unbiased estimator was presented in \cite{AlexZvikaICASSP,AlexZvikaJournal}. However, the variance of an unbiased estimator is always equal to its MSE.}
As discussed in Section \ref{sec_sep_vector_scalar_param_function} we have that minimum variance estimation of the parameter vector is equivalent to separate minimum variance estimation of the coefficients $x_{k}$.
In particular, the bound given in \cite{AlexZvikaICASSP,AlexZvikaJournal} is obtained by summing the bound in Theorem \ref{thm_HCRB_SLM} over all minimum variance problems $\mathcal{M}_{\text{\tiny{SLM}}}$ 
that are obtained for a specific $k \in [N]$ in \eqref{equ_def_SLM_est_problem}.


While in general the bound in Theorem \ref{thm_HCRB_SLM} is tighter, i.e. higher, than the bound of Theorem \ref{thm_CRB_SLM} (when specialized to $c(\cdot) \equiv 0$ and $\mathbf{H} = \mathbf{I}$) it 
is again upper semi-continuous which implies by Theorem \ref{thm_SLM_min_achiev_var_lower_semi_cont} that it cannot be tight, i.e., we have a strict inequality in \eqref{equ_HCRB_SLM_full_sparsity} in general. However, for 
the case $\| \mathbf{x}_{0} \|_{0} < S$ or $k \in \supp(\mathbf{x}_{0})$, $\| \mathbf{x}_{0} \|_{0} = S$ the bound in \eqref{equ_HCRB_SLM_not_full_sparsity} is tight since as already mentioned above, 
it is achieved by the ordinary LS estimator $\hat{x}_{k,\text{\tiny{LS}}}(\mathbf{y}) = y_{k}$.

An improved lower bound on $L_{\mathcal{M}_{\text{\tiny{SLM}}}}$ has been presented in \cite{RKHSAsilomar2010}: 
\begin{theorem} 
\label{thm_bound_asilomar}
Consider the minimum variance problem $\mathcal{M}_{\text{\tiny{SLM}}}=\left( \mathcal{E}_{\text{\tiny{SLM}}},c(\cdot),\mathbf{x}_{0}\right)$ with a system matrix $\mathbf{H} \in \mathbb{R}^{M \times N}$ satisfying \eqref{equ_spark_cond} 
and with prescribed mean function $\gamma(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}: \gamma(\mathbf{x}) = c(\mathbf{x}) + x_{k}$. 
We assume that the prescribed bias function $c(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}$ is such that the partial derivatives $\frac{ \partial^{\mathbf{e}_{l}} c(\mathbf{x})}{\partial \mathbf{x}^{\mathbf{e}_{l}}}$ exist for any $l \in [N]$. 
Then we have for an arbitrary set $\mathcal{K} =\{i_1,\ldots,i_{|\mathcal{K}|} \} \subseteq [N]$ consisting of no more than $S$ different indices, i.e., $|\mathcal{K}| \leq S$, the bound
\begin{equation} 
\label{equ_bound_asilomar_1}
L_{\mathcal{M}_{\text{\tiny{SLM}}}} \geq  \exp\left( - \frac{1}{\sigma^{2}}\| (\mathbf{I} - \mathbf{P}_{\mathcal{K}}) \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} \right) \left( \sigma^{2} \mathbf{r}_{\mathbf{x}_{0}}^{T} \left( \mathbf{H}_{\mathcal{K}}^{T} \mathbf{H}_{\mathcal{K}} \right)^{-1} \mathbf{r}_{\mathbf{x}_{0}} + \gamma^{2}(\widetilde{\mathbf{x}}_{0}) \right) - \gamma^{2}(\mathbf{x}_{0}). 
\end{equation} 
where $\mathbf{P}_{\mathcal{K}} \triangleq \mathbf{H}_{\mathcal{K}} \mathbf{H}_{\mathcal{K}}^{\dagger}$, the vector $\mathbf{r}_{\mathbf{x}_{0}} \in \mathbb{R}^{|\mathcal{K}|}$ is defined element-wise as $r_{\mathbf{x}_{0},l} \triangleq \frac{ \partial^{\mathbf{e}_{i_{l}}} \gamma(\mathbf{x})}{\partial \mathbf{x}^{\mathbf{e}_{i_{l}}}} \big|_{\mathbf{x} = \widetilde{\mathbf{x}}_{0}}$  and $\widetilde{\mathbf{x}}_{0} \in \mathbb{R}^{N}$ is defined as the unique (due to \eqref{equ_spark_cond}) 
vector with $\supp(\widetilde{\mathbf{x}}_{0})=\mathcal{K}$ that solves 
\begin{equation} 
\label{equ_def_x_0_tilde_asiloamr_bound_1}
\mathbf{H} \widetilde{\mathbf{x}}_{0} = \mathbf{H}_{\mathcal{K}} \mathbf{H}_{\mathcal{K}}^{\dagger} \mathbf{H} \mathbf{x}_{0}. 
\end{equation} 
\end{theorem}
\begin{proof}
First we note that since $\mathbf{H}$ is assumed to satisfy \eqref{equ_spark_cond}, the matrix $\mathbf{H}_{\mathcal{K}} \in \mathbb{R}^{M \times |\mathcal{K}|}$ has full column rank which implies that 
$\mathbf{H}_{\mathcal{K}}^{\dagger} = (\mathbf{H}_{\mathcal{K}}^{T} \mathbf{H}_{\mathcal{K}})^{-1} \mathbf{H}_{\mathcal{K}}^{T}$ \cite{golub96}. Thus, 
\begin{align}
\label{equ_proof_lower_bound_asilomar_relation_1}
\mathbf{H}_{\mathcal{K}}^{T} \mathbf{H} (\widetilde{\mathbf{x}}_{0} - \mathbf{x}_{0}) & = \mathbf{H}_{\mathcal{K}}^{T}( \mathbf{H}_{\mathcal{K}} \mathbf{H}_{\mathcal{K}}^{\dagger} \mathbf{H} \mathbf{x}_{0} - \mathbf{H}\mathbf{x}_{0})   = \mathbf{H}_{\mathcal{K}}^{T}\mathbf{H}_{\mathcal{K}} \mathbf{H}_{\mathcal{K}}^{\dagger} \mathbf{H} \mathbf{x}_{0} - \mathbf{H}_{\mathcal{K}}^{T}\mathbf{H} \mathbf{x}_{0} \nonumber \\Ê
&=  \mathbf{H}_{\mathcal{K}}^{T}\mathbf{H}_{\mathcal{K}}(\mathbf{H}_{\mathcal{K}}^{T} \mathbf{H}_{\mathcal{K}})^{-1} \mathbf{H}_{\mathcal{K}}^{T} \mathbf{H} \mathbf{x}_{0} - \mathbf{H}_{\mathcal{K}}^{T}\mathbf{H} \mathbf{x}_{0} =   \mathbf{H}_{\mathcal{K}}^{T} \mathbf{H} \mathbf{x}_{0} - \mathbf{H}_{\mathcal{K}}^{T}\mathbf{H} \mathbf{x}_{0} = \mathbf{0}, 
\end{align} 
which implies in turn that $\linspan(\mathbf{H}_{\mathcal{K}})$ is orthogonal to $\mathbf{H} (\widetilde{\mathbf{x}}_{0} - \mathbf{x}_{0})$. 
%$R_{\mathcal{M}_{\text{\tiny{SLM}}}}$ in \eqref{equ_kernel_SLM} as follows 
%\begin{align}
% \label{equ_kernel_SLM_rewritten_asilomar_1}
%R_{\mathcal{M}_{\text{\tiny{SLM}}}}(\mathbf{x}_{1}, \mathbf{x}_{2})  &  =  \exp   \left(  (\mathbf{x}_{1} - \mathbf{x}_{0})^{T}\mathbf{H}^{T} \mathbf{H} (\mathbf{x}_{2} - \mathbf{x}_{0}) \right) \nonumber \\Ê
%& =  \exp   \left(  ( \mathbf{x}^{\mathcal{K}}_{1} - \mathbf{x}^{\mathcal{K}}_{0})^{T}\mathbf{H}^{T} \mathbf{H} (\mathbf{x}^{\mathcal{K}}_{2} - \mathbf{x}^{\mathcal{K}}_{0}) \right) \exp   \left(  ( \mathbf{x}^{[N] \setminus \mathcal{K}}_{1} - \mathbf{x}^{\mathcal{K}}_{0})^{T}\mathbf{H}^{T} \mathbf{H} (\mathbf{x}^{[N] \setminus \mathcal{K}}_{2} - \mathbf{x}^{\mathcal{K}}_{0}) \right) . 
%\end{align} 

Let us then consider the subspace 
\begin{equation} 
\label{equ_proof_lower_bound_asilomar_def_subspace}
\mathcal{U}_{4} \triangleq \linspan \{ v_{0} (\cdot) \cup \{ v_{l}(\cdot) \}_{l \in \mathcal{K}}Ê\}
\end{equation}
spanned by the functions $v_{0}(\cdot) \triangleq R_{\mathcal{M}_{\text{\tiny{SLM}}}}(\cdot, \widetilde{\mathbf{x}}_{0})$ and 
$v_{l}(\cdot) \triangleq \frac{\partial^{\mathbf{e}_{l}}R_{\mathcal{M}_{\text{\tiny{SLM}}}}(\cdot, \mathbf{x}_{2})}{\partial \mathbf{x}_{2}^{\mathbf{e}_{l}}}Ê\big|_{\mathbf{x}_{2} = \widetilde{\mathbf{x}}_{0}}$, which by Theorem \ref{thm_der_repr_prop} belong to the RKHS $\mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}})$.
The inner-product between any $v_{l}(\cdot)$ with $l \in \mathcal{K}$ and $v_{0}(\cdot)$ is given due to Theorem \ref{thm_der_repr_prop} by 
\begin{align} 
\label{equ_proof_lower_bound_asilomar_orthog_vecs_1}
\langle v_{0}(\cdot) , v_{l}(\cdot) \rangle_{\mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}})} & = \frac{\partial R_{\mathcal{M}_{\text{\tiny{SLM}}}}(\mathbf{x}_{1},\mathbf{x}_{2})}{\partial x_{2,l}} \bigg|_{\mathbf{x}_{1} = \mathbf{x}_{2} = \widetilde{\mathbf{x}}_{0}}  \nonumber \\
 & = \frac{1}{\sigma^{2}} ( \widetilde{\mathbf{x}}_{0} - \mathbf{x}_{0})^{T} \mathbf{H}^{T} \mathbf{H} \mathbf{e}_{l} \exp\left( \frac{1}{\sigma^{2}} ( \widetilde{\mathbf{x}}_{0} - \mathbf{x}_{0})^{T} \mathbf{H}^{T} \mathbf{H} ( \widetilde{\mathbf{x}}_{0} - \mathbf{x}_{0}) \right) \stackrel{(a)}{=} 0
\end{align} 
where $(a)$ follows from the fact that $\mathbf{H} \mathbf{e}_{l}  \in \linspan(\mathbf{H}_{\mathcal{K}})$ and therefore, as shown by \eqref{equ_proof_lower_bound_asilomar_relation_1}, has to be orthogonal to $\mathbf{H} (\widetilde{\mathbf{x}}_{0} - \mathbf{x}_{0})$, i.e., 
$( \widetilde{\mathbf{x}}_{0} - \mathbf{x}_{0})^{T} \mathbf{H}^{T} \mathbf{H} \mathbf{e}_{l} =0$.
Now, we define the matrix $\mathbf{V}Ê\in \mathbb{R}^{|\mathcal{K}| \times |\mathcal{K}| }$ element-wise via
\begin{align} 
\label{equ_proof_lower_bound_asilomar_grammian}
\left( \mathbf{V} \right)_{m,n} & \triangleq \langle v_{i_m}(\cdot) , v_{i_n}(\cdot) \rangle_{\mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}})}  \stackrel{(a)}{=} \frac{\partial R_{\mathcal{M}_{\text{\tiny{SLM}}}}(\mathbf{x}_{1},\mathbf{x}_{2})}{\partial x_{1,i_n} \partial x_{2,i_m}} \bigg|_{\mathbf{x}_{1} = \mathbf{x}_{2} = \widetilde{\mathbf{x}}_{0}} \nonumber \\
&= \frac{1}{\sigma^{2}} \frac{\partial (\mathbf{x}_{1}- \mathbf{x}_{0})^{T} \mathbf{H}^{T} \mathbf{H} \mathbf{e}_{i_{m}} \exp \left( \frac{1}{\sigma^{2}} (\mathbf{x}_{1} - \mathbf{x}_{0})^{T} \mathbf{H}^{T} \mathbf{H} (\widetilde{\mathbf{x}}_{0} - \mathbf{x}_{0}) \right)}{\partial x_{1,i_n}} \bigg|_{\mathbf{x}_{1} = \widetilde{\mathbf{x}}_{0}} \nonumber \\ 
& =  \frac{1}{\sigma^{2}} \mathbf{e}_{i_n}^{T} \mathbf{H}^{T} \mathbf{H} \mathbf{e}_{i_{m}} \exp \left( \frac{1}{\sigma^{2}} (\widetilde{\mathbf{x}}_{0} - \mathbf{x}_{0})^{T} \mathbf{H}^{T} \mathbf{H} (\widetilde{\mathbf{x}}_{0} - \mathbf{x}_{0}) \right) \nonumber \\ 
& + \frac{1}{\sigma^{4}}  \bigg( (\widetilde{\mathbf{x}}_{0}- \mathbf{x}_{0})^{T} \mathbf{H}^{T} \mathbf{H} \mathbf{e}_{i_{m}} \bigg) \mathbf{e}^{T}_{i_{n}}\mathbf{H}^{T} \mathbf{H} (\widetilde{\mathbf{x}}_{0} - \mathbf{x}_{0}) \exp \left( \frac{1}{\sigma^{2}} (\widetilde{\mathbf{x}}_{0}- \mathbf{x}_{0})^{T} \mathbf{H}^{T} \mathbf{H} (\widetilde{\mathbf{x}}_{0} - \mathbf{x}_{0}) \right)
 \nonumber \\ 
& \stackrel{(b)}{=} \frac{1}{\sigma^{2}} \mathbf{e}_{i_n}^{T} \mathbf{H}^{T} \mathbf{H}  \mathbf{e}_{i_{m}} \exp \left( \frac{1}{\sigma^{2}} (\widetilde{\mathbf{x}}_{0} - \mathbf{x}_{0})^{T} \mathbf{H}^{T} \mathbf{H} (\widetilde{\mathbf{x}}_{0} - \mathbf{x}_{0}) \right),
\end{align} 
where $(a)$ follows again from Theorem \ref{thm_der_repr_prop} and $(b)$ follows from the fact that $\mathbf{H} \mathbf{e}_{i_{m}} \! \in \! \linspan(\mathbf{H}_{\mathcal{K}})$ implying via \eqref{equ_proof_lower_bound_asilomar_relation_1} that $(\widetilde{\mathbf{x}}_{0}- \mathbf{x}_{0})^{T} \mathbf{H}^{T} \mathbf{H} \mathbf{e}_{i_{m}}=0$. 
From \eqref{equ_proof_lower_bound_asilomar_grammian} we have by element-wise comparison that 
\begin{equation} 
\mathbf{V} =  \frac{1}{\sigma^{2}} \mathbf{H}_{\mathcal{K}}^{T} \mathbf{H}_{\mathcal{K}} \exp \left( \frac{1}{\sigma^{2}} (\widetilde{\mathbf{x}}_{0} - \mathbf{x}_{0})^{T} \mathbf{H}^{T} \mathbf{H} (\widetilde{\mathbf{x}}_{0} - \mathbf{x}_{0}) \right). \nonumber
\end{equation} 

Since furthermore 
\begin{align} 
(\widetilde{\mathbf{x}}_{0} - \mathbf{x}_{0})^{T} \mathbf{H}^{T} \mathbf{H} (\widetilde{\mathbf{x}}_{0} - \mathbf{x}_{0})& = \| \mathbf{H} (\widetilde{\mathbf{x}}_{0} - \mathbf{x}_{0})\|^{2}_{2}  
 = \| \mathbf{H} \mathbf{x}_{0} - \mathbf{H}_{\mathcal{K}}\mathbf{H}_{\mathcal{K}}^{\dagger} \mathbf{H} \mathbf{x}_{0} \|^{2}_{2}   = \| (\mathbf{I} - \mathbf{H}_{\mathcal{K}}\mathbf{H}_{\mathcal{K}}^{\dagger}) \mathbf{H} \mathbf{x}_{0} \|^{2}_{2}  \nonumber \\ 
& = \| (\mathbf{I} -\mathbf{P}_{\mathcal{K}}) \mathbf{H} \mathbf{x}_{0} \|^{2}_{2}
\end{align} 
the bound in \eqref{equ_bound_asilomar_1} follows from Theorem \ref{thm_main_facts_RKHS_MVE} and Theorem \ref{thm_norm_projection_finite_dim_subspace_union_orthog_subspaces} 
(note that due to \eqref{equ_spark_cond} we have that $\left( \mathbf{H}_{\mathcal{K}}^{T} \mathbf{H}_{\mathcal{K}} \right)^{-1} =\left( \mathbf{H}_{\mathcal{K}}^{T} \mathbf{H}_{\mathcal{K}} \right)^{\dagger}$) 
via \eqref{equ_proof_lower_bound_asilomar_grammian}, \eqref{equ_proof_lower_bound_asilomar_orthog_vecs_1} and 
the inner-products
%\begin{equation}
$\langle v_{0}(\cdot) , \gamma(\cdot) \rangle_{\mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}})}  = \gamma(\widetilde{\mathbf{x}}_{0})$ and 
%\end{equation}
%\begin{equation} 
$\langle v_{l}(\cdot) , \gamma(\cdot) \rangle_{\mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}})} = \frac{ \partial^{\mathbf{e}_{i_{l}}} \gamma(\mathbf{x})}{\partial \mathbf{x}^{\mathbf{e}_{i_{l}}}} \bigg|_{\mathbf{x} = \widetilde{\mathbf{x}}_{0}} =  r_{\mathbf{x}_{0},l}$ (cf. Theorem \ref{thm_der_repr_prop}). 
%\end{equation} 
%Here, we used for the step $(a)$ the definition of the functions $v_{l}(\cdot)$ and the reproducing property \eqref{equ_reproduction_property} and for $(b)$ the definition of the kernel $R_{\mathcal{M}_{\text{\tiny{SLM}}}}$ (cf. \eqref{equ_def_kernel_M}). 
\end{proof}
Note that the matrix $\mathbf{P}_{\mathcal{K}}$ defined in Theorem \ref{thm_bound_asilomar} is an orthogonal projection matrix \cite{golub96} on the subspace $\mathcal{U}_{\mathcal{K}} \triangleq \linspan(\mathbf{H}_{\mathcal{K}}) \subseteq \mathbb{R}^{M}$ 
and correspondingly, $(\mathbf{I} - \mathbf{P}_{\mathcal{K}})$ is a projection matrix on the orthogonal complement \cite{HalmosFiniteDimVecSpace,golub96} of $\mathcal{U}_{\mathcal{K}}$. 
Therefore, the factor $\exp\left( - \frac{1}{\sigma^{2}} \| (\mathbf{I} - \mathbf{P}_{\mathcal{K}}) \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} \right)$ appearing in the  bound \eqref{equ_bound_asilomar_1} can be interpreted as a measure 
of the distance between the point $\mathbf{H} \mathbf{x}_{0}$ and the subspace $\mathcal{U}_{\mathcal{K}}$. In general the bound \eqref{equ_bound_asilomar_1} is tighter, i.e. higher, if $\mathcal{K}$ is chosen such that this distance is small, i.e., $\| (\mathbf{I} - \mathbf{P}_{\mathcal{K}}) \mathbf{H} \mathbf{x}_{0} \|^{2}_{2}$ 
is small. 

One of the appealing properties of the bound in \eqref{equ_bound_asilomar_1} is that it is continuous for the special case $\mathbf{H}=\mathbf{I}$ and $c(\cdot) \equiv 0$, 
irrespective of what index $k$ is chosen for the parameter function in the SLM (cf. \eqref{equ_def_SLM_est_problem}). 
We also have for this specific instance of $\mathcal{M}_{\text{\tiny{SLM}}}$ that the 
bound \eqref{equ_bound_asilomar_1} is tighter, i.e., higher, than the bounds given in Theorem \ref{thm_CRB_SLM} and Theorem \ref{thm_HCRB_SLM}. 

The quantity $\sigma^{2} \mathbf{r}_{\mathbf{x}_{0}}^{T} \left( \mathbf{H}_{\mathcal{K}}^{T} \mathbf{H}_{\mathcal{K}} \right)^{-1} \mathbf{r}_{\mathbf{x}_{0}}$ appearing in the bound \eqref{equ_bound_asilomar_1} 
has a remarkable interpretation as the unconstrained CRB (cf. Section \ref{sec_CRB}) for a minimum variance problem associated with the LGM with $N = |\mathcal{K}|$. 

For $k \in \supp(\mathbf{x}_{0})$, the factor $\exp\left( - \frac{1}{\sigma^{2}} \| (\mathbf{I} - \mathbf{P}_{\mathcal{K}}) \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} \right)$ can be made equal to $1$ by choosing $\mathcal{K} = \supp(\mathbf{x}_{0})$. 
On the other hand, for $k \notin \supp(\mathbf{x}_{0})$ and chosing $\mathcal{K} =\{ \{k\} \cup \mathcal{L} \}$ where $\mathcal{L}$ denotes the indices of the $S-1$ largest (in magnitude) entries of $\mathbf{x}_{0}$, 
the bound \eqref{equ_bound_asilomar_1} indicates a transition from a ``low''-SNR region, where the factor 
$\exp\left( - \frac{1}{\sigma^{2}} \| (\mathbf{I} - \mathbf{P}_{\mathcal{K}}) \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} \right)$ is nearly equal to $1$, to a ``high''-SNR regime where the factor $\exp\left( - \frac{1}{\sigma^{2}} \| (\mathbf{I} - \mathbf{P}_{\mathcal{K}}) \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} \right)$ is nearly $0$. In the low-SNR regime the bound \eqref{equ_bound_asilomar_1} is equal to the CRB of a LGM with $N = |\mathcal{K}|$ while in the 
high-SNR regime the bound becomes approximately equal to $0$ which means that the non-zero entries $x_{k}$ with $k \notin \supp(\mathbf{x})$ can be estimated with small variance in the high SNR regime. 

While in \cite{RKHSAsilomar2010} a complete derivation of the bound \eqref{equ_bound_asilomar_1} is sketched, we present in \cite{RKHSAsilomar2010} not directly the bound \eqref{equ_bound_asilomar_1}, 
but the bound that is obtained by choosing the index set $\mathcal{K}$ for which the right hand side of \eqref{equ_bound_asilomar_1} is largest.
We note also that the derivation of the bound \eqref{equ_bound_asilomar_1} used here is slightly different from those sketched in \cite{RKHSAsilomar2010}. 
However, the derivation presented here seems to be more direct. 

By a slight modification in the derivation of Theorem \ref{thm_bound_asilomar} we obtain 
\begin{theorem} 
\label{thm_bound_asilomar_2}
Consider the minimum variance problem $\mathcal{M}_{\text{\tiny{SLM}}}=\left( \mathcal{E}_{\text{\tiny{SLM}}},c(\cdot),\mathbf{x}_{0}\right)$ with a system matrix $\mathbf{H}$ 
satisfying \eqref{equ_spark_cond} and with prescribed mean function $\gamma(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}: \gamma(\mathbf{x}) = c(\mathbf{x}) + x_{k}$.
We assume that the prescribed bias function $c(\cdot)$ is valid and such that the partial derivatives $\frac{ \partial^{\mathbf{e}_{l}} c(\mathbf{x})}{\partial \mathbf{x}^{\mathbf{e}_{l}}}$ exist for any $l \in [N]$. 

Then we have for an arbitrary set $\mathcal{K} =\{i_1,\ldots,i_{|\mathcal{K}|} \} \subseteq [N]$ consisting of no more than $S$ different indices, i.e., $|\mathcal{K}| \leq S$, the bound
\begin{equation} 
\label{equ_bound_asilomar_2}
L_{\mathcal{M}_{\text{\tiny{SLM}}}} \geq  \exp\left( - \frac{1}{\sigma^{2}} \| (\mathbf{I} - \mathbf{P}_{\mathcal{K}}) \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} \right) \sigma^{2} \mathbf{r}_{\mathbf{x}_{0}}^{T} \left( \mathbf{H}_{\mathcal{K}}^{T} \mathbf{H}_{\mathcal{K}} \right)^{-1} \mathbf{r}_{\mathbf{x}_{0}}. 
\end{equation} 
where $\mathbf{P}_{\mathcal{K}} \in \mathbb{R}^{M \times M}$ and $\mathbf{r}_{\mathbf{x}_{0}} \in \mathbb{R}^{|\mathcal{K}|}$ are defined as in Theorem \ref{thm_bound_asilomar}.
\end{theorem}
\begin{proof}
Use the same derivation as in the proof of Theorem \ref{thm_bound_asilomar} but with subspace $\mathcal{U}_{4}$ in \eqref{equ_proof_lower_bound_asilomar_def_subspace} replaced by 
the subspace 
\begin{equation} 
\mathcal{U}_{5} \triangleq \linspan \{ v_{0} (\cdot) \cup \{ v_{l}(\cdot) \}_{l \in \mathcal{K}}Ê\}
\end{equation}
which is spanned by the functions $v_{0}(\cdot) \triangleq R_{\mathcal{M}_{\text{\tiny{SLM}}}}(\cdot,\mathbf{x}_{0})$ and 
$v_{l}(\cdot) \triangleq \frac{\partial^{\mathbf{e}_{l}}R_{\mathcal{M}_{\text{\tiny{SLM}}}}(\cdot, \mathbf{x}_{2})}{\partial \mathbf{x}_{2}^{\mathbf{e}_{l}}}Ê\big|_{\mathbf{x}_{2} = \widetilde{\mathbf{x}}_{0}}$.
%where $\widetilde{\mathbf{x}}_{0}$ is defined as in Theorem \ref{thm_bound_asilomar}.
\end{proof}
The difference between the bound \eqref{equ_bound_asilomar_2} and the bound \eqref{equ_bound_asilomar_1} is equal to 
\begin{equation} 
\label{equ_diff_asilomar_bounds}
 \gamma^{2}(\mathbf{x}_{0}) - \exp\left( - \frac{1}{\sigma^{2}}\| (\mathbf{I} - \mathbf{P}_{\mathcal{K}}) \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} \right)  \gamma^{2}(\widetilde{\mathbf{x}}_{0}) 
\end{equation} 
which depend on the choice of the index set $\mathcal{K}$. 
If for a specific index set $\mathcal{K}$ (note that $\mathbf{r}_{\mathbf{x}_{0}}$ depends on $\mathcal{K}$) the prescribed bias is such that 
$\gamma^{2}(\widetilde{\mathbf{x}}_{0}) Ê\approx \gamma^{2}(\mathbf{x}_{0})$,\footnote{This is the case e.g. if $c(\cdot)Ê\equiv 0$, i.e. for unbiased estimation, and the columns of $\mathbf{H}_{\mathcal{K}}$ are 
nearly orthonormal.}
then we have that the quantity \eqref{equ_diff_asilomar_bounds} is approximately always non-negative since 
\begin{equation} 
\exp\left( - \frac{1}{\sigma^{2}}\| (\mathbf{I} - \mathbf{P}_{\mathcal{K}}) \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} \right) \leq 1,
\end{equation} 
which in turn implies that the bound \eqref{equ_bound_asilomar_2} tends to be tighter, i.e. higher, in this case. 
%\subsection{RKHS Interpretation of existing bounds for the SLM}
%Related Work so far: Zvika CRB, AlexZvika HCRB  ---> Interpretation of these bounds in terms of RKHS 
%ZvikaCRB -----> If UMVU exists for the general SLM it will not exploit sparsity

%\subsection{Novel Lower Bounds on the Est. Variance} 

%
%\section{Constructing Estimators with a prescribed bias -- Upper bounds on the minimum achievable variance} 
%\label{sec_constr_est_SLM}
%A particular method of constructing an estimator $\hat{\mathbf{x}}$ having a prescribed bias $\mathbf{c}(\mathbf{x})$ and yielding a small variance 
%at a given parameter vector $\mathbf{x}_{0}$ can be based on the decomposition 
%\begin{equation}
%\hat{\mathbf{x}} = \hat{\mathbf{x}}' + \hat{\mathbf{x}}'', 
%\end{equation} 
%where the estimator $\hat{\mathbf{x}}'$ satisfies  
%\begin{equation} 
%\mathsf{E}_{\mathbf{x}} \{ \hat{\mathbf{x}}'  \} = \mathbf{c}(\mathbf{x}) 
%\end{equation} 
%and the estimator $\hat{\mathbf{x}}''$ satisfies   
%\begin{equation} 
%\mathsf{E}_{\mathbf{x}} \{ \hat{\mathbf{x}}''  \} = \mathbf{0}.  
%\end{equation} 
%In general it is difficult to carry out this procedure since every submatrix of the SLM matrix $\mathbf{H}$ would have to be evaluated. However, in practical situations 
%it is unrealistic to be able evaluate all size $M \times S$ columns of a large matrix $\mathbf{H}$. 

\section{The Sparse Signal in Noise Model}
\label{sec_SSNM} 
%The sparse signal in noise model (SSNM) is obtained from the SLM by setting $\mathbf{H} = \mathbf{I}$. We denote 
%a minimum variance problem associated to the SSNM by $\mathcal{M}_{\text{\tiny{SSNM}}}$, i.e., $\mathcal{M}_{\text{\tiny{SSNM}}}= \left( \mathcal{E}_{\text{\tiny{SSNM}}},c(\cdot), \mathbf{x}_{0} \right)$ where $c(\cdot)$ and $\mathbf{x}_{0}$ being 
%an arbitrary prescribed bias function and fixed parameter vector respectively. 
%By specializing the kernel \eqref{equ_kernel_SLM} associated with the SLM we obtain the kernel associated with $\mathcal{M}_{\text{\tiny{SSNM}}}$ as 
%\begin{equation} 
%R_{\mathcal{M}_{\text{\tiny{SSNM}}}}(\mathbf{x}_{1}, \mathbf{x}_{2}) = \exp \left( (\mathbf{x}_{1} - \mathbf{x}_{0})^{T} ( \mathbf{x}_{2} - \mathbf{x}_{0}) \right). 
%\end{equation} 
We now specialize the results obtained for minimum variance estimation associated with the general SLM  $\mathcal{E}_{\text{\tiny{SLM}}}$ 
to the special case of the SLM given by the SSNM $\mathcal{E}_{\text{\tiny{SSNM}}}$ (cf. \eqref{equ_def_SSNM_est_problem}) 
which is obtained from the SLM by choosing $\mathbf{H} = \mathbf{I}$ (which implies that $M=N$). 
We denote by $\mathcal{M}_{\text{\tiny{SSNM}}} \triangleq \left( \mathcal{E}_{\text{\tiny{SSNM}}},c(\cdot),\mathbf{x}_{0} \right)$ any minimum variance problem that is associated with 
$\mathcal{E}_{\text{\tiny{SSNM}}}$, a specific prescribed bias function $c(\cdot):\mathcal{X}_{S} \rightarrow \mathbb{R}$ and parameter vector $\mathbf{x}_{0}Ê\in \mathcal{X}_{S}$.
The specific choices for $c(\cdot)$ and $\mathbf{x}_{0}$ should be clear from the context. 
The following discussions and results are presented in part in \cite{RKHSISIT2011}. 

%\subsection{RKHS Associated with the SSNM} 
While in principle we can characterize the RKHS $\mathcal{H}(\mathcal{M}_{\text{\tiny{SSNM}}})$ with the kernel 
$R_{\mathcal{M}_{\text{\tiny{SSNM}}}}(\cdot,\cdot): \mathcal{X}_{S} \times \mathcal{X}_{S} \rightarrow \mathbb{R}: R_{\mathcal{M}_{\text{\tiny{SSNM}}}}(\mathbf{x}_{1},\mathbf{x}_{2})\triangleq \exp \left( \frac{1}{\sigma^{2}} (\mathbf{x}_{1} - \mathbf{x}_{0})^{T} (\mathbf{x}_{2} - \mathbf{x}_{0}) \right)$, using Theorem \ref{thm_isometry_LGM} and Theorem \ref{thm_relation_RKHS_LGM_SLM} specialized to $\mathbf{H}=\mathbf{I}$, it will turn out that a more convenient characterization is possible by exploiting the specific structure of $\mathcal{H}(\mathcal{M}_{\text{\tiny{SLM}}})$ induced by the choice $\mathbf{H} = \mathbf{I}$. 

In particular we have 
\begin{theorem} 
\label{thm_entire_charact_RKHS_SSNM}
Consider the minimum variance problem $\mathcal{M}_{\text{\tiny{SSNM}}} = \left( \mathcal{E}_{\text{\tiny{SSNM}}},c(\cdot),\mathbf{x}_{0} \right)$ with 
a specific choice for $\sigma$, $S$, $N$, $\mathbf{x}_{0} \in \mathcal{X}_{S}$ and $c(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}$. 
The RKHS $\mathcal{H}(\mathcal{M}_{\text{\tiny{SSNM}}})$ is isometric to the RKHS $\mathcal{H}(R_{e})$ associated with 
the kernel $R_{e}(\cdot,\cdot): \mathcal{X}_{S} \times \mathcal{X}_{S} \rightarrow \mathbb{R}$: 
\begin{equation} 
R_{e}(\mathbf{x}_{1}, \mathbf{x}_{2}) = \exp(\mathbf{x}_{2}^{T} \mathbf{x}_{1}). 
\end{equation}
A congruence from $\mathcal{H}(\mathcal{M}_{\text{\tiny{SSNM}}})$ to $\mathcal{H}(R_{e})$ is given by $\mathsf{K}_{e}[\cdot]: \mathcal{H}(\mathcal{M}_{\text{\tiny{SSNM}}}) \rightarrow \mathcal{H}(R_{e})$: 
\begin{equation} 
\label{equ_def_congruence_SSNM}
f(\cdot) \mapsto \widetilde{f}(\cdot) =  \mathsf{K}_{e}[f(\cdot)] :  \widetilde{f}(\mathbf{x}') 
= f(\sigma \mathbf{x}') \exp\left( - \frac{1}{2 \sigma^{2}} \|\mathbf{x}_{0} \|^{2}_{2} + \frac{1}{\sigma}(\mathbf{x}')^{T} \mathbf{x}_{0}\right).
\end{equation} 
The RKHS $\mathcal{H}(R_{e})$ is differentiable up to any order and contains 
the functions 
\begin{equation} 
g^{(\mathbf{p})}(\mathbf{x}) \triangleq \frac{1}{\sqrt{\mathbf{p}!}} \frac{ \partial^{\mathbf{p}} R_{e}(\mathbf{x}, \mathbf{x}_{2})}{\partial \mathbf{x}_{2}^{\mathbf{p}}}\bigg|_{\mathbf{x}_{2} = \mathbf{0}} = \frac{1}{\sqrt{\mathbf{p}!}} \mathbf{x}^{\mathbf{p}}, 
\end{equation}
i.e., 
\begin{equation} 
\label{equ_def_SSNM_par_der_R_e}
g^{(\mathbf{p})}(\cdot) \in \mathcal{H}(R_{e}), 
\end{equation}
%\end{equation}
where $\mathbf{p} \in \mathbb{Z}_{+}^{N}$ is an arbitrary multi-index with $\| \mathbf{p} \|_{0} \leq S$, i.e., $\mathbf{p} \in \mathbb{Z}_{+}^{N} \cap \mathcal{X}_{S}$.

The inner-product of an arbitrary function $f(\cdot) \in \mathcal{H}(R_{e})$ with any function $g^{(\mathbf{p})}(\cdot)$ is given by 
\begin{equation} 
\label{equ_inner_prod_part_der_RKHS_Re}
\langle f (\cdot), g^{(\mathbf{p})}(\cdot) \rangle_{\mathcal{H}(R_{e})} = \frac{1}{\sqrt{\mathbf{p}!}} \frac{ \partial^{\mathbf{p}} f(\mathbf{x})} { \mathbf{x}^{\mathbf{p}}} \bigg|_{\mathbf{x} = 0}. 
\end{equation} 

Moreover, the set $\{g^{(\mathbf{p})}(\cdot) \}_{\mathbf{p} \in \mathbb{Z}_{+}^{N} \cap \mathcal{X}_{S}}$ is an ONB for $\mathcal{H}(R_{e})$ and therefore
any function $f(\cdot) \in \mathcal{H}(R_{e})$ can be written point-wise as 
\begin{equation}
\label{equ_series_repr_RKHS_R_e}
f(\mathbf{x}) = \sum_{\mathbf{p} \in \mathbb{Z}_{+}^{N} \cap \mathcal{X}_{S}} a[\mathbf{p}] g^{(\mathbf{p})}(\mathbf{x}) =   \sum_{\mathbf{p} \in \mathbb{Z}_{+}^{N} \cap \mathcal{X}_{S}} a[\mathbf{p}] \frac{1}{\sqrt{\mathbf{p}!}} \mathbf{x}^{\mathbf{p}}
\end{equation} 
with  a coefficient sequence $a[\mathbf{p}] \in \ell^{2}(\mathbb{Z}_{+}^{N} \cap \mathcal{X}_{S})$. 
\end{theorem}

\begin{proof} 
The derivation of the congruence in \eqref{equ_def_congruence_SSNM} is completely analogous to the proof of Theorem \ref{thm_isometry_LGM} specialized to $\mathbf{H} = \mathbf{I}$. 
From Theorem \ref{thm_der_repr_prop} we obtain \eqref{equ_def_SSNM_par_der_R_e} and \eqref{equ_inner_prod_part_der_RKHS_Re}. 
The fact that the set $\{g^{(\mathbf{p})}(\cdot) \}_{\mathbf{p} \in \mathbb{Z}_{+}^{N} \cap \mathcal{X}_{S}}$ is an ONB follows from Theorem \ref{thm_pointwise_series_kernel_ONB} by \eqref{equ_inner_prod_part_der_RKHS_Re} 
(which implies that $\langle g^{(\mathbf{p}')} (\cdot), g^{(\mathbf{p})}(\cdot) \rangle_{\mathcal{H}(R_{e})}= \delta_{\mathbf{p}', \mathbf{p}}$) and the identity 
$R_{e}(\mathbf{x}_{1}, \mathbf{x}_{2}) = \sum_{\mathbf{p} \in\mathbb{Z}_{+}^{N} \cap \mathcal{X}_{S}} \frac{ \mathbf{x}_{1}^{\mathbf{p}}}{\sqrt{\mathbf{p}!}}\frac{ \mathbf{x}_{2}^{\mathbf{p}}}{\sqrt{\mathbf{p}!}}$ which is valid for every $\mathbf{x}_{1}, \mathbf{x}_{2} \in \mathcal{X}_{S}$.
Finally, the series representation in \eqref{equ_series_repr_RKHS_R_e} follows from Theorem \ref{thm_isometry_hilbert_space_coeffs_space}.  
\end{proof} 

Note that the kernel $R_{e}(\cdot,\cdot)$ in Theorem \ref{thm_entire_charact_RKHS_SSNM} is the restriction to the sub-domain $\mathcal{X}_{S} \times \mathcal{X}_{S}$ of the kernel $R_{g}^{(N)}(\cdot,\cdot)$ defined in Theorem \ref{thm_isometry_LGM}, i.e., $R_{e}(\cdot,\cdot) =  R_{g}^{(N)}(\cdot,\cdot)\big|_{\mathcal{X}_{S} \times \mathcal{X}_{S}}$. From this we have that the RKHS $\mathcal{H}(R_{e})$ and $\mathcal{H}(R_{g}^{(N)})$ are related via Theorem \ref{thm_reducing_domain_RKHS}. 

Based on Theorem \ref{thm_entire_charact_RKHS_SSNM} we have the following general characterization of the minimum achievable variance and the corresponding LMV estimator 
for the minimum variance problem $\mathcal{M}_{\text{\tiny{SSNM}}} = \left( \mathcal{E}_{\text{\tiny{SSNM}}},c(\cdot),\mathbf{x}_{0} \right)$:
\begin{theorem} 
\label{thm_general_min_achiev_var_LMV_SSNM}
Given the minimum variance problem $\mathcal{M}_{\text{\tiny{SSNM}}} = \left( \mathcal{E}_{\text{\tiny{SSNM}}},c(\cdot),\mathbf{x}_{0} \right)$ we have that the prescribed bias function 
$c(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}$ is valid if and only if 
there exists a necessarily unique coefficient sequence $a[\mathbf{p}] \in \ell^{2}(\mathbb{Z}_{+}^{N} \cap \mathcal{X}_{S})$ solving the equation 
\begin{equation}
\label{equ_condition_gamma_valid_SSNM_fourier_series_R_e}
\gamma(\sigma \mathbf{x}) \nu_{\mathbf{x}_{0}}(\mathbf{x}) = \sum_{\mathbf{p} \in \mathbb{Z}_{+}^{N} \cap \mathcal{X}_{S}} a[\mathbf{p}] \frac{\mathbf{x}^{\mathbf{p}}}{\sqrt{\mathbf{p}!}}
\end{equation}
for every $\mathbf{x} \in \mathcal{X}_{S}$, where $\nu_{\mathbf{x}_{0}}(\mathbf{x}) \triangleq \exp\left( - \frac{1}{2 \sigma^{2}} \|\mathbf{x}_{0} \|^{2}_{2} + Ê\frac{1}{\sigma} \mathbf{x}^{T} \mathbf{x}_{0}\right)$ and $\gamma(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}: \gamma(\mathbf{x}) \triangleq c(\mathbf{x}) + x_{k}$ denotes the prescribed mean function. 

If the prescribed bias $c(\cdot)$ is valid for $\mathcal{M}_{\text{\tiny{SSNM}}}$, then the minimum achievable variance is given by 
\begin{equation}
\label{equ_ssnm_expr_min_ach_var}
L_{\mathcal{M}_{\text{\tiny{SSNM}}}}  = \sum_{\mathbf{p} \in \mathbb{Z}_{+}^{N} \cap \mathcal{X}_{S}} \frac{1}{\mathbf{p}!}  \left( \frac{ \partial^{\mathbf{p}} ( \gamma(\sigma \mathbf{x}) \nu_{\mathbf{x}_{0}}(\mathbf{x}))}{\partial \mathbf{x}^{\mathbf{p}}} \bigg|_{\mathbf{x}=\mathbf{0}} \right)^{2} - (\gamma(\mathbf{x}_{0}))^{2}.
\end{equation}

The corresponding LMV estimator $\hat{x}_{k}^{(\mathbf{x}_{0})}(\cdot)$ is obtained as 
\begin{equation}
\label{equ_ssnm_general_expr_LMV}
\hat{x}_{k}^{(\mathbf{x}_{0})}(\mathbf{y}) = \sum_{\mathbf{p} \in \mathbb{Z}_{+}^{N} \cap \mathcal{X}_{S}} \frac{a_{\mathbf{x}_{0}}[\mathbf{p}]}{\sqrt{\mathbf{p}!}} 
\frac{\partial^{\mathbf{p}} \exp  \bigg(Ê\! \frac{1}{\sigma^{2}} \mathbf{y}^{T}( \sigma \mathbf{x} - \mathbf{x}_{0}) + \frac{1}{\sigma} \mathbf{x}_{0}^{T} \mathbf{x} \!-\! \frac{1}{2} \| \mathbf{x} \|^{2}_{2}  \bigg)}{ \partial \mathbf{x}^{\mathbf{p}}} \bigg|_{\mathbf{x}= \mathbf{0}}
\end{equation}
with coefficients 
\begin{equation} 
a_{\mathbf{x}_{0}}[\mathbf{p}] Ê\triangleq  \langle \gamma(\sigma \mathbf{x}) \nu_{\mathbf{x}_{0}}(\mathbf{x}), g^{(\mathbf{p})}(\mathbf{x}) \rangle_{\mathcal{H}(R_{e})} = 
\frac{1}{\sqrt{\mathbf{p}!}} \frac{ \partial^{\mathbf{p}} \left( \gamma( \sigma \mathbf{x}) \nu_{\mathbf{x}_{0}}(\mathbf{x}) \right)}{\partial \mathbf{x}^{\mathbf{p}}} \bigg|_{\mathbf{x}=\mathbf{0}}, 
\end{equation} 
i.e., $b(\hat{x}_{k}^{(\mathbf{x}_{0})}(\cdot); \mathbf{x})  = c(\mathbf{x})$ for every $\mathbf{x} \in \mathcal{X}_{S}$ and $v(\hat{x}_{k}^{(\mathbf{x}_{0})}(\cdot); \mathbf{x}_{0}) = L_{\mathcal{M}_{\text{\tiny{SSNM}}}}$. 
\end{theorem}

\begin{proof}
By Theorem \ref{thm_main_facts_RKHS_MVE} we have that the prescribed bias function $c(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}$ is valid for $\mathcal{M}_{\text{\tiny{SSNM}}}$ 
if and only if the prescribed bias $\gamma(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}: \gamma(\mathbf{x}) = c(\mathbf{x}) + x_{k}$ belongs to 
$\mathcal{H}(\mathcal{M}_{\text{\tiny{SSNM}}})$ which by Theorem \ref{thm_entire_charact_RKHS_SSNM} is the case if and only if 
\begin{equation} 
\label{equ_cond_valid_gamma_element_RKHS}
\gamma( \sigma \mathbf{x})  \exp\left( - \frac{1}{2 \sigma^{2}} \| \mathbf{x}_{0} \|^{2}_{2} + \frac{1}{\sigma} \mathbf{x}^{T} \mathbf{x}_{0}\right)  \in \mathcal{H}(R_{e}),
\end{equation} 
which by Theorem \ref{thm_entire_charact_RKHS_SSNM} is the case if and only if there exists a coefficient sequence $a[\mathbf{p}] \in \ell^{2}(\mathbb{Z}_{+}^{N} \cap \mathcal{X}_{S})$ that solves \eqref{equ_condition_gamma_valid_SSNM_fourier_series_R_e} for every $\mathbf{x} \in \mathcal{X}_{S}$.

Lets assume from now on that the prescribed bias function $c(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}$ is valid for $\mathcal{M}_{\text{\tiny{SSNM}}}$, i.e., \eqref{equ_cond_valid_gamma_element_RKHS} holds. 
By Theorem \ref{thm_main_facts_RKHS_MVE}, Theorem \ref{thm_entire_charact_RKHS_SSNM} and Theorem \ref{thm_fourier_onb} we obtain 
\begin{align}
L_{\mathcal{M}_{\text{\tiny{SSNM}}}}  & = \| \gamma(\sigma \mathbf{x}) \nu_{\mathbf{x}_{0}}(\mathbf{x}) \|_{\mathcal{H}(R_{e})}^{2} - \left( \gamma(\mathbf{x}_{0}) \right)^{2} = 
\sum_{\mathbf{p} \in \mathbb{Z}_{+}^{N} \cap \mathcal{X}_{S}}  \left( \langle \gamma(\sigma \mathbf{x}) \nu_{\mathbf{x}_{0}}(\mathbf{x}), g^{(\mathbf{p})}(\mathbf{x}) \rangle_{\mathcal{H}(R_{e})} \right)^{2}   - \left( \gamma(\mathbf{x}_{0}) \right)^{2} \nonumber \\ 
& = \sum_{\mathbf{p} \in \mathbb{Z}_{+}^{N} \cap \mathcal{X}_{S}} \frac{1}{\mathbf{p}!}  \left( \frac{ \partial^{\mathbf{p}} ( \gamma(\sigma\mathbf{x}) \nu_{\mathbf{x}_{0}}(\mathbf{x}))}{\partial \mathbf{x}^{\mathbf{p}}} \bigg|_{\mathbf{x}=\mathbf{0}} \right)^{2} - (\gamma(\mathbf{x}_{0}))^{2},
\end{align} 
which verifies \eqref{equ_ssnm_expr_min_ach_var}. 

We then have also by  
\eqref{equ_condition_gamma_valid_SSNM_fourier_series_R_e} that 
\begin{equation} 
\label{equ_ssnm_expr_gamma_valid}
\gamma(\mathbf{x}) =  \exp\left(  \frac{1}{2 \sigma^{2}} \|\mathbf{x}_{0} \|^{2}_{2} - Ê
\frac{1}{\sigma^2 } \mathbf{x}^{T} \mathbf{x}_{0}\right) \sum_{\mathbf{p} \in \mathbb{Z}_{+}^{N} \cap \mathcal{X}_{S}} \frac{a_{0}[\mathbf{p}]}{\sqrt{\mathbf{p}!}}  \Bigg( \frac{\mathbf{x}}{\sigma}\Bigg)^{\mathbf{p}},
\end{equation}
with a suitable coefficient sequence $a_{0}[\mathbf{p}] \in \ell^{2}(\mathbb{Z}_{+}^{N} \cap \mathcal{X}_{S})$. 
It can be easily verified that due to \eqref{equ_condition_gamma_valid_SSNM_fourier_series_R_e} and Theorem \ref{thm_entire_charact_RKHS_SSNM}, the coefficients 
$a_{0}[\mathbf{p}]$ can be calculated from $\gamma(\cdot)$ as 
\begin{equation}
a_{0}[\mathbf{p}]= \langle \gamma(\sigma \mathbf{x}) \nu_{\mathbf{x}_{0}}(\mathbf{x}), g^{(\mathbf{p})}(\mathbf{x}) \rangle_{\mathcal{H}(R_{e})} = \frac{1}{\sqrt{\mathbf{p}!}} \frac{ \partial^{\mathbf{p}} \left( \gamma( \sigma \mathbf{x}) \nu_{\mathbf{x}_{0}}(\mathbf{x}) \right)}{\partial \mathbf{x}^{\mathbf{p}}} \bigg|_{\mathbf{x}=\mathbf{0}}
\end{equation} 
implying their uniqueness. 

We can further develop \eqref{equ_ssnm_expr_gamma_valid} as 
%\begin{align} 
\begin{align} 
\gamma(\mathbf{x}) & =   \exp\left(  \frac{1}{2 \sigma^{2}} \|\mathbf{x}_{0} \|^{2}_{2} - Ê\frac{1}{\sigma^2 } \mathbf{x}^{T} \mathbf{x}_{0}\right) \sum_{\mathbf{p} \in \mathbb{Z}_{+}^{N} \cap \mathcal{X}_{S}} \frac{a_{0}[\mathbf{p}]}{\sqrt{\mathbf{p}!}}  \Bigg( \frac{1}{\sigma} \mathbf{x} \Bigg)^{\mathbf{p}} \nonumber \\ 
& = \exp \bigg( - \frac{1}{2\sigma^{2}} \| \mathbf{H} \mathbf{x}_{0} \|^{2}_{2} \bigg)  \sum_{\mathbf{p} \in \mathbb{Z}_{+}^{N}} \frac{a_{0}[\mathbf{p}]}{\sqrt{\mathbf{p}!}}   
\frac{ \partial^{\mathbf{p}} \bigg( R_{\mathcal{M}_{\text{\tiny{SSNM}}}}(\mathbf{x}, \sigma \mathbf{x}') \exp \big( \frac{1}{\sigma} \mathbf{x}_{0}^{T} \mathbf{x}' \big) \bigg)}{\partial \mathbf{x}'^{\mathbf{p}}}\Bigg|_{\mathbf{x}'=\mathbf{0}}  \label{equ_def_arb_bias_coeffs_SSNM_2}.
\end{align} 
%is valid for $\mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}}(\mathbf{x}_{0}))$ and by its very definition satisfies $\tilde{c}(\cdot) \big|_{\mathcal{X}_{S}} = c(\cdot)$. 
which implies via Theorem \ref{thm_der_repr_prop_mult_func}, Theorem \ref{thm_main_facts_RKHS_MVE}, Theorem \ref{thm_isometry_RKHS_rhos_derivative_kernel} and the identity 
$\rho_{\text{\tiny{SSNM}}}(\mathbf{y}, \mathbf{x}) = \exp \left( \frac{1}{\sigma^{2}} \mathbf{y}^{T}(\mathbf{x}-\mathbf{x}_{0}) - \frac{1}{2 \sigma^{2}}(\| \mathbf{x} \|^{2}_{2} - \|Ê\mathbf{x}_{0} \|^{2}_{2}) \right)$ that the estimator defined by \eqref{equ_ssnm_general_expr_LMV} is nothing but the 
LMV estimator for $\mathcal{M}_{\text{\tiny{SSNM}}}$. 
\end{proof}

Theorem \ref{thm_general_min_achiev_var_LMV_SSNM} is the specialization to the SSNM of Theorem \ref{thm_condition_valid_bias_SLM} which applies for a general SLM. 
The statement of Theorem \ref{thm_general_min_achiev_var_LMV_SSNM} 
is stronger than that of Theorem \ref{thm_condition_valid_bias_SLM} because 
it contains an explicit expression for the minimum achievable variance $L_{\mathcal{M}_{\text{\tiny{SSNM}}}}$ and corresponding LMV estimator. This is possible because of the 
isometry between the RKHS $\mathcal{H}(\mathcal{M}_{\text{\tiny{SSNM}}})$ itself and the RKHS $\mathcal{H}(R_{e})$, i.e., without the intermediate step via the LGM and Theorem \ref{thm_reducing_domain_RKHS}, 
as used in Theorem \ref{thm_condition_valid_bias_SLM}. 

Note that the expression \eqref{equ_ssnm_expr_min_ach_var} nicely shows the influence of the sparsity constraints on minimum variance estimation for the SSNM. 
Indeed, for a fixed prescribed bias $c_{0}(\cdot): \mathbb{R}^{N} \rightarrow \mathbb{R}$ and parameter vector $\mathbf{x}_{0} \in \mathcal{X}_{S}$, denoting 
the minimum achievable variance for $\mathcal{M}_{\text{\tiny{non-sparse}}}= \left( \mathcal{E}_{\text{\tiny{SSNM}}},c_{0}(\cdot),\mathbf{x}_{0} \right)$ with $S=N$, i.e. without any sparsity constraints in which case the SSNM coincides with the LGM with system matrix $\mathbf{H}=\mathbf{I}$, 
by $L_{\text{\tiny{non-sparse}}}$ and the minimum achievable variance for 
$\mathcal{M}_{\text{\tiny{SSNM}}}= \left( \mathcal{E}_{\text{\tiny{SSNM}}},c_{0}(\cdot)\big|_{\mathcal{X}_{S}},\mathbf{x}_{0} \right)=\mathcal{M}_{\text{\tiny{non-sparse}}}\big|_{\mathcal{X}_{S}}$ 
with $S<N$ by $L_{S}$, we have 
\begin{equation}
\label{equ_diff_min_achiev_var_SSNM}
L_{\text{\tiny{non-sparse}}}-L_{S}  =
 \sum_{\mathbf{p} \in    \mathbb{Z}_{+}^{N} \setminus \left(\mathbb{Z}_{+}^{N} \cap \mathcal{X}_{S} \right)} \frac{1}{\mathbf{p}!}  
 \left( \frac{ \partial^{\mathbf{p}} ( (c_{0}(\sigma \mathbf{x}) + \sigma x_{k})\nu_{\mathbf{x}_{0}}(\mathbf{x}))}{\partial \mathbf{x}^{\mathbf{p}}} \bigg|_{\mathbf{x}=\mathbf{0}} \right)^{2}.
\end{equation}
Since the summands in \eqref{equ_diff_min_achiev_var_SSNM} are non-negative, we have that by reducing the sparsity degree $S$ the number of summands 
is reduced and so is the minimum achievable variance $L_{S}$. 

Based on Theorem \ref{thm_general_min_achiev_var_LMV_SSNM} we have the following obvious result concerning the existence of a UMV estimator for the SSNM:  
%is obtained by $\mathc: 
\begin{lemma} 
Consider the SSNM $\mathcal{E}_{\text{\tiny{SSNM}}}=\left(\mathcal{X}_{S},f_{\text{\tiny{LGM}},\mathbf{I}}(\mathbf{y};\mathbf{x}),g(\mathbf{x}) = x_{k} \right)$ 
and a prescribed bias function $c(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}$. Then there exists a UMV estimator for $\mathcal{E}_{\text{\tiny{SSNM}}}$ and $c(\cdot)$ if 
and only if the LMV $\hat{x}_{k}^{(\mathbf{x}_{0})}(\mathbf{y})$ for the minimum variance problem $\mathcal{M}_{\text{\tiny{SSNM}}} = \left(\mathcal{E}_{\text{\tiny{SSNM}}},c(\cdot), \mathbf{x}_{0} \right)$ given 
explicitly by \eqref{equ_ssnm_general_expr_LMV} does not depend on $\mathbf{x}_{0}$. 
%\begin{equation}
%\sum_{\mathbf{p} \in \mathbb{Z}_{+}^{N} \cap \mathcal{X}_{S}} a_{\mathbf{x}_{0}}[\mathbf{p}] \frac{\partial^{\mathbf{p}} \exp  \bigg(Ê\! \mathbf{y}^{T}(\mathbf{x} - \mathbf{x}_{0}) + \mathbf{x}_{0}^{T} \mathbf{x} \!-\! \frac{1}{2} \| \mathbf{x} \|^{2}_{2}  \bigg)}{ \partial^{\mathbf{p}} \mathbf{x}} \bigg|_{\mathbf{x}= \mathbf{0}}
%\end{equation}
\end{lemma}
%\begin{proof} 
%\end{proof} 

We now specialize Theorem \ref{thm_general_min_achiev_var_LMV_SSNM} to a specific class of bias functions $c(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}$ that we call ``diagonal'' bias functions. 
A diagonal bias function $c(\mathbf{x})$ depends on the parameter $\mathbf{x}$ only through the $k$th component (where $k$ is the same index as used for the parameter 
function of the SSNM in \eqref{equ_def_SSNM_est_problem}), i.e., $c(\mathbf{x}) = \tilde{c}(x_{k})$ where 
$\tilde{c}(\cdot) : \mathbb{R} \rightarrow \mathbb{R}$ is a certain function, which may vary with the index $k$ used for the definition 
of the parameter function of $\mathcal{E}_{\text{\tiny{SSNM}}}$ in \eqref{equ_def_SSNM_est_problem}. 
Similarly we say that an estimator $\hat{x}_{k}(\mathbf{y})$ for the SSNM is 
diagonal if it depends on the observation $\mathbf{y}$ only via the $k$th entry, i.e., $\hat{x}_{k}(\mathbf{y}) = \hat{x}_{k}(y_{k})$ for a diagonal estimator. 
Obviously, the bias function of a diagonal estimator for the SSNM is diagonal. 
The well known hard- and soft-thresholding estimators are diagonal estimators for the SSNM in this sense. However, the bias function of the 
maximum likelihood (ML) estimator for the SSNM is not diagonal in this sense. 

Making the weak assumption that $\tilde{c}(x_{k}): \mathbb{R} \rightarrow \mathbb{R}$ can be represented by a power-series which converges everywhere on $\mathbb{R}$ we obtain 
\begin{theorem} 
\label{thm_diag_bias_min_achiev_var_LMV}
Consider the minimum variance problem $\mathcal{M}_{\text{\tiny{SSNM}}}=\left(\mathcal{E}_{\text{\tiny{SSNM}}},c(\cdot),\mathbf{x}_{0}\right)$ for a specific choice for 
$\sigma$, $S$, $M$, $N$, $\mathbf{x}_{0}$ where 
the prescribed bias $c(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}$ is diagonal, i.e., $c(\mathbf{x}) = c'(x_{k})$. Moreover, we assume that the function $c'(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}$ 
is such that the prescribed mean function $\gamma(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}: \gamma(\mathbf{x}) = c(\mathbf{x}) + x_{k}$ can be written as a power series 
at $\mathbf{x}_{0}$ which converges everywhere on $\mathbb{R}$, i.e., 
\begin{equation}
\label{equ_prescr_mean_diag_bias}
\gamma(\mathbf{x}) = \sum\limits_{l \in \mathbb{Z}_{+}} \frac{m_{l}}{l!} (x_{k} - x_{0,k})^{l}
\end{equation}
with suitable coefficients $m_{l} \in \mathbb{R}$. 
We then have that the bias $c(\cdot)$ is valid for $\mathcal{M}_{\text{\tiny{SSNM}}}$ if and only if 
\begin{equation} 
\label{equ_cond_valid_bias_diagon_bias_SSNM}
\sum\limits_{l \in \mathbb{Z}_{+}} \frac{(m_{l})^{2} \sigma^{2l}}{l!}  < \infty. 
\end{equation}

If the coefficients $m_{l}$ satisfy \eqref{equ_cond_valid_bias_diagon_bias_SSNM} then we have for the case where $| \supp(\mathbf{x}_{0}) \cup \{k\}| < S+1$ that
\begin{equation}
\label{equ_expr_min_achiev_var_case_1_SSNM}
L_{\mathcal{M}_{\text{\tiny{SSNM}}}}  = \sum\limits_{lÊ\in \mathbb{N}} \frac{(m_{l})^{2}}{l!} \sigma^{2l}
\end{equation} 
with the corresponding LMV estimator 
\begin{equation}
\label{equ_expr_LMV_diag_bias_case_1_SSNM}
\hat{x}_{k}^{(\mathbf{x}_{0})}(\mathbf{y}) = \sum_{l \in \mathbb{Z}_{+}} \frac{ m_{l}}{l!} \sigma^{l} \mathsf{H}_{l} \left(\frac{ y_k-x_{0,k} }{\sigma} \right) 
\end{equation} 
i.e., $b(\hat{x}_{k}^{(\mathbf{x}_{0})}(\cdot);\mathbf{x})  = m(x_{k}) - x_{k}$ for every $\mathbf{x} \in \mathcal{X}_{S}$ and $v(\hat{x}_{k}^{(\mathbf{x}_{0})}(\cdot); \mathbf{x}_{0}) = L_{\mathcal{M}_{\text{\tiny{SSNM}}}}$.

For the remaining case where $| \supp(\mathbf{x}_{0}) \cup \{k\}| = S+1$ we have, by denoting the indices of the support of $\mathbf{x}_{0}$ as $\supp(\mathbf{x}_{0})=(i_{1},\ldots,i_{S})$, that
\begin{equation}
\label{equ_min_achiev_var_case_2_ssnm_main}
L_{\mathcal{M}_{\text{\tiny{SSNM}}}}  = \left(\sum_{l \in \mathbb{Z}_{+}} \frac{m_{l}^{2} \sigma^{2l}}{l!} \right) \left( \sum_{j \in [S]} \exp\bigg( - \frac{x_{0,i_{j}}^{2}}{\sigma^{2}} \bigg) 
\prod_{j' \in [j-1]}  \bigg(Ê\! 1 - \exp\bigg( - \frac{x_{0,i_{j'}}^{2}}{\sigma^{2}} \bigg) \! \bigg)Ê\right)- \big(\gamma(\mathbf{x}_{0})Ê\big)^{2}
\end{equation} 
with the corresponding LMV estimator 
\begin{align}
\label{equ_lmv_case_2_ssnm_main}
\hat{x}_{k}^{(\mathbf{x}_{0})}(\mathbf{y}) & = \nonumber \\ 
& \hspace*{-10mm} \! \sum_{l\in \mathbb{Z}_{+}} \frac{ m_{l}}{l!} \sigma^{l} \mathsf{H}_{l} \left( \frac{y_k}{\sigma} \right)\! \sum_{j \in [S]} \exp\bigg( -  \frac{x_{0,i_{j}}^{2}+2y_{i_{j}}x_{0,i_{j}}}{2 \sigma^{2}} \! \bigg)
 \prod_{j' \in [j-1]}  \bigg(Ê\! 1  -  \exp\bigg( - \frac{x_{0,i_{j'}}^{2}+2y_{j'}x_{0,i_{j'}}}{2 \sigma^{2}} \! \bigg) \! \bigg).
\end{align} 
Here, we used the $l$th order (probabilists') Hermite polynomial $\mathsf{H}_{l}(\cdot): \mathbb{R} \rightarrow \mathbb{R}$ defined as
\begin{equation}
\mathsf{H}_{l}(x) = (-1)^l e^{x^2/2}\frac{d^l}{dx^l}e^{-x^2/2}. 
\end{equation} 
\end{theorem} 
\begin{proof}
Appendix A. 
\end{proof}


A slight reformulation of Theorem \ref{thm_diag_bias_min_achiev_var_LMV} yields 
\begin{corollary} 
\label{cor_thm_min_var_lmv_ssnm_diag_bias_ISIT}
Consider the minimum variance problem $\mathcal{M}_{\text{\tiny{SSNM}}}=\left(\mathcal{E}_{\text{\tiny{SSNM}}},c(\cdot),\mathbf{x}_{0}\right)$ for a specific choice for 
$\sigma$, $S$, $N$, $\mathbf{x}_{0}\in \mathcal{X}_{S}$ where $S <N$ and the prescribed bias $c(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}$ is diagonal, i.e., $c(\mathbf{x}) = \tilde{c}(x_{k})$. 
Moreover we assume that the bias function $c(\cdot)$ is valid and such that the prescribed mean function $\gamma(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}: \gamma(\mathbf{x}) = c(\mathbf{x}) + x_{k}$ can be written 
as a power series at $x_{0,k}$ which converges everywhere, i.e., we have $\gamma(\mathbf{x}) = \sum\limits_{l \in \mathbb{Z}_{+}} \frac{m_{l}}{l!} (x_{k} - x_{0,k})^{l}$ with coefficients $m_{l}$ 
satisfying \eqref{equ_cond_valid_bias_diagon_bias_SSNM}. 

Then we obtain for the minimum achievable variance 
\begin{equation}
\label{equ_expr_min_achiev_var_ISIT_SSNM}
L_{\mathcal{M}_{\text{\tiny{SSNM}}}}  = \bigg( \sum_{l \in \mathbb{Z}_{+}} \frac{m_{l}^{2} \sigma^{2l}}{l!} \bigg) h(\mathbf{x}_{0}; \mathcal{I}) - \big(\gamma(\mathbf{x}_{0})Ê\big)^{2}
\end{equation} 
and the corresponding LMV estimator 
\begin{equation}
\label{equ_expr_LMV_diag_bias_ISIT_SSNM}
\hat{x}_{k}^{(\mathbf{x}_{0})}(\mathbf{y})  = h(\mathbf{y}, \mathbf{x}_{0}; \mathcal{I}) \sum_{l\in \mathbb{Z}_{+}} \frac{ m_{l}}{l!} \sigma^{l} \mathsf{H}_{l} \left( \frac{y_k}{\sigma} \right)
\end{equation} 
with 
\begin{equation} 
\label{equ_factor_ISIT_SSNM_min_achiev_var}
h(\mathbf{x}; \mathcal{I}) \triangleq \sum_{j \in [S]} \exp\bigg( - \frac{x_{i_{j}}^{2}}{\sigma^{2}} \bigg) \prod_{j' \in [j-1]}  \bigg(Ê\! 1 - \exp\bigg( - \frac{x_{i_{j'}}^{2}}{\sigma^{2}} \bigg) \bigg) \leq 1,
\end{equation}
\begin{align} 
\label{equ_factor_ISIT_SSNM_LMV}
h(\mathbf{y}, \mathbf{x}; \mathcal{I}) & \triangleq\sum_{j \in [S]} \exp\bigg( -  \frac{x_{i_{j}}^{2}+2y_{i_{j}}x_{i_{j}}}{2 \sigma^{2}} \! \bigg)   \prod_{j' \in [j-1]}  \bigg(Ê\! 1  -  \exp\bigg( - \frac{x_{i_{j'}}^{2}+2y_{j'}x_{i_{j'}}}{2 \sigma^{2}} \! \bigg) \bigg) ,
\end{align}
and an arbitrary index set $\mathcal{I} = \{ i_{1}, \ldots, i_{S} \}$ such that $|\mathcal{I}| = S$ and $\supp(\mathbf{x}_{0}) \setminus \{k\} \subseteq \mathcal{I}$. 
\end{corollary}
\begin{proof}
The statement is readily obtained from \ref{thm_diag_bias_min_achiev_var_LMV}, since in the case where 
$| \supp(\mathbf{x}_{0}) \cup \{k\}| = S+1$ we have necessarily that $\mathcal{I}=\supp(\mathbf{x}_{0})$ implying that \eqref{equ_expr_min_achiev_var_ISIT_SSNM}, \eqref{equ_expr_LMV_diag_bias_ISIT_SSNM} coincide with \eqref{equ_min_achiev_var_case_2_ssnm_main}, \eqref{equ_lmv_case_2_ssnm_main}. 
In the remaining case, where $|\supp(\mathbf{x}_{0}) \cup \{k\}| < S+1$, there must be some index $i \in \mathcal{I}$ (note that we assume $S < N$) for which $x_{0,i}=1$ implying that $h(\mathbf{x}_{0}; \mathcal{I})=1$, $h(\mathbf{y}, \mathbf{x}_{0}; \mathcal{I}) =1$ and in 
turn that \eqref{equ_expr_min_achiev_var_ISIT_SSNM}, \eqref{equ_expr_LMV_diag_bias_ISIT_SSNM} coincide with \eqref{equ_expr_min_achiev_var_case_1_SSNM}, \eqref{equ_expr_LMV_diag_bias_case_1_SSNM} in this case.

The inequality $h(\mathbf{x}; \mathcal{I}) \leq 1$ is verified by observing that
\begin{align} 
& \sum_{j \in [S]} \exp\bigg( - \frac{x_{i_{j}}^{2}}{\sigma^{2}} \bigg) \prod_{j' \in [j-1]}  \bigg(Ê\! 1 - \exp\bigg( - \frac{x_{i_{j'}}^{2}}{\sigma^{2}} \bigg) \bigg)  \nonumber \\Ê
& = \prod_{j' \in [S]}   \exp\bigg( - \frac{x_{i_{j'}}^{2}}{\sigma^{2}} \bigg) \sum_{j \in [S]} \Bigg( \prod_{j''' \in [S]Ê\setminus [j]} \!  \exp\bigg( \frac{x_{i_{j'''}}^{2}}{\sigma^{2}} \bigg) \Bigg) \Bigg( \prod_{j'' \in [j-1]}  \bigg(Ê\!  \exp\bigg( \frac{x_{i_{j''}}^{2}}{\sigma^{2}} \bigg)-1 \bigg) \Bigg)  \nonumber \\Ê
&  \leq \prod_{j' \in [S]}   \exp\bigg( - \frac{x_{i_{j'}}^{2}}{\sigma^{2}} \bigg) \sum_{j \in [S]}  \Bigg( \prod_{j''' \in [S]Ê\setminus [j]} \!  \exp\bigg( \frac{x_{i_{j'''}}^{2}}{\sigma^{2}} \bigg) \Bigg) \Bigg( \prod_{j'' \in [j-1]}  \exp\bigg(  \frac{x_{i_{j''}}^{2}}{\sigma^{2}} \bigg) \Bigg) \nonumber \\Ê
&  \stackrel{(a)}{\leq} \Bigg( \prod_{j' \in [S]}   \exp\bigg( - \frac{x_{i_{j'}}^{2}}{\sigma^{2}} \bigg) \Bigg) \Bigg( \prod_{j \in [S]}  \exp\bigg( \frac{x_{i_{j}}^{2}}{\sigma^{2}} \bigg) \Bigg)   =1 \nonumber \\Ê
\end{align}  
where the step $(a)$ can be verified by the distributive law and the series representation $\exp\bigg( \frac{x_{i_{j}}^{2}}{\sigma^{2}} \bigg) = \sum_{l \in \mathbb{Z}_{+}} \frac{1}{l!} \Bigg( \frac{x_{i_{j}}^{2}}{\sigma^{2}} \Bigg)^{l}$. 
\end{proof}
Note that the coefficients $m_{l}$ appearing in the representation \eqref{equ_prescr_mean_diag_bias} of the prescribed mean function 
depend on the parameter vector $\mathbf{x}_{0} \in \mathcal{X}_{S}$ associated with the minimum variance problem $\mathcal{M}_{\text{\tiny{SSNM}}}$. 
Thus, we have the somewhat counterintuitive fact that for one and the same prescribed diagonal bias function $c(\mathbf{x}) = \gamma(\mathbf{x}) - x_{k}$, the corresponding coefficients $m_{l}$ 
vary with the parameter vector $\mathbf{x}_{0}$ of $\mathcal{M}_{\text{\tiny{SSNM}}}$.  

If the prescribed bias function $c(\cdot)$ is the actual bias function $b(\hat{x}'_{k}(\cdot); \mathbf{x})$ of a given diagonal estimator $\hat{x}'_{k}(\mathbf{y}) = \hat{x}'_{k}(y_{k})$ with 
finite variance at $\mathbf{x}_{0}$, i.e., $\hat{x}'_{k}(\cdot) \in \mathcal{P}(\mathcal{M}_{\text{\tiny{SSNM}}})$ (cf. \eqref{equ_def_est_finite_power}), the coefficients $m_{l}$ appearing in Corollary \ref{cor_thm_min_var_lmv_ssnm_diag_bias_ISIT} and Theorem \ref{thm_diag_bias_min_achiev_var_LMV} 
have a particular interpretation. To that end we need the following result:

\begin{lemma}
\label{lem_def_diag_finite_var_est_hilbert_space}
Consider the minimum variance problem $\mathcal{M}_{\text{\tiny{SSNM}}}=\left(\mathcal{E}_{\text{\tiny{SSNM}}},c(\cdot),\mathbf{x}_{0}\right)$ and the associated function Hilbert space $\mathcal{P}(\mathcal{M}_{\text{\tiny{SSNM}}})$ of 
finite variance estimators with inner-product 
\begin{equation} 
\langle \hat{g}_{1}(\cdot), \hat{g}_{2}(\cdot) \rangle_{\text{\tiny{RV}}} = 
 \frac{1}{(2 \pi \sigma^{2})^{N/2}} \int_{\mathbf{y}} \hat{g}_{1}(\mathbf{y}) \hat{g}_{2}(\mathbf{y}) \exp \left( - \frac{1}{2 \sigma^{2}} \| \mathbf{y} - \mathbf{x}_{0} \|^{2}_{2} \right) dÊ\mathbf{y}. 
\end{equation}
Then the subset $\mathcal{D}(\mathcal{M}_{\text{\tiny{SSNM}}}) \subseteq \mathcal{P}(\mathcal{M}_{\text{\tiny{SSNM}}})$ which consists 
only of diagonal estimators $\hat{g}(\mathbf{y}) = \hat{g}(y_{k})$ is a Hilbert subspace with induced inner product: 
\begin{equation} 
\langle \hat{g}_{1}(\cdot), \hat{g}_{2}(\cdot) \rangle_{\mathcal{D}(\mathcal{M}_{\text{\tiny{SSNM}}})} = 
 \frac{1}{ \sqrt{2 \pi} \sigma} \int_{y_{k}} \hat{g}_{1}(y_{k}) \hat{g}_{2}(y_{k}) \exp \left( - \frac{1}{2 \sigma^{2}} (y_k - x_{0,k} )^{2} \right) dÊy_{k}. 
\end{equation}

A specific ONB for $\mathcal{D}(\mathcal{M}_{\text{\tiny{SSNM}}})$ is given by $\left\{ h^{(l)}(\cdot) \right\}_{l \in \mathbb{Z}_{+}}$ with functions $h^{(l)}(\cdot): \mathbb{R}^{N} \rightarrow \mathbb{R}$ defined as 
\begin{equation}
h^{(l)}(\mathbf{y}) = \frac{1}{\sqrt{l!}} \mathsf{H}_{l}\left(\frac{y_{k} - x_{0,k}}{\sigma}\right).
\end{equation}
\end{lemma}
\begin{proof}
\cite{SzegoOrthogPoly}
\end{proof}

We have 
\begin{corollary} 
\label{cor_diag_est_min_achiev_var_LMV_ISIT}
Consider the minimum variance problem $\mathcal{M}_{\text{\tiny{SSNM}}}=\left(\mathcal{E}_{\text{\tiny{SSNM}}},c(\cdot),\mathbf{x}_{0}\right)$ for a specific choice for 
$\sigma$, $S$, $N$, $\mathbf{x}_{0} \in \mathcal{X}_{S}$ where $S <N$ and the prescribed bias $c(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}$ is given as the actual 
bias of a diagonal estimator $\hat{x}_{k}(\mathbf{y}) = \hat{x}_{k}(y_{k})$, i.e., $c(\mathbf{x}) = b(\hat{x}_{k}(\cdot); \mathbf{x})$. The estimator $\hat{x}_{k}(\mathbf{y})$ is 
assumed to have finite variance at $\mathbf{x}_{0}$, i.e., $\hat{x}_{k}(\mathbf{y}) \in \mathcal{D}(\mathcal{M}_{\text{\tiny{SSNM}}})$. 

Then we have that the prescribed mean function $\gamma(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}: \gamma(\mathbf{x}) = c(\mathbf{x}) + x_{k}= \mathsf{E}_{\mathbf{x}} \{ \hat{x}_{k}(\mathbf{y}) \}$ can be written 
in the form \eqref{equ_prescr_mean_diag_bias} with coefficients $m_{l}$ given by scaled expansion coefficients of $\hat{x}_{k}(\mathbf{y})$ w.r.t. to the ONB $\left\{ h^{(l)}(\cdot) \right\}_{l \in \mathbb{Z}_{+}}$ defined in 
Lemma \eqref{lem_def_diag_finite_var_est_hilbert_space}, i.e., 
\begin{align} 
m_{l}& = \frac{\sqrt{l!}}{\sigma^{l}} \langle \hat{x}_{k}(\cdot), h^{(l)}(\cdot) \rangle_{\mathcal{D}(\mathcal{M}_{\text{\tiny{SSNM}}})}  \nonumber \\Ê
& = \frac{1}{\sqrt{2 \pi} \sigma^{l+1}} \int_{y_{k}} \hat{x}_{k}(y_{k})   \mathsf{H}_{l}\left(\frac{y_{k} - x_{0,k}}{\sigma}\right)\exp \left( - \frac{1}{2 \sigma^{2}} (y_k - x_{0,k} )^{2} \right) dÊy_{k}.
\end{align} 

This bias $c(\cdot)$ is valid by construction and the minimum achievable variance and corresponding LMV estimator are obtained as 
\begin{equation}
\label{equ_expr_min_achiev_var_diag_est_ISIT_SSNM}
L_{\mathcal{M}_{\text{\tiny{SSNM}}}}  = v(\hat{x}_{k}(\cdot); \mathbf{x}_{0}) h(\mathbf{x}_{0}; \mathcal{I}) + \left(h(\mathbf{x}_{0}; \mathcal{I}) - 1 \right)\big(\gamma(\mathbf{x}_{0})Ê\big)^{2}
\end{equation} 
and the corresponding LMV estimator 
\begin{equation}
\label{equ_expr_LMV_diag_est_ISIT_SSNM}
\hat{x}_{k}^{(\mathbf{x}_{0})}(\mathbf{y})  = \hat{x}_{k}(y_{k})  h(\mathbf{y}, \mathbf{x}_{0}; \mathcal{I}) 
\end{equation} 
with the functions $h(\mathbf{x}; \mathcal{I})$, $h(\mathbf{y}, \mathbf{x}; \mathcal{I})$ as defined in \eqref{equ_factor_ISIT_SSNM_min_achiev_var}, \eqref{equ_factor_ISIT_SSNM_LMV} respectively.
\end{corollary} 

\begin{proof} 
The prescribed mean function can be expressed as 
\begin{align} 
\gamma(\mathbf{x}) & = \mathsf{E}_{\mathbf{x}} \{ \hat{x}_{k}(\mathbf{y}) \} = \frac{1}{\sqrt{2 \pi} \sigma}  \int_{y_{k}} \hat{x}_{k}(y_{k}) \exp \left( - \frac{1}{2 \sigma^{2}} (y_k - x_{k} )^{2} \right) d y_{k}. 
\end{align}
Since the functions $\left\{ h^{(l)}(\cdot) \right\}_{l \in \mathbb{Z}_{+}}$ form an ONB for $\mathcal{D}(\mathcal{M}_{\text{\tiny{SSNM}}})$ we have by Theorem \ref{thm_fourier_onb}: 
\begin{align}
\label{equ_bessel_series_power_diag_est_SSNM_ISIT}
\| \hat{x}_{k}(\cdot) \|^{2}_{\mathcal{D}(\mathcal{M}_{\text{\tiny{SSNM}}})} & =   P(\hat{x}_{k}(\cdot); \mathbf{x}_{0}) Ê = v(\hat{x}_{k}(\cdot); \mathbf{x}_{0}) + \left( \mathsf{E}_{\mathbf{x}_{0}} \{ \hat{x}_{k}(\mathbf{y}) \} \right)^{2} \nonumber \\Ê
& = v(\hat{x}_{k}(\cdot); \mathbf{x}_{0}) + \left( \gamma(\mathbf{x}_{0}) \right)^{2}= \sum_{l \in \mathbb{Z}_{+}} \big| \langle \hat{x}_{k}(\cdot), h^{(l)}(\cdot) \rangle_{\mathcal{D}(\mathcal{M}_{\text{\tiny{SSNM}}})} \big|^{2},  
\end{align} 
and  
\begin{equation} 
\label{equ_fourier_series_power_diag_est_SSNM_ISIT}
\lim_{L \rightarrow \infty}Ê\sum_{l \in [L] \cup \{0\}} \langle \hat{x}_{k}(\cdot), h^{(l)}(\cdot) \rangle_{\mathcal{D}(\mathcal{M}_{\text{\tiny{SSNM}}})}h^{(l)}(\cdot) = \hat{x}_{k}(\cdot). 
\end{equation} 
Another relation that can be verified easily is 
\begin{equation}
\label{equ_mean_inner_prod_diag_est_SSNM_ISIT}
\mathsf{E}_{\mathbf{x}_{0}} \{ \hat{x}_{k}(\mathbf{y}) \} = \gamma(\mathbf{x}_{0})= \langle \hat{x}_{k}(\cdot), h^{(0)}(\cdot) \rangle_{\mathcal{D}(\mathcal{M}_{\text{\tiny{SSNM}}})}. 
\end{equation} 

Differentiating the mean function $\gamma(\mathbf{x}) = \mathsf{E}_{\mathbf{x}} \{ \hat{x}_{k}(\mathbf{y}) \}$ $l$-times w.r.t. to $x_{k}$ yields 
\begin{align} 
\label{equ_part_der_inner_prod_diag_est_SSNM_ISIT}
\frac{\partial^{l \mathbf{e}_{k}} \gamma(\mathbf{x})}{\partial \mathbf{x}^{l \mathbf{e}_{k}}} \bigg|_{\mathbf{x} = \mathbf{x}_{0}} 
& \stackrel{(a)}{=}  \frac{1}{\sqrt{2 \pi} \sigma}  \int_{y_{k}} \hat{x}_{k}(y_{k}) \frac{\partial^{l} \exp \left( - \frac{1}{2 \sigma^{2}} (y_k - x_{k} )^{2} \right)}{\partial x_{k}^{l}} \bigg|_{\mathbf{x} = \mathbf{x}_{0}} d y_{k} \nonumber \\Ê
& \stackrel{(b)}{=}  \frac{1}{\sqrt{2 \pi} \sigma^{l+1}}  \int_{y_{k}} \hat{x}_{k}(y_{k})  \mathsf{H}_{l}\left( \frac{y_{k}- x_{0,k}}{\sigma} \right) \exp \left( - \frac{1}{2 \sigma^{2}} (y_k - x_{0,k} )^{2} \right) d y_{k}Ê\nonumber \\Ê
& =   \frac{\sqrt{l!}}{\sigma^{l}} \langle \hat{x}_{k}(\cdot), h^{(l)}(\cdot) \rangle_{\mathcal{D}(\mathcal{M}_{\text{\tiny{SSNM}}})},
\end{align} 
where $(a)$ can be verified by a standard argument using the dominated convergence theorem \cite{FundmentExpFamBrown,RudinBookPrinciplesMatheAnalysis,HalmosMeasure} and 
$(b)$ can be verified by a calculation similar to \eqref{equ_proof_main_thm_diag_bias_SSNM_cases_identiy_case_1_hermite}. 
From \eqref{equ_bessel_series_power_diag_est_SSNM_ISIT} (implying that the inner products $ \langle \hat{x}_{k}(\cdot), h^{(l)}(\cdot) \rangle_{\mathcal{D}(\mathcal{M}_{\text{\tiny{SSNM}}})}$ must be bounded) and \eqref{equ_part_der_inner_prod_diag_est_SSNM_ISIT} it follows by Taylor's theorem \cite{RudinBookPrinciplesMatheAnalysis} that the mean function can be written as a power series in the form \eqref{equ_prescr_mean_diag_bias} with coefficients $m_{l} =  \frac{\sqrt{l!}}{\sigma^{l}} \langle \hat{x}_{k}(\cdot), h^{(l)}(\cdot) \rangle_{\mathcal{D}(\mathcal{M}_{\text{\tiny{SSNM}}})}$. 
The relation \eqref{equ_expr_min_achiev_var_diag_est_ISIT_SSNM} follows then from \eqref{equ_expr_min_achiev_var_ISIT_SSNM} via \eqref{equ_bessel_series_power_diag_est_SSNM_ISIT} and \eqref{equ_mean_inner_prod_diag_est_SSNM_ISIT}. 
Finally, the relation \eqref{equ_expr_LMV_diag_est_ISIT_SSNM} follows from \eqref{equ_expr_LMV_diag_bias_ISIT_SSNM} by \eqref{equ_fourier_series_power_diag_est_SSNM_ISIT}. 
\end{proof} 
Note that Corollary \ref{cor_diag_est_min_achiev_var_LMV_ISIT} also applies to unbiased estimation where $c(\cdot) \equiv 0$ and $\gamma(\mathbf{x}) = x_{k}$, since this is the bias and mean function of the 
ordinary LS estimator $\hat{x}_{\text{\tiny{LS}},k}(\mathbf{y}) = y_{k}$ which obviously is diagonal and has finite variance at $\mathbf{x}_{0}$. 

%Let us consider the application of Theorem \ref{thm_diag_bias_min_achiev_var_LMV} to the case of unbiased estimation, i.e., we choose the prescribed bias $c(\cdot) \equiv 0$. The 
%prescribed mean function is then given as $\gamma(\mathbf{x}) = c(\mathbf{x}) + x_{k} = x_{k}$. Thus we can apply Theorem \ref{thm_diag_bias_min_achiev_var_LMV} 
%with $m_{l}$ in \eqref{equ_prescr_mean_diag_bias} being zero for all $l$ except for $l\in \{0,1\}$ where $m_{0} = x_{0,k}$ and $m_{1} = 1$. 
%Note that this bias function is obviously valid by \eqref{equ_cond_valid_bias_diagon_bias_SSNM} since the expansion coefficients $m_{l}$ are zero for every $l>1$. 
Remarkably, according to Corollary \ref{cor_diag_est_min_achiev_var_LMV_ISIT} every diagonal estimator $\hat{x}'_{k}(\cdot): \mathbb{R}^{N} \rightarrow \mathbb{R}$ for the SSNM with finite variance at $\mathbf{x}_{0} \in \mathcal{X}_{S}$ is 
necessarily the LMV estimator for the minimum variance problem $\mathcal{M}_{\text{\tiny{SSNM}}}=\left(\mathcal{E}_{\text{\tiny{SSNM}}},c(\mathbf{x})=,\mathbf{x}_{0}\right)$ whenever $|\supp(\mathbf{x}_{0}) \cup \{ k \}| < S +1$, irrespective of the sparsity degree $S$.
Thus, in this case the sparsity constraints do not help anything with regard to minimum variance estimation, i.e., the estimator $\hat{x}'_{k}(\cdot)$ is the LMV estimator for any parameter set $\mathcal{X}_{S}$ including the non-sparse case $\mathcal{X} = \mathbb{R}^{N}$ 
and the variance $v(\hat{x}'_{k}(\cdot);\mathbf{x}_{0})$ coincides with the minimum achievable variance $L_{\mathcal{M}_{\text{\tiny{SSNM}}}}$, i.e., the Barankin bound. 
%We have for the case $$ by Theorem \ref{thm_diag_bias_min_achiev_var_LMV} that the minimum achievable variance 
%of any unbiased estimator, i.e., the unbiased Barankin bound, is given by 
%\begin{equation} 
%\label{equ_min_achiev_var_non_zero_coeff_ssnm}
%L_{\mathcal{M}_{\text{\tiny{SSNM}}}}  = \sigma^{2}
%\end{equation} 
%and the corresponding LMVU estimator is 
%\begin{equation}
%\label{equ_lmvu_ssnm}
%\hat{x}_{k}^{(\mathbf{x}_{0})}(\mathbf{y}) = y_{k}.
%\end{equation} 
%Since the estimator in \eqref{equ_lmvu_ssnm} is also the LMVU for the LGM (i.e., for $S=N$) with $\mathbf{H}=\mathbf{I}$ we have that for $\| \mathbf{x}_{0} \|_{0} < S$ and arbitrary $k \in [N]$, or $\| \mathbf{x}_{0} \|_{0}=S$, $k \in \supp(\mathbf{x}_{0})$ 
%the sparsity constraints on the parameter vector, i.e., the a-priori knowledge that $\mathbf{x} \in \mathcal{X}$, does not help anything with regard to minimum variance unbiased estimation.
%However, for the case $\| \mathbf{x}_{0} \|_{0}=S$, $k \notin \supp(\mathbf{x}_{0})$ we obtain for the minimum achievable variance, i.e., the unbiased Barankin bound, 
%\begin{equation}
%\label{equ_min_achiev_var_zero_coeff_ssnm}
%L_{\mathcal{M}_{\text{\tiny{SSNM}}}}  = \sigma^{2} \left( \sum_{j \in [S]} \exp\bigg( - \frac{x_{0,j}^{2}}{\sigma^{2}} \bigg) \prod_{j' \in [j-1]}  \bigg(Ê\! 1 \! -\! \exp\bigg( -\frac{x_{0,j'}^{2}}{\sigma^{2}} \bigg) \! \bigg)Ê\right)
%\end{equation} 
%with corresponding LMVU estimator 
%\begin{equation} 
%\label{equ_lmvu_zero_coeff_ssnm}
%\hat{x}_{k}^{(\mathbf{x}_{0})}(\mathbf{y}) = 
%y_{k} \sum_{j \in [S]} \exp\bigg( \! \frac{-x_{0,j}^{2}-2y_{j}x_{0,j}}{2 \sigma^{2}} \! \bigg)
% \prod_{j' \in [j-1]}  \bigg(Ê\! 1 \! -\! \exp\bigg(\!-\!\frac{x_{0,j'}^{2}+2y_{j'}x_{0,j'}}{2Ê\sigma^{2}} \! \bigg) \! \bigg).
%\end{equation} 

However, whenever $|\supp(\mathbf{x}_{0}) \cup \{ k \}| =S+1$ we have by Corollary \ref{cor_diag_est_min_achiev_var_LMV_ISIT} and the inequality in \eqref{equ_factor_ISIT_SSNM_min_achiev_var}, that there are estimators with the same bias and mean as $\hat{x}'_{k}(\cdot)$ 
but with a smaller variance at $\mathbf{x}_{0}$. The LMV estimator that achieves the minimum variance at $\mathbf{x}_{0}$ is obtained by a multiplication of the estimator $\hat{x}'_{k}(\mathbf{y})=\hat{x}'_{k}(y_{k})$ with a ``correction'' factor $h(\mathbf{y},\mathbf{x}_{0}; \mathcal{I})$ that 
does not depend on $y_{k}$ (as can be verified easily). Note that by a straightforward calculation one can show that the LMV estimator in \eqref{equ_expr_LMV_diag_est_ISIT_SSNM} is robust against deviations from the nominal parameter $\mathbf{x}_{0}$. In particular, the estimator given by \eqref{equ_expr_LMV_diag_est_ISIT_SSNM} has always finite mean 
and variance for any parameter vector $\mathbf{x} \in \mathbb{R}^{N}$ and the statistical model of the LGM with $\mathbf{H} = \mathbf{I}$. 

%Since in this case $L_{\mathcal{M}_{\text{\tiny{SSNM}}}}$ is strictly smaller (as can be verified easily using the proof of Theorem \ref{thm_diag_bias_min_achiev_var_LMV}) than the minimum achievable variance for the LGM with $\mathbf{H} = \mathbf{I}$ we have that 
%for $\| \mathbf{x}_{0} \|_{0}=S$, $k \notin \supp(\mathbf{x}_{0})$, i.e., the estimation of a coefficient $x_{k}$ that is not in the support of the fixed parameter vector $\mathbf{x}_{0}$ which 
%has $S$ non-zeros, the minimum achievable variance for unbiased estimators is strictly smaller than for the corresponding estimation problem without sparsity constraints. Moreover, 
%we have by \eqref{equ_lmvu_zero_coeff_ssnm} an explicit expression for the LMVU that is unbiased for all $\mathbf{x} \in \mathcal{X}_{S}$ and whose variance at $\mathbf{x}_{0}$ is equal to 
%$L_{\mathcal{M}_{\text{\tiny{SSNM}}}}$ in \eqref{equ_min_achiev_var_zero_coeff_ssnm}. Note that the expressions on the RHS of \eqref{equ_min_achiev_var_zero_coeff_ssnm} and \eqref{equ_min_achiev_var_non_zero_coeff_ssnm} are nothing but the (unbiased) Barankin bound for the SSNM. We also have trivially from \eqref{equ_lmvu_ssnm} and \eqref{equ_lmvu_zero_coeff_ssnm} that there does not exist a UMVU for the SSNM with $S< N$ since the LMVU depends on the parameter vector $\mathbf{x}_{0}$ associated with the 
%minimum variance problem $\mathcal{M}_{\text{\tiny{SSNM}}}$. The non-existence of a UMVU for the SSNM with $S < N$ has also been proven in a different way in \cite{AlexZvikaICASSP,AlexZvikaJournal}. 

%\subsection{Barankin Bound and LMVU estimator} 
%\subsection{Nonexistence of UMVU estimator for $S < N$} 
%The non-existence of a UMVU estimator is a straight consequence of the fact that for $S < N$ the LMVU depends on $\mathbf{x}_{0}$. 
%\subsection{Existence of a UMV estimator} 
%Regarding the existence of a UMV estimator for the estimation problem $\mathcal{E}_{\text{\tiny{SLM}}}$ and a prescribed bias function $c(\cdot)$ we state 
%\begin{theorem}
%Consider a prescribed bias function that is valid for $\mathcal{M}_{\text{\tiny{SSNM}}}(\mathbf{x}_{0})$ for any $\mathbf{x}_{0} \in \mathcal{X}$.  
%\end{theorem} 
%\section{Conditions for the Existence of a UMV estimator} 
%\label{sec_exist_UMV_SLM}


%\section{Special case: Compressed Sensing} 
%\label{sec_SLM_CS} 



\section{Necessity of Strict Sparsity} 
\label{sec_strict_sparstiy_SLM}

In what follows we consider the SLM $\mathcal{E}_{\text\tiny{SLM}}$ and the LGM $\mathcal{E}_{\text{\tiny{LGM}}}$ with the same fixed choice for $\sigma$, $M$, $N$ and $\mathbf{H}$. 
Lets consider then the associated minimum variance problems $\mathcal{M}_{\text{\tiny{SLM}}}= \left( \mathcal{E}_{\text\tiny{SLM}},c'(\cdot), \mathbf{x}_{0} \right)$ and $\mathcal{M}_{\text{\tiny{LGM}}}= \left( \mathcal{E}_{\text\tiny{LGM}},c(\cdot), \mathbf{x}_{0} \right)$ with 
the same parameter vector $\mathbf{x}_{0} \in \mathcal{X}_{S}$ and the prescribed bias $c'(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}$ given by the restriction of $c(\cdot): \mathbb{R}^{N} \rightarrow \mathbb{R}$, i.e, $c'(\cdot) = c(\cdot) \big|_{\mathcal{X}_{S}}$. 
%In the following we will consider one specific but arbitrary choice for the system matrix $\mathbf{H}$ and dimension $N$ for the SLM $\mathcal{E}_{\text\tiny{SLM}}$ and LGM $\mathcal{E}_{\text{\tiny{LGM}}}$ (cf. \eqref{equ_linear_observation_model}). 
In particular we do not require that $\mathbf{H}$ satisfies \eqref{equ_spark_cond}. 

Since the SLM for $S <N$ is obtained by reducing the parameter set $\mathcal{X} = \mathbb{R}^{N}$ of the LGM $\mathcal{E}_{\text{\tiny{LGM}}}$ to the 
set of $S$-sparse vectors $\mathcal{X}_{S}$, we have that the set of allowed estimators for $\mathcal{M}_{\text{\tiny{SLM}}}$ given by $\mathcal{F}(\mathcal{M}_{\text{\tiny{SLM}}})$ (cf. \eqref{equ_est_finite_var_prescr_bias}) in general becomes larger than 
the set of allowed estimators for $\mathcal{M}_{\text{\tiny{LGM}}}$ given by $\mathcal{F}(\mathcal{M}_{\text{\tiny{LGM}}})$, i.e., $\mathcal{F}(\mathcal{M}_{\text{\tiny{SLM}}}) \supseteq \mathcal{F}(\mathcal{M}_{\text{\tiny{LGM}}})$. 

It is this increase of the set of allowed estimators that causes the minimum achievable variance $L_{\mathcal{M}_{\text{\tiny{SLM}}}}$ (with $S < N$) to be smaller than $L_{\mathcal{M}_{\text{\tiny{LGM}}}}$ in general. An important exception to this 
rule is the special case of an affine prescribed bias, i.e., $c(\mathbf{x}) = \mathbf{a}^{T} \mathbf{x} + b$ with a fixed vector $\mathbf{a} \in \mathbb{R}^{N}$ and number $b \in \mathbb{R}$, and a full column rank system matrix $\mathbf{H}$ 
where the bound in Theorem \ref{thm_CRB_SLM} for the case $\| \mathbf{x}_{0} \|_{0} < S$ coincides with $L_{\mathcal{M}_{\text{\tiny{LGM}}}}$. 

Note that the reduction from the parameter set $\mathcal{X} = \mathbb{R}^{N}$ of the LGM $\mathcal{E}_{\text{\tiny{LGM}}}$ to the parameter set $\mathcal{X} = \mathcal{X}_{S}$ of the SLM $\mathcal{E}_{\text{\tiny{SLM}}}$ with $S < N$ is rather large, 
since the Lesbegue measure of $\mathcal{X}_{S}$ (with $S < N$) is zero w.r.t. to $\mathbb{R}^{N}$ \cite{HalmosMeasure}. 

Intuitively, it should make not a big difference if we relax the constraint $\mathbf{x} \in \mathcal{X}_{S}$ and include 
also approximately $S$-sparse vectors in the parameter set. Thus we prescribe the estimator bias not only for strictly but also for approximately $S$-sparse vectors.  

A specific definition of approximate $S$-sparsity is used e.g. in \cite{WainwrightMinimaxSLM, DonohoJohnstone94,Donoho94idealspatial} where the authors model the set of approximately 
$S$-sparse vectors by an $\ell_{q}$ ball with $q \leq 1$ and radius $S$. The $\ell_{q}$ ball $\mathcal{B}_{q}(S)$ with radius $S$ is defined by 
\begin{equation}
\label{equ_def_approximate_S_sparse_vecs_q_ball} 
\mathcal{B}_{q}(S)Ê\triangleq \bigg \{ \mathbf{x}' \in \mathbb{R}^{N} \big|  \| \mathbf{x}' \|^{q}_{q} \leq S \bigg\}.
\end{equation} 

Note that the set of strictly sparse vectors $\mathcal{X}_{S}$ is obtained as the limiting case when $q=0$, i.e., $\mathcal{X}_{S} = \mathcal{B}_{0}(S)$. 
\begin{figure}[htbp]
\begin{center}
\subfigure[]
{\label{fig_B_q_0}
\pspicture(-2.5,-2.5)(2.5,2.5) 
\psline[linewidth=2pt](-2,0)(2,0)
\psline[linewidth=2pt](0,-2)(0,2) % y-axis 
\endpspicture
}
\hspace*{2cm}
\subfigure[]
{\label{fig_B_q_0_25}
\pspicture(-2.5,-2.5)(2.5,2.5) 
\psline[linewidth=0.5pt](-2,0)(2,0)
\psline[linewidth=0.5pt](0,-2)(0,2) % y-axis 
\pscustom[fillcolor=lightgray, fillstyle=solid]{
\psplot[linewidth=0.1pt,plotpoints=300]{-1.5}{1.5} {1.5 0.25 exp x abs 0.25 exp  sub 4 exp}
\psplot[linewidth=0.1pt,plotpoints=300]{1.5}{-1.5} {1.5 0.25 exp x abs 0.25 exp  sub 4 exp -1 mul}
%\pscurve{1.5
}
\endpspicture
} \\
\subfigure[]
{%\vspace*{1cm}
\label{fig_B_q_0_75}
\pspicture(-2.5,-2.5)(2.5,2.5) 
\psline[linewidth=0.5pt](-2,0)(2,0)
\psline[linewidth=0.5pt](0,-2)(0,2) % y-axis 
\pscustom[fillcolor=lightgray, fillstyle=solid]{
\psplot[linewidth=0.1pt,plotpoints=300]{-1.5}{1.5} {1.5 0.75 exp x abs 0.75 exp  sub 1.333 exp}
\psplot[linewidth=0.1pt,plotpoints=300]{1.5}{-1.5} {1.5 0.75 exp x abs 0.75 exp  sub 1.333 exp -1 mul}
%\pscurve{1.5
}
\endpspicture
}
\hspace*{2cm}
\subfigure[]
{%\vspace*{1cm}
\label{fig_B_q_1}
\pspicture(-2.5,-2.5)(2.5,2.5) 
\psline[linewidth=0.5pt](-2,0)(2,0)
\psline[linewidth=0.5pt](0,-2)(0,2) % y-axis 
\pscustom[fillcolor=lightgray, fillstyle=solid]{
\psplot[linewidth=0.1pt,plotpoints=300]{-1.5}{1.5} {1.5 1 exp x abs 1 exp  sub 1 exp}
\psplot[linewidth=0.1pt,plotpoints=300]{1.5}{-1.5} {1.5 1 exp x abs 1 exp  sub 1 exp -1 mul}
%\pscurve{1.5
}
\endpspicture
}
\end{center}
\caption{Different parameter sets consisting of strictly and approximate $1$-sparse 
vectors $\mathbf{x} \in \mathbb{R}^{2}$.  \subref{fig_B_q_0} $ \mathcal{X}= \mathcal{B}_{q=0}(1) = \mathcal{X}_{S=1}$. 
\subref{fig_B_q_0_25} $ \mathcal{X} = \mathcal{B}_{q=0.25}(1)$. \subref{fig_B_q_0_75} $ \mathcal{X} = \mathcal{B}_{q=0.75}(1)$. \subref{fig_B_q_1} $ \mathcal{X} = \mathcal{B}_{q=1}(1).$}
\label{fig_approx_sparse_par_set}
\end{figure}
In Figure \ref{fig_approx_sparse_par_set} we illustrate for $N=2$, $S=1$ the parameter sets given by $\mathcal{B}_{q}(S)$ for various $q$. 
\begin{figure} 
\end{figure}
Note that in contrast to $\mathcal{X}_{S}$ the parameter sets $\mathcal{B}_{q}(S)$ are bounded for $q>0$.

Let us now define a minimum variance problem $\mathcal{M}^{(q)} = \left( \mathcal{E}^{(q)}, c(\cdot) \big|_{\mathcal{B}_{q}(S)}, \mathbf{x}_{0} \right)$ associated with the estimation problem $\mathcal{E}^{(q)} \triangleq \left( \mathcal{B}_{q}(S), f_{\text{\tiny{LGM}}, \mathbf{H}}(\mathbf{y}; \mathbf{x}), g(\mathbf{x}) = x_{k} \right)$, with the same choices for $c(\cdot)$, $\mathbf{x}_{0}$ and $\mathbf{H}$ as for $\mathcal{M}_{\text{\tiny{SLM}}}$. Then, one might expect that for $q \rightarrow 0$, i.e., when $B_{q}(S) \rightarrow \mathcal{X}_{S}$ we should have 
$L_{\mathcal{M}^{(q)}} \rightarrow L_{\mathcal{M}_{\text{\tiny{SLM}}}}$. 

Despite the intuition that a change of the parameter set from $\mathcal{X}_{S}$ to $\mathcal{B}_{q}(S)$ with small $q>0$, i.e., considering $\mathcal{M}^{(q)}$ instead of $\mathcal{M}_{\text{\tiny{SLM}}}$, should make not a big difference, the next result 
tells us that for minimum variance estimation it makes a very big difference if we use $\mathcal{X}_{S}$ or $\mathcal{B}_{q}(S)$ no matter how small $q$ is:  
%The following result shows that concerning minimum variance esitmation there is a fundamental difference between the parameter set $\mathcal{X}_{S}$ 
%and a parameter set $\mathcal{X} = \mathcal{B}_{q}(S)$ with $q > 0$: 
\begin{theorem}
\label{thm_strict_sparsity_nec_SLM} 
Consider the estimation problem $\mathcal{E}' = \left(\mathcal{X}, f_{\text{\tiny{LGM}},\mathbf{H}}(\mathbf{y}; \mathbf{x}), g(\mathbf{x}) = x_{k} \right)$ that coincides 
with the LGM $\mathcal{E}_{\text{\tiny{LGM}}}$ except for the parameter set $\mathcal{X} \subseteq \mathbb{R}^{N}$. 

We then define two minimum variance problems $\mathcal{M}'=\left(\mathcal{E}', c'(\cdot), \mathbf{x}_{0}Ê\right)$ and $\mathcal{M}_{\text{\tiny{LGM}}} = \left( \mathcal{E}_{\text{\tiny{LGM}}}, c(\cdot), \mathbf{x}_{0} \right)$
that are identical, except for the parameter set of their estimation problems and the prescribed bias functions which are assumed to 
be valid for the corresponding minimum variance problem. 

Furthermore, we assume that the prescribed bias function $c'(\cdot): \mathcal{X} \rightarrow \mathbb{R}$ of $\mathcal{M}'$ is 
the restriction of the prescribed bias function $c(\cdot): \mathbb{R}^{N} \rightarrow \mathbb{R}$ of $\mathcal{M}_{\text{\tiny{LGM}}}$ to the sub-domain $\mathcal{X} \subseteq \mathbb{R}^{N}$, i.e., 
\begin{equation}
c_{0}(\cdot) = c(\cdot) \big|_{\mathcal{X}}.  
\end{equation} 

If the parameter set $\mathcal{X}$ contains an open ball $\mathcal{B}(\mathbf{x}_{c},r)$ with some radius $r>0$ and center $\mathbf{x}_{c} \in \mathcal{X}$, i.e., 
\begin{equation} 
\label{equ_thm_strict_spar_nec_contains_ball}
\mathcal{B}(\mathbf{x}_{c},r) \subseteq \mathcal{X}
\end{equation}
then we have that 
\begin{equation}
L_{\mathcal{M}'} = L_{\mathcal{M}_{\text{\tiny{LGM}}}}.
\end{equation}
\end{theorem} 
\begin{proof} 
We will denote the prescribed means of the minimum variance problems by $\gamma'(\cdot): \mathcal{X} \rightarrow \mathbb{R}: \gamma'(\mathbf{x}) \triangleq c'(\mathbf{x}) + x_{k}$ and $\gamma(\cdot): \mathbb{R}^{N} \rightarrow \mathbb{R}: \gamma(\mathbf{x}) \triangleq c(\mathbf{x}) + x_{k}$ respectively. 
Note that the assumption that $c(\cdot)$ is valid for $\mathcal{M}_{\text{\tiny{LGM}}}$ already implies that the bias function $c'(\cdot) = c(\cdot) \big|_{\mathcal{X}}$ is valid for $\mathcal{M}'$ due to Theorem \ref{thm_reducing_domain_RKHS} 
We then have that $\gamma'(\cdot) \in \mathcal{H}(\mathcal{M}')$ and $\gamma(\cdot) \in  \mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}})$. 

Since the kernel $R_{\mathcal{M}'}(\cdot,\cdot)$ is the restriction of the kernel $R_{\mathcal{M}_{\text{\tiny{LGM}}}}(\cdot,\cdot)$ to the sub-domain $\mathcal{X} \times \mathcal{X}$, i.e., 
$R_{\mathcal{M}'}(\cdot,\cdot) = R_{\mathcal{M}_{\text{\tiny{LGM}}}}(\cdot,\cdot)\big|_{\mathcal{X} \times \mathcal{X}}$, we have by
Theorem \ref{thm_main_facts_RKHS_MVE}, Theorem \ref{thm_reducing_domain_RKHS} and the obvious fact $\gamma'(\cdot) = \gamma(\cdot) \big|_{\mathcal{X}}$ that
\begin{equation} 
\label{equ_min_var_strict_spar_nec}
L_{\mathcal{M}'}  = \min_{\gamma'' (\cdot) \in \mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}}) }\| \gamma'' (\cdot)+ \gamma(\cdot) \|^{2}_{\mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}})} \quad \mbox{s.t.} \quad \gamma''(\mathbf{x}) = 0 \,\, \forall \mathbf{x} \in \mathcal{X}. 
\end{equation}
Using Theorem \ref{thm_isometry_LGM} we can reformulate \eqref{equ_min_var_strict_spar_nec} as 
\begin{equation} 
L_{\mathcal{M}'}  = \min_{\gamma''(\cdot) \in \mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}})}\| \mathsf{K}_{g}[\gamma''(\cdot) + \gamma(\cdot)] \|^{2}_{\mathcal{H}(R_{g}^{(D)})} \quad \mbox{s.t.} \quad \gamma''(\mathbf{x}) = 0 \,\, \forall \mathbf{x} \in \mathcal{X}
\end{equation}
with $D = \rank(\mathbf{H})$. 

Consider an arbitrary $\gamma''(\cdot) \in \mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}})$ which vanishes for every $\mathbf{x} \in \mathcal{X}$. We then have due to \eqref{equ_thm_strict_spar_nec_contains_ball} that 
$\mathsf{K}_{g}[\gamma''(\cdot)](\mathbf{x}')$ vanishes for every $\mathbf{x}' \in \mathcal{B}(\widetilde{\mathbf{H}} \mathbf{x}_{c},r_{1}) \subseteq \mathbb{R}^{D}$ 
with a specific radius $r_{1} >0$ and centered at $\widetilde{\mathbf{H}} \mathbf{x}_{c}$, where $\widetilde{\mathbf{H}}$ is defined as in Theorem \ref{thm_isometry_LGM}. 
From this it follows via Theorem \ref{thm_part_der_any_origin_complete_R_g} that 
\begin{align}
L_{\mathcal{M}'}  & = \min_{\gamma''(\cdot) \in \mathcal{H}(\mathcal{M}_{\text{\tiny{LGM}}})}\| \mathsf{K}_{g}[\gamma''(\cdot) + \gamma(\cdot)] \|^{2}_{\mathcal{H}(R_{g}^{(D)})} \quad \mbox{s.t.} \quad \gamma''(\mathbf{x}) = 0 \,\, \forall \mathbf{x} \in \mathcal{X} \\Ê
				& =  \| \mathsf{K}_{g}[\gamma(\cdot)] \|^{2}_{\mathcal{H}(R_{g}^{(D)})} = L_{\mathcal{M}_{\text{\tiny{LGM}}}}
\end{align}
where for the last step we used again Theorem \ref{thm_isometry_LGM}. 
\end{proof}

Since we have obviously that the parameter set $\mathcal{X} = \mathcal{B}_{q}(S)$ satisfies \eqref{equ_thm_strict_spar_nec_contains_ball} for any $q>0$, Theorem \ref{thm_strict_sparsity_nec_SLM} implies that 
$L_{\mathcal{M}^{(q)}} = L_{\mathcal{M}_{\text{\tiny{LGM}}}}$ for any $q>0$. Thus the minimum achievable variance for $\mathcal{M}^{(q)}$ with $q >0$ is always equal to that of the minimum variance problem $\mathcal{M}_{\text{\tiny{LGM}}}$ which 
does not include any sparsity constrains since its parameter set is given by $\mathcal{X} = \mathbb{R}^{N}$. Furthermore since in general $ L_{\mathcal{M}_{\text{\tiny{LGM}}}} >  L_{\mathcal{M}_{\text{\tiny{SLM}}}}$ we have also 
in general that $L_{\mathcal{M}^{(q)}}$ does not converge to $L_{\mathcal{M}_{\text{\tiny{SLM}}}}$ as $q$ goes to zero. 


\section{The SLM Viewpoint on CS}
\label{sec_slm_viewpoint_CS}
The compressive measurement process of a CS application is often described by a linear measurement equation in the form 
\cite{JustRelax,GreedisGood,Can06a,ZvikaCoherenceTSP,MallatBook}
\begin{equation}
\label{equ_measurment_equ_CS}
\mathbf{y} = \mathbf{M} \mathbf{x} + \mathbf{n} 
\end{equation} 
where $\mathbf{y} \in \mathbb{R}^{M}$ denotes the compressive measurements, $\mathbf{M} \in \mathbb{R}^{M \times N}$ denotes the CS measurement matrix, the signal or parameter vector $\mathbf{x} \in \mathbb{R}^{N}$ is 
assumed to be sparse and $\mathbf{n}$ represents some additive measurement noise. 

Any CS recovery method, e.g. the ``Basis Pursuit'' (BP) (cf. \cite{JustRelax}) or the ``Orthogonal Matching Pursuit'' (OMP) (cf. \cite{GreedisGood}), can be interpreted as an estimator $\hat{\mathbf{x}}(\mathbf{y})$ that aims to estimate the sparse vector $\mathbf{x}$ using 
the observation $\mathbf{y}$ given by \eqref{equ_measurment_equ_CS}. 

If the vector $\mathbf{n} \in \mathbb{R}^{M}$ in \eqref{equ_measurment_equ_CS} is assumed to be AWGN, i.e., $\mathbf{n} \sim \mathcal{N}(\mathbf{0}, \sigma^{2} \mathbf{I})$, then the CS measurement equation \eqref{equ_measurment_equ_CS} is nothing but the observation model of the SLM (cf. \eqref{equ_linear_observation_model}) with the system matrix $\mathbf{H}$ being the CS measurement matrix $\mathbf{M}$.  

In general it is infeasible to characterize the measurement matrix $\mathbf{M}$ in an exact analytic manner, due to the large dimension (typically $M \geq 10$ and $NÊ\geq 100$). Instead 
one can use an incomplete characterization via the concept of (mutual) coherence and the restricted isometry property (cf. \cite{JustRelax,GreedisGood,Can06a,ZvikaCoherenceTSP}) which we will now define precisely.
\begin{definition}
Given a matrix $\mathbf{M} \in \mathbb{R}^{M \times N}$ we define its coherence, denoted by $\mu(\mathbf{M})$, as 
\begin{equation} 
\mu(\mathbf{M}) \triangleq \max\limits_{i \neq j} | \mathbf{m}_{j}^{T} \mathbf{m}_{i} |. 
\end{equation} 
where $\mathbf{m}_{i} \in \mathbb{R}^{M}$ denotes the $i$th column of the matrix $\mathbf{M} \in \mathbb{R}^{M \times N}$. 
\end{definition} 
\begin{definition} 
A matrix $\mathbf{M} \in \mathbb{R}^{M \times N}$ is said to satisfy the restricted isometry property (RIP) of order $K$ 
with parameter $\delta_{K} \in \mathbb{R}_{+}$ if for every index set $\mathcal{I}Ê\subseteq [N]$ of size $K$, i.e., $|\mathcal{I}| = K$, we have 
\begin{equation} 
(1-\delta_{K}) \| \mathbf{z} \|^{2}_{2} \leq \| \mathbf{M}_{\mathcal{I}} \mathbf{z} \|^{2}_{2} \leq (1+\delta_{K}) \| \mathbf{z} \|^{2}_{2}
\end{equation}
for every $\mathbf{z} \in \mathbb{R}^{K}$. 
\end{definition}
It can be straightforwardly shown that one has $\delta_{K} \leq \delta_{K'}$ if $K' \geq K$. 

While the coherence of a matrix can be calculated more efficiently than the RIP constant $\delta_{K}$ (cf. \cite{ZvikaCoherenceTSP}) it is 
a coarser description of the matrix $\mathbf{M}$ than the RIP constants. However, as stated in \cite{ZvikaCoherenceTSP} we have the following relation between these two concepts: 
\begin{theorem}
Given a matrix $\mathbf{M}$ with coherence $\mu(\mathbf{M})$ we have that the RIP constant $\delta_{K}$ satisfies 
\begin{equation} 
\label{equ_bound_coherence_RIP}
\delta_{K} \leq (K-1) \mu(\mathbf{M}). 
\end{equation} 
\end{theorem} 
\begin{proof}
\cite{ZvikaCoherenceTSP}
\end{proof}

%In the following we will make use of 
%\begin{theorem}
%\label{thm_RIP_sing_values_product}
%Consider a matrix $\mathbf{M} \in \mathbb{R}^{M \times N}$ that satisfies the RIP of order $2S$ with RIP constant $\delta_{2S} < 1$. 
%Then we have for any pair of sub-matrices $\mathbf{M}_{\mathcal{K}_{1}}$ and $\mathbf{M}_{\mathcal{K}_{2}}$, obtained 
%by index sets $\mathcal{K}_{1}, \mathcal{K}_{2} \subseteq [N]$ which satisfy $\mathcal{K}_{1} \cap \mathcal{K}_{2} = \emptyset$, $| \mathcal{K}_{1} \cup \mathcal{K}_{2}| \leq 2S$, 
%that the magnitude of the singular values of the matrix $\mathbf{M}_{\mathcal{K}_{2}}^{T} \mathbf{M}_{\mathcal{K}_{1}}$ is upper bounded by $\delta_{2S}+\delta_{S}$. 
%%\begin{equation}
%%-(\delta_{2S}+ \delta_{S}) (\| \mathbf{x}_{1} \|^{2}_{2}+\| \mathbf{x}_{2} \|^{2}_{2}) \leq 2\mathbf{x}_{2}^{T} \mathbf{M}_{\mathcal{K}_{2}}^{T} \mathbf{M}_{\mathcal{K}_{1}} \mathbf{x}_{1}   \leq (\delta_{2S}+ \delta_{S}) (\| \mathbf{x}_{1} \|^{2}_{2}+\| \mathbf{x}_{2} \|^{2}_{2}) 
%%\end{equation}
%\end{theorem}
%\begin{proof} 
%Consider an arbitrary vector $\mathbf{x} \in \mathbb{R}^{N}$ with $\supp(\mathbf{x}) = \mathcal{K}_{1} \cup \mathcal{K}_{2}$, 
%where $\mathcal{K}_{1} \cap \mathcal{K}_{2} = \emptyset$, $|\mathcal{K}_{1} \cup \mathcal{K}_{2}| \leq 2S$ 
%and denote the sub-vectors corresponding to the indices in $\mathcal{K}_{1}$ and $\mathcal{K}_{2}$ by $\mathbf{x}_{1} \in \mathbb{R}^{|\mathcal{K}_{1}|}$ and $\mathbf{x}_{2} \in \mathbb{R}^{|\mathcal{K}_{2}|}$ respectively. 
%We then have  
%\begin{align} 
%\hspace*{-5mm} (1-\delta_{2S}) \| \mathbf{x} \|^{2}_{2} & \leq \| \mathbf{M} \mathbf{x} \|^{2}_{2}  \leq (1+\delta_{2S}) \| \mathbf{x} \|^{2}_{2} \label{equ_proof_svd_rip_1} \\ 
%\hspace*{-5mm} (1-\delta_{2S}) \| \mathbf{x} \|^{2}_{2} & \leq \| \mathbf{M} (\mathbf{x}^{\mathcal{K}_{1}} +\mathbf{x}^{\mathcal{K}_{2}}) \|^{2}_{2}  \leq (1+\delta_{2S}) \| \mathbf{x} \|^{2}_{2}  \label{equ_proof_svd_rip_2}\\ 
%\hspace*{-5mm} (1-\delta_{2S}) \| \mathbf{x} \|^{2}_{2} & \leq \| \mathbf{M}_{\mathcal{K}_{1}} \mathbf{x}_{1} \|^{2}_{2}+  \| \mathbf{M}_{\mathcal{K}_{2}} \mathbf{x}_{2} \|^{2}_{2} + 2\mathbf{x}_{2}^{T} \mathbf{M}_{\mathcal{K}_{2}}^{T} \mathbf{M}_{\mathcal{K}_{1}} \mathbf{x}_{1}   \leq (1+\delta_{2S}) \| \mathbf{x} \|^{2}_{2}  \label{equ_proof_svd_rip_3}\\ 
%\hspace*{-5mm} -(\delta_{2S}+ \delta_{S}) \| \mathbf{x} \|^{2}_{2} & \leq 2\mathbf{x}_{2}^{T} \mathbf{M}_{\mathcal{K}_{2}}^{T} \mathbf{M}_{\mathcal{K}_{1}} \mathbf{x}_{1}   \leq (\delta_{2S}+ \delta_{S}) \| \mathbf{x} \|^{2}_{2} \label{equ_proof_svd_rip_4} \\ 
%\hspace*{-5mm} -(\delta_{2S}+ \delta_{S}) (\| \mathbf{x}_{1} \|^{2}_{2}+\| \mathbf{x}_{2} \|^{2}_{2}) & \leq 2\mathbf{x}_{2}^{T} \mathbf{M}_{\mathcal{K}_{2}}^{T} \mathbf{M}_{\mathcal{K}_{1}} \mathbf{x}_{1}   \leq (\delta_{2S}+ \delta_{S}) (\| \mathbf{x}_{1} \|^{2}_{2}+\| \mathbf{x}_{2} \|^{2}_{2}) \label{equ_proof_svd_rip_5}.
%\end{align}
%The inequality \eqref{equ_proof_svd_rip_4} follows from \eqref{equ_proof_svd_rip_3} because the matrix $\mathbf{M}$ also satisfies the RIP of order $S$ with $\delta_{S} \leq \delta_{2S} < 1$ and therefore 
%$(1-\delta_{S}) \| \mathbf{x}_{1} \|^{2}_{2}  \leq \| \mathbf{M}_{\mathcal{K}_{1}} \mathbf{x}_{1} \|^{2}_{2}  \leq (1+\delta_{S}) \| \mathbf{x}_{1} \|^{2}_{2}$ as well as $(1-\delta_{S}) \| \mathbf{x}_{2} \|^{2}_{2}  \leq \| \mathbf{M}_{\mathcal{K}_{2}} \mathbf{x}_{2} \|^{2}_{2}  \leq (1+\delta_{S}) \| \mathbf{x}_{2} \|^{2}_{2}$. 

%The statement follows then from \eqref{equ_proof_svd_rip_5} by choosing the vector $\mathbf{x} \in \mathbb{R}^{N}$ such that $\mathbf{x}_{1}$ and $\mathbf{x}_{2}$ 
%are the singular vectors \cite{golub96} of the matrix $\mathbf{M}_{\mathcal{K}_{2}}^{T} \mathbf{M}_{\mathcal{K}_{1}}$. 
%\end{proof}

We now specialize Theorem \ref{thm_bound_asilomar_2}  to the CS scenario for the SLM, i.e., where the system matrix $\mathbf{H}$ of the SLM is a CS measurement matrix $\mathbf{M}$ with known RIP constants.   
\begin{theorem}
\label{thm_CS_measur_matrix_asilomar_bound}
Consider the minimum variance problem $\mathcal{M}_{\text{\tiny{SLM}}}=\left( \mathcal{E}_{\text{\tiny{SLM}}}, c(\cdot), \mathbf{x}_{0} \right)$ 
with specific choices for $\sigma$, $S$, $M$, $N$, $\mathbf{x}_{0} \in \mathcal{X}_{S}$ and system matrix $\mathbf{H} = \mathbf{M}$, where $\mathbf{M} \in \mathbb{R}^{M \times N}$ is a CS measurement matrix satisfying the RIP of order $S$ 
with constant  $\delta_{S} < 1$. 

Then we have for an arbitrary set $\mathcal{K} =\{i_1,\ldots,i_{|\mathcal{K}|} \} \subseteq [N]$ consisting of no more than $S$ different indices, i.e., $|\mathcal{K}| \leq S$, and a 
prescribed bias $c(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}$ for which the partial derivatives 
$\frac{ \partial^{\mathbf{e}_{i_{l}}} c(\mathbf{x})}{\partial \mathbf{x}^{\mathbf{e}_{i_{l}}}}$ exist, that
\begin{equation}
\label{equ_CS_measur_matrix_asilomar_bound}
%L_{\mathcal{M}_{\text{\tiny{SLM}}}} \geq  \expÊ\bigg( - \big\| \mathbf{x}_{0}^{\supp(\mathbf{x}_{0}) \setminus \mathcal{K}} \big \|^{2}_{2}  \bigg[ (1+\delta_{S}) + \frac{(\delta_S + \delta_{2S})^2}{1-\delta_{S}} \bigg] \bigg) \mathbf{r}_{\mathbf{x}_{0}}^{T} \left( \mathbf{H}_{\mathcal{K}}^{T} 
L_{\mathcal{M}_{\text{\tiny{SLM}}}} \geq  \expÊ\bigg( - \frac{1+\delta_{S}}{\sigma^{2}} \big\| \mathbf{x}_{0}^{\supp(\mathbf{x}_{0}) \setminus \mathcal{K}} \big \|^{2}_{2}    \bigg) \mathbf{r}_{\mathbf{x}_{0}}^{T} \left( \mathbf{H}_{\mathcal{K}}^{T} 
\mathbf{H}_{\mathcal{K}} \right)^{-1} \mathbf{r}_{\mathbf{x}_{0}}. 
\end{equation} 
where  $\gamma(\cdot): \mathcal{X}_{S} \rightarrow \mathbb{R}: \gamma(\mathbf{x}) = c(\mathbf{x}) + x_{k}$, the vector $\widetilde{\mathbf{x}}_{0}$ is defined as in Theorem \ref{thm_bound_asilomar} and the vector $\mathbf{r}_{\mathbf{x}_{0}} \in \mathbb{R}^{|\mathcal{K}|}$ 
is defined element-wise as $r_{\mathbf{x}_{0},l} \triangleq \frac{ \partial^{\mathbf{e}_{i_{l}}} \gamma(\mathbf{x})}{\partial \mathbf{x}^{\mathbf{e}_{i_{l}}}} \big|_{\mathbf{x} = \widetilde{\mathbf{x}}_{0}}$. 
\end{theorem}
\begin{proof}
Denoting by $\mathbf{P}_{\mathcal{K}} \in \mathbb{R}^{M \times |\mathcal{K}|}$ the orthogonal projection matrix on the 
subspace $\linspan( \mathbf{M}_{\mathcal{K}} ) \subseteq \mathbb{R}^{M}$ we have 
that $\mathbf{P}_{\mathcal{K}} = \mathbf{M}_{\mathcal{K}} \left(\mathbf{M}_{\mathcal{K}}^{T}\mathbf{M}_{\mathcal{K}}\right)^{-1} \mathbf{M}_{\mathcal{K}}^{T}$ since $\mathbf{M}$ satisfies the RIP or order $2S$ which implies 
that $\mathbf{M}_{\mathcal{K}}$ has full column rank (cf. \cite{golub96}). 

We then have also that 
\begin{equation} 
(\mathbf{I} - \mathbf{P}_{\mathcal{K}})^{T} \mathbf{H}_{\mathcal{K}} = (\mathbf{I} - \mathbf{P}_{\mathcal{K}}) \mathbf{H}_{\mathcal{K}} = \mathbf{0} \nonumber
\end{equation} 
,i.e., for every vector $\mathbf{x}' \in \linspan(\mathbf{H}_{\mathcal{K}})$ we have that $ (\mathbf{I} - \mathbf{P}_{\mathcal{K}}) \mathbf{x}' = \mathbf{0}$. 
This implies that 
\begin{equation} 
\label{equ_slm_CS_proof_reformulation_factor}
(\mathbf{I} - \mathbf{P}_{\mathcal{K}})^{T} \mathbf{H} \mathbf{x}_{0} = 
(\mathbf{I} - \mathbf{P}_{\mathcal{K}})\mathbf{H} ( \mathbf{x}_{0}^{\supp(\mathbf{x}_{0}) \setminus \mathcal{K}}  + \mathbf{x}_{0}^{\mathcal{K}}) =  
(\mathbf{I} - \mathbf{P}_{\mathcal{K}})\mathbf{H} \mathbf{x}_{0}^{\supp(\mathbf{x}_{0}) \setminus \mathcal{K}},
\end{equation} 
since $\mathbf{H} \mathbf{x}_{0}^{\mathcal{K}} \in  \linspan(\mathbf{H}_{\mathcal{K}})$. 

Based on \eqref{equ_slm_CS_proof_reformulation_factor} and using the shorthand $\mathbf{x}'_{0} \triangleq  \mathbf{x}_{0}^{\supp(\mathbf{x}_{0}) \setminus \mathcal{K}}$ we have 
\begin{align}
\label{equ_slm_CS_inequ_rip}
\big \| (\mathbf{I} - \mathbf{P}_{\mathcal{K}} ) \mathbf{H} \mathbf{x}_{0} \big \|^{2}_{2} & = \big \| (\mathbf{I} - \mathbf{P}_{\mathcal{K}} ) \mathbf{H}\mathbf{x}_{0}' \big \|^{2}_{2}  \nonumber  \\ 
& =  \big \| \mathbf{H} \mathbf{x}'_{0} \big \|^{2}_{2} - 2 \left( \mathbf{x}'_{0} \right)^{T} \mathbf{H}^{T} \mathbf{P}_{\mathcal{K}} \mathbf{H}\mathbf{x}'_{0} + 
\left(\mathbf{x}'_{0} \right)^{T} \mathbf{H}^{T} \mathbf{P}^{2}_{\mathcal{K}} \mathbf{H}\mathbf{x}'_{0} \nonumber \\ 
& \stackrel{(a)}{=}  \big \| \mathbf{H}\mathbf{x}'_{0} \big \|^{2}_{2} - \left(\mathbf{x}'_{0}\right)^{T} \mathbf{H}^{T} \mathbf{P}_{\mathcal{K}} \mathbf{H}\mathbf{x}'_{0} \nonumber \\ 
%& =\big \| \mathbf{H}\mathbf{x}'_{0} \big \|^{2}_{2} - \left(\mathbf{x}'_{0}\right)^{T} \mathbf{H}^{T}  
%\mathbf{M}_{\mathcal{K}} \left(\mathbf{M}_{\mathcal{K}}^{T}\mathbf{M}_{\mathcal{K}}\right)^{-1} \mathbf{M}_{\mathcal{K}}^{T}  \mathbf{H}\mathbf{x}'_{0} \nonumber \\
%+ {\mathbf{x}'}_{0}^{T} \mathbf{H}^{T} \mathbf{P}_{\mathcal{K}} \mathbf{H}{\mathbf{x}'}_{0} \nonumber \\ 
& \stackrel{(b)}{\leq}  \big \| \mathbf{H}\mathbf{x}'_{0} \big \|^{2}_{2} \nonumber \\
& \stackrel{(c)}{\leq}  (1+\delta_{S}) \big \| \mathbf{x}'_{0} \big \|^{2}_{2},
\end{align} 
where the step $(a)$ follows from $\left( \mathbf{P}_{\mathcal{K}} \right)^{2} = \mathbf{P}_{\mathcal{K}}$ since $\mathbf{P}_{\mathcal{K}}$ is an orthogonal projection matrix (cf. \cite{golub96}), the 
step $(b)$ follows from the fact that $\mathbf{P}_{\mathcal{K}}$ is psd and $(c)$ is due to $\| \mathbf{x}_{0}' \|_{0} \leq S$ and the assumption that $\mathbf{H}=\mathbf{M}$ satisfies the RIP of order $S$ with constant $\delta_{S} < 1$.  
The statement follows then as a reformulation of \eqref{equ_bound_asilomar_2} from Theorem \ref{thm_bound_asilomar_2} using \eqref{equ_slm_CS_inequ_rip}. 
\end{proof}
 
Note that the condition \eqref{equ_spark_cond} is necessary for a matrix to have the RIP of order $S$ with a constant $\delta_{S}<1$. 
Moreover, for CS applications one favors in general measurement matrices $\mathbf{M}$ that have RIP constants close to zero, i.e., $\delta_{S} \approx 0$ (cf. \cite{Can06a}). However, in this 
case the bound in \eqref{equ_CS_measur_matrix_asilomar_bound} is nearly identical with the bound \eqref{equ_bound_asilomar_2} for the SLM with $\mathbf{H} = \mathbf{I}$. 

Thus if one uses a ``good'' CS measurement matrix, i.e., with RIP constant $\delta_{S}$ close to zero, then Theorem \ref{thm_CS_measur_matrix_asilomar_bound} suggests that the minimum achievable variance 
is close to the minimum achievable variance of the SLM with the same $S$, $N$ but with $\mathbf{H} = \mathbf{I}$ instead of the measurement matrix $\mathbf{M}$ which means that in terms of achievable estimation accuracy, 
there is no loss of information incurred by applying the CS measurement matrix $\mathbf{M} \in \mathbb{R}^{M \times N}$ and thereby reducing the signal dimension from $N$ to $M$, where $M \ll N$ in general. 

This agrees with the fact that if the RIP constants are sufficiently small then one can recover the sparse parameter vector $\mathbf{x} \in \mathcal{X}_{S}$ up to an 
accuracy that is solely determined by the noise (cf. \cite{Can06a,DantzigCandes}). 

The CS measurement model in \eqref{equ_measurment_equ_CS} assumes that the noise component is added after the measurement process. However, 
in some applications it might be more accurate to model to the effect of the noise before the measurement process takes place, i.e., to use the following measurement model: 
\begin{equation}
\label{equ_CS_model_noise_before_measurement}
\mathbf{y}' = \mathbf{M} (\mathbf{x} + \mathbf{n}) 
\end{equation}
where the meanings of $\mathbf{y}$, $\mathbf{H}$, $\mathbf{x}$ and $\mathbf{n}$ are the same as for \eqref{equ_measurment_equ_CS}. 

Note that the observation given by \eqref{equ_CS_model_noise_before_measurement} is obtained by applying a deterministic mapping, i.e., the matrix multiplication with $\mathbf{M}$ to the 
observation $\mathbf{y} = \mathbf{x} + \mathbf{n}$ of the SSNM.  

Therefore, if the CS measurement process is modeled by \eqref{equ_CS_model_noise_before_measurement}, then we can analyze the resulting minimum variance problem of estimating the 
sparse vector $\mathbf{x} \in \mathcal{X}_{S}$ based on the observation $\mathbf{y}'$ given by \eqref{equ_CS_model_noise_before_measurement}, 
using the results on the SSNM of Section \ref{sec_SSNM} together with Theorem \ref{thm_data_proc_inequ_classical_est} presented in Section \ref{sec_data_proc_inequ_classical_est}. 






%Interpreation: sobald man eine (kleine) Kugel im parameterset hat wird die menge aller erlaubten estimators soweit reduziert dass keine verbesserung der varianz moeglich ist. 

\section{Comparison of the Bounds with Existing Estimators} 
\label{sec_numerical_SLM}

Let us now compare the lower bounds derived so far with the actual variance behavior of some well known estimators. 




For the 
%% special case of the 
SSNM in \eqref{equ_observation_model_SSNM},
%%  with $S \!=\! 1$, 
we will compute the lower variance 
bound $\sum_{k=1}^{N} \rmv\rmv L_{\gamma_k}^*\rmv (\mathbf{x}_{0})$
(see \eqref{equ_lower_vec_est}) and compare it with the 
%% actual 
variance of two established estimators, namely, the maximum likelihood (ML) estimator and the hard-thresholding (HT) estimator.
The ML estimator is given by 
\[
%% \label{equ_ML_est}
\ML_est(\mathbf{y}) \,\triangleq\, \argmax_{\mathbf{x}' \in \mathcal{X}_{S}} f ( \mathbf{y};  \mathbf{x}' ) \ist=\, {\mathsf P}_{\!S} ( \mathbf{y}  ) \,,
\]
where the operator $\mathsf{P}_{\! S}$ retains the $S$ largest (in magnitude) entries and zeros out
all others. The HT estimator $\hat{\mathbf{x}}_{\text{HT}}  (\mathbf{y})$ is given 
\vspace{-.5mm}
by
\begin{equation}
\label{equ_def_thr_func}
\hat{x}_{\text{HT},k}  (\mathbf{y}) \eq \begin{cases} y_k \,,  & |y_k| \geq T\\[.5mm]
  0 \,, & \text{else} \ist,
\end{cases} 
\end{equation} 
where $T$ is a fixed threshold.
%% A popular choice for the threshold is $T= \sigma \sqrt{2 \log_{e} N}$  \cite{Mallat2008}. 

For simplicity, we consider the SSNM for $S \!=\! 1$.
In this case, the bound \eqref{equ_lower_vec_est} can be shown to 
\vspace{.5mm}
be
\begin{equation}
\label{equ_lower_bound_ml_ht}
v(\hat{\mathbf{x}}(\cdot); \mathbf{x}_0) \ist\geq\ist\ist L_{\gamma_{j}}^{\mathcal{K}_j}\rmv (\mathbf{x}_{0})
\ist+\ist (N \!-\! 1) \, e^{ - \xi^2(\mathbf{x}_{0}) / \sigma^{2}} L_{\gamma_{i}}^{\mathcal{K}_i}\rmv (\mathbf{x}_{0}) \,, 
\vspace{.5mm}
\end{equation} 
where $j \!\triangleq\! j(\mathbf{x}_{0})$, $i$ is any index different from $j(\mathbf{x}_{0})$ (it can be shown that all such indices equally maximize
the lower bound), $\mathcal{K}_{j} \!\triangleq\! \{ j(\mathbf{x}_{0}) \}$, and $\mathcal{K}_{i} \!\triangleq\! \{i \}$.
(We note that \eqref{equ_lower_bound_ml_ht} simplifies to \eqref{equ_lower_bound_unbiased_ssnm} for the special case of an unbiased estimator.)
%% As always, the function $\bm{\gamma}(\mathbf{x})$ involved in the bound 
%% %% on the right-hand side 
%% is the mean of the estimator $\hat{\mathbf{x}}(\cdot)$. 
%%   lower variance bound holds for any estimator $\hat{\mathbf{x}}(\cdot)$ with mean $\bm{\gamma}(\mathbf{x})$.
Since we 
%% consider specifically 
compare the bound \eqref{equ_lower_bound_ml_ht} to the ML and HT estimators, $\bm{\gamma}(\mathbf{x})$ is set equal to the 
mean of the respective estimator (ML or HT).

For a numerical evaluation, we generated parameter vectors $\mathbf{x}_0$ with $N\!\rmv=\!5$, $S\!=\!1$, $j(\mathbf{x}_{0}) \!=\! 1$, and different $\xi(\mathbf{x}_{0})$.
(The fixed choice $j(\mathbf{x}_{0}) \!=\! 1$ is justified by the fact that neither the variances of the ML and HT estimators nor the corresponding variance bounds depend on $j(\mathbf{x}_{0})$.)
In Fig.~\ref{fig_bounds_1}, we plot the variances $v(\ML_est(\cdot); \mathbf{x}_0)$ and $v( \hat{\mathbf{x}}_{\text{HT}} (\cdot); \mathbf{x}_0)$ 
(the latter for three different choices of 
%% the threshold parameter 
$T$ in \eqref{equ_def_thr_func}) along with the corresponding bounds \eqref{equ_lower_bound_ml_ht}, as a function of the signal-to-noise ratio (SNR) 
$\xi^{2}(\mathbf{x}_{0})/\sigma^{2}$. It is seen that for SNR larger than about 18 dB, %%% BLIBLABLU
%% 15\,dB, 
all variances and bounds are effectively equal (for the HT estimator, 
this is true if $T$ is not too small). However, in the medium-SNR
%% intermediate SNR 
range, the variances of the ML and HT estimators are significantly higher than
%% there is a significant gap between the actual variance performance of the ML and HT estimators and 
the corresponding lower bounds. 
We can conclude that there \emph{might} exist estimators with the same mean as that of the ML or HT estimator but a smaller variance.
%% (or MSE).  
Note, that a positive statement regarding the existence of an estimator that has the same mean of the ML or HT estimator but a uniformly lower variance cannot be 
based on our analysis. 

However, for the special case of diagonal estimators like the HT estimator, Theorem \ref{} makes a positive statement about the existence of estimators that 
have locally a smaller variance. 

% can only be given for esitmator with a diagonal bias function like the HT estimator. 
%For the ML estimator, our analysis does not allow for such a statement. 

\begin{figure}
\vspace{-1mm}
\centering
\psfrag{SNR}[c][c][.9]{\uput{3.4mm}[270]{0}{\hspace{3mm}SNR [dB]}}
\psfrag{title}[c][c][.9]{\uput{2.5mm}[270]{0}{}}
\psfrag{x_0}[c][c][.9]{\uput{0.3mm}[270]{0}{$0$}}
\psfrag{x_0_001}[c][c][.9]{\uput{0.3mm}[270]{0}{$-30$}}
\psfrag{x_0_01}[c][c][.9]{\uput{0.3mm}[270]{0}{$-20$}}
\psfrag{x_0_1}[c][c][.9]{\uput{0.3mm}[270]{0}{$-10$}}
\psfrag{x_1}[c][c][.9]{\uput{0.3mm}[270]{0}{$0$}}
\psfrag{x_10}[c][c][.9]{\uput{0.3mm}[270]{0}{$10$}}
\psfrag{x_100}[c][c][.9]{\uput{0.3mm}[270]{0}{$20$}}
\psfrag{y_0}[c][c][.9]{\uput{0.1mm}[180]{0}{$0$}}
\psfrag{y_1}[c][c][.9]{\uput{0.1mm}[180]{0}{}}
\psfrag{y_10}[c][c][.9]{\uput{0.1mm}[180]{0}{$10$}}
\psfrag{y_2}[c][c][.9]{\uput{0.1mm}[180]{0}{$2$}}
\psfrag{y_3}[c][c][.9]{\uput{0.1mm}[180]{0}{}}
\psfrag{y_4}[c][c][.9]{\uput{0.1mm}[180]{0}{$4$}}
\psfrag{y_5}[c][c][.9]{\uput{0.1mm}[180]{0}{}}
\psfrag{y_6}[c][c][.9]{\uput{0.1mm}[180]{0}{$6$}}
\psfrag{y_7}[c][c][.9]{\uput{0.1mm}[180]{0}{}}
\psfrag{y_8}[c][c][.9]{\uput{0.1mm}[180]{0}{$8$}}
\psfrag{y_9}[c][c][.9]{\uput{0.1mm}[180]{0}{}}
\psfrag{variancebound}[c][c][.9]{\uput{1mm}[90]{0}{variance/bound}}
\psfrag{bML}[l][l][0.8]{bound on $v(\ML_est(\cdot);\mathbf{x}_0)$}
\psfrag{ML}[l][l][0.8]{$v(\ML_est(\cdot);\mathbf{x}_0)$}
\psfrag{HT3}[l][l][0.8]{$v(\hat{\mathbf{x}}_{\text{HT}}(\cdot); \mathbf{x}_0)$, $T \!\rmv=\! 3$}
\psfrag{HT4}[l][l][0.8]{$v(\hat{\mathbf{x}}_{\text{HT}}(\cdot); \mathbf{x}_0)$, $T \!\rmv=\! 4$}
\psfrag{HT5}[l][l][0.8]{$v(\hat{\mathbf{x}}_{\text{HT}}(\cdot); \mathbf{x}_0)$, $T \!\rmv=\! 5$}
\psfrag{bHT3}[l][l][0.8]{bound on $v(\hat{\mathbf{x}}_{\text{HT}}(\cdot); \mathbf{x}_0)$, $T \!\rmv=\! 3$}
\psfrag{bHT4}[l][l][0.8]{bound on $v(\hat{\mathbf{x}}_{\text{HT}}(\cdot); \mathbf{x}_0)$, $T \!\rmv=\! 4$}
\psfrag{bHT5}[l][l][0.8]{bound on $v(\hat{\mathbf{x}}_{\text{HT}}(\cdot); \mathbf{x}_0)$, $T \!\rmv=\! 5$}
\psfrag{MLarrow}[l][l][0.8]{ML}
\psfrag{T3}[l][l][0.8]{HT \!($T \!\rmv=\! 3$)}
\psfrag{T4}[l][l][0.8]{HT \!($T \!\rmv=\! 4$)}
\psfrag{T5}[l][l][0.8]{HT \!($T \!\rmv=\! 5$)}
\centering
\hspace*{-0mm}\includegraphics[height=7cm,width=13cm]{var_bound_ML_HT_ssnm.eps}
\vspace{-2.5mm}
  \caption{$\hspace*{-2mm}$Variance of the ML and HT estimators and corresponding lower bounds versus the SNR $\xi^{2}(\mathbf{x}_{0})/\sigma^{2}\rmv\rmv$,
  for the SSNM
  %% SLM with $\mathbf{H}=\mathbf{I}$, 
  with $N\!=\!5$ and $S\!=\!1$.} %%  and $\sigma^{2}=1$
\label{fig_bounds_1}
\vspace*{-2mm}
\end{figure}



Compare with Hard, Soft-Thresholding, ML - Estimator, Basis Pursuit, OMP, Ad-hoc Scheme which first detects the support and the estimates non-zeros. 





